Nonparametric Bootstrap Inference for the Targeted Highly Adaptive LASSO Estimator

The Highly-Adaptive-LASSO Targeted Minimum Loss Estimator (HAL-TMLE) is an efficient plug-in estimator of a pathwise differentiable parameter in a statistical model that at minimal (and possibly only) assumes that the sectional variation norm of the true nuisance functional parameters (i.e., the relevant part of data distribution) are finite. It relies on an initial estimator (HAL-MLE) of the nuisance functional parameters by minimizing the empirical risk over the parameter space under the constraint that the sectional variation norm of the candidate functions are bounded by a constant, where this constant can be selected with cross-validation. In this article, we establish that the nonparametric bootstrap for the HAL-TMLE, fixing the value of the sectional variation norm at a value larger or equal than the cross-validation selector, provides a consistent method for estimating the normal limit distribution of the HAL-TMLE. In order to optimize the finite sample coverage of the nonparametric bootstrap confidence intervals, we propose a selection method for this sectional variation norm that is based on running the nonparametric bootstrap for all values of the sectional variation norm larger than the one selected by cross-validation, and subsequently determining a value at which the width of the resulting confidence intervals reaches a plateau. We demonstrate our method for 1) nonparametric estimation of the average treatment effect based on observing on each unit a covariate vector, binary treatment, and outcome, and for 2) nonparametric estimation of the integral of the square of the multivariate density of the data distribution. In addition, we also present simulation results for these two examples demonstrating the excellent finite sample coverage of bootstrap-based confidence intervals.

==> archive.tex <==
\subsection{Why does it work, and how it applies to adaptive TMLE}

The key behind the validity of the nonparametric bootstrap for estimation of the sampling distribution of the HAL-MLE and HAL-TMLE is that the HAL-MLE is an actual MLE thereby avoiding data adaptive trade-off of bias and variance as naturally achieved with cross-validation.
However, even though the inference is based on such a non-adaptive HAL-TMLE, one can still use an highly adaptive HAL-TMLE as point estimate in  our reported confidence intervals. Specifically, one can  use our confidence intervals with the point estimate defined as  a TMLE using a super-learner \citep{vanderLaan&Dudoit03,vanderVaart&Dudoit&vanderLaan06,vanderLaan&Dudoit&vanderVaart06,vanderLaan&Polley&Hubbard07,Chpt3} that includes the HAL-MLE as one of the candidate estimators in its library. By the oracle inequality for the cross-validation selector, such a super-learner will improve on the HAL-MLE so that the proposed inference based on the non-adaptive HAL-TMLE will be more conservative. In addition, our confidence intervals can be used with the point estimate defined by adaptive TMLEs incorporating additional refinements such as collaborative TMLE \citep{vanderLaan:Gruber10,Gruber:vanderLaan10a,Stitelman:vanderLaan10,vanderLaan:Rose11,Wang:Rose:vanderLaan11,gruber2012ijb}; cross-validated TMLE
\citep{Zheng&vanderLaan12,vanderLaan&Rose11}; higher order TMLE \citep{Carone2014techreport,Caroneetal17,diaz2016ijb};  and double robust inference TMLE \citep{vanderLaan14a,Benkeseretal17}. Again, such refinements generally improve the finite sample accuracy of the estimator, so that  it will improve the coverage of the confidence intervals based on the non-adaptive HAL-TMLE.

Our confidence intervals can also be used if the statistical model ${\cal M}$ has  no known bound on the sectional variation norm of the nuisance parameters. In that case, we recommend  to select such a  bound with cross-validation (just as one selects the $L_1$-norm penalty in Lasso regression with cross-validation), which, by the oracle inequality for the cross-validation selector \citep{vanderLaan&Dudoit03,vanderVaart&Dudoit&vanderLaan06,vanderLaan&Dudoit&vanderVaart06}
is guaranteed to be larger that the  sectional variation norm of the true nuisance parameters $(Q_0,G_0)$  with probability tending to 1. In that case, the confidence intervals will still be asymptotically correct, incorporate most of the higher order variability, but ignores the potential finite sample underestimation of the true sectional variation norm.    In addition, in that case the inference adapts to the underlying unknown  sectional variation norm of the true nuisance parameters $(Q_0,G_0)$. We plan to evaluate the practical performance of our  methods in the near future.

\subsection{Relation to literature on higher order influence functions}
J. Pfanzagl \citep{pfanzagl1985} introduced the notion of higher order pathwise differentiability of finite dimensional target parameters and corresponding higher order gradients. He used these higher order expansions of the target parameter to define higher order one-step estimators that might result in asymptotically linear estimators where regular one-step estimators \citep{levit1975,ibragimov1981,pfanzagl1982,bickel1982annals} might fail to behave well due to a too large second-order remainder.
 This is the perspective that inspired the seminal contributions of J. Robins, L. Li, E. Tchetgen \& A. van der Vaart (e.g., \citealp{robins2008imsnotes,robins2009metrika,li2011statsprobletters,vandervaart2014statscience}).  They develop a rigorous theory for (e.g.)  second-order one-step estimators, including the typical case that the parameter is not second-order pathwise differentiable. They allow the case that the second-order remainder asymptotically dominates the first order term, resulting in estimators and confidence intervals that converge to zero at a slower rate than $n^{-1/2}$. Their second-order expansion uses  approximations of ''would be'' second-order gradients, where the approximation results in a bias term they termed the representation error. Unfortunately, this representation error, due to the lack of second order pathwise differentiability, obstructs the construction of estimators with a third order remainder (and thereby asymptotic linearity under the condition that a third order term is $o_P(n^{-1/2})$) These second-order one-step estimators involve careful selection of tuning/smoothing parameters for approximating the ''would be'' second-order gradient in order to obtain an optimal bias-variance trade-off.  These authors applied their theory to nonparametric estimation of a mean with missing data and the  integral of the square of the density.
 The higher-order expansions that come with the construction of higher order one-step estimators  can be  directly incorporated in
the construction of confidence intervals, thereby possibly leading to improved finite sample  coverage. These higher order expansions  rely on hard to estimate objects such as a multivariate density in a denominator, giving rise to enormous practical challenges to construct robust higher order confidence intervals, as noted in the above articles.

 \cite{pfanzagl1982} already pointed out that the one-step estimators and till a larger degree higher order one-step estimators fail to respect global known bounds implied by the model and target parameter mapping, by adding to an initial estimator  an empirical mean of a first order influence function and higher order U-statistics (i.e. higher orders empirical averages) of higher order influence functions. He suggested that to circumvent this problem one would have to carry out the updating process in the model space instead of in the parameter space. This is precisely what is carried out by the general TMLE framework \citep{vanderLaan&Rubin06,vanderLaan&Rose11}, and higher order TMLE based on approximate higher order influence functions were developed in \citep{Carone2014techreport,diaz2016ijb,Caroneetal17}. These higher order TMLE represents the TMLE-analogue of higher order one-step estimators, just as the regular TMLE is an analogue of the regular one-step estimator.
 These TMLEs automatically satisfy the known bounds and thus never produce non-sensical output such a negative number for a probability.  The higher order TMLE is just another TMLE but using  a least favorable submodel with an extra parameter, thereby providing a crucial safeguard against erratic behavior due to estimation of the higher order influence functions, while also being able to utilize the C-TMLE framework to select the tuning parameters for approximating these higher order influence functions.

%A higher-order expansions that come with the construction of higher order one-step estimators and higher order TMLE can be  directly incorporated inthe construction of confidence intervals, thereby possibly leading tofinite-sample performance improvements. In that sense, this literature is related to the goal of finite sample inference set out in this article.

The approach in this article for construction of higher order confidence intervals is quite different from the construction of higher order one-step estimators or higher order TMLE and using the corresponding higher order expansion for inference. To start with, we use an asymptotically efficient HAL-TMLE so that we preserve the $n^{-1/2}$-rate of convergence, asymptotic normality and efficiency, even in nonparametric models that only assume that the true nuisance parameters have finite sectional variation norm. As point estimate we can still use an adaptive HAL-TMLE which can, for example, include the  higher-order HAL-TMLE refinement, beyond refinements mentioned above. However, for inference,  we avoid the  delicate higher order expansions based on approximate higher order gradients, but instead use the exact second-order expansion $\Psi(Q_n^*)-\Psi(Q_0)=(P_n-P_0)D^*(Q_n^*,G_n)+R_{20}(Q_n^*,G_n,Q_0,G_0)$  implied by the definition of the exact second-order remainder $R_{20}()$ (\ref{exactremainder}), which thus incorporates any higher order term. In addition, by using the robust HAL-MLE as estimators of $Q_0,G_0$,  the HAL-TMLE is not only efficient but  one can also use nonparametric bootstrap to estimate its sampling distribution. We then  use the nonparametric bootstrap to estimate the sampling distribution of HAL-TMLE itself, or its exact expansion, or an exact conservative expansion in which $R_{20}()$ is replaced by a robust upper bound which only depends on well behaved empirical processes for which the nonparametric bootstrap works  (again, due to using the HAL-MLE). Our confidence intervals have width of order $n^{-1/2}$ and are asymptotically sharp by converging to the optimal normal distribution based confidence interval as sample size increases. In addition, they are easy to implement as a by product of the computation of the HAL-TMLE itself.


% ==================================================================


\paragraph{Super learner including HAL-MLE outperforms HAL-MLE}
Suppose that we estimate $Q_0$ and $G_0$ instead with super-learners $\tilde{Q}_n,\tilde{G}_n$  in which the library of the super-learners contains this HAL-MLE $Q_n$ and $G_n$. Then, by the oracle inequality for the super-learner, we know that 
$d_{01}(\tilde{Q}_n,Q_0)$ and $d_{02}(\tilde{G}_n,G_0)$ will be asymptotically equivalent with the oracle selected estimator, so that $d_{01}(Q_n,Q_0)$ and $d_{02}(G_n,G_0)$ represent asymptotic upper bounds for $d_{01}(\tilde{Q}_n,Q_0)$ and $d_{02}(\tilde{G}_n,G_0)$ \citep{vanderLaan15}.
In addition, practical experience has demonstrated that the super-learner outperforms its library candidates in finite samples. 
% or at least has a very similar performance than its best candidate.  
Therefore, assuming that each estimator in the library of the super-learners for $Q_0$ and $G_0$  falls in the parameter spaces ${\cal F}_1$ and ${\cal F}_2$ of $Q$ and $G$, respectively, our proposed  estimators of the sampling distribution of the HAL-TMLE can also be used to construct a confidence interval around the super-learner based TMLE. These width of these confidence intervals are not adapting to possible superior performance of the  super-learner and could thus be overly conservative in case the super-learner outperforms the HAL-MLE.
%If $C_j$ is truly a known upper bound, then it is recommended that the library only contains candidate estimators that are included in the parameter space ${\cal F}_j$, such as HAL-MLEs for subsets of ${\cal F}_j$. 
% ==================================================================

\subsection{Motivation for finite sample inference}

In order to understand how large the exact remainder $\tilde{R}_{2n}$ could be relative to the leading first order term, we need to understand the size of $d_{01}(Q_n,Q_0)$ and $d_{02}(G_n,G_0)$. This will then motivate us to propose methods that estimate the finite sample distribution of the HAL-TMLE or conservative versions thereof.

%Motivate need for better methods by saying theoretically how fast/slow $d_{01}(Q_n^*,Q_0)$ $d_{02}(G_n,G_0)$ converges in terms of $M_j $ and $d$.so use intergraiotn by parts bound we have below. $\sqrt{d}$. so   say bound could easily be bigger than main term. 
To establish this behavior of $d_{01}(Q_n,Q_0)$ we will use the following general integration by parts formula, and a resulting bound.

\begin{lemma}\label{lemmaip}
Let $F,Z\in D_d[0,\tau]$. 
%For a $F\in D_d[0,\tau]$ define the supremum norm $\pl F\pl_{\infty}=\sup_{x\in [0,\tau]}\mid F(x)\mid$ and its sectional variation norm as follows:\[ \pl F\pl_v^*=F(0)+\sum_{s\subset\{1,\ldots,d\}}\int_{(0_s,x_s]} dF_s(u_s),\] where$F_s(u_s)=F(u_s,0_{-s})$ is the $s$-specific section of $F$ that sets the coordinates in the complement of $s$ equal to 0.For any cadlag function $F\in D[0,\tau]$ with $\pl F\pl_v^*<\infty$, we have\[F(x)=F(0)+\sum_{s\subset\{1,\ldots,d\}}\int_{(0_s,x_s]} dF_s(u_s).\]
For a given function $Z\in D_d[0,\tau]$ we define
\[
\bar{Z}(u)=Z([u,\tau])=\int_{[u,\tau]} dZ(s),\]
the measure $dZ$ assigns to the cube $[u,\tau]$, which is a generalized difference across the $2^d$-corners of $[u,\tau]$ \citep{Gill&vanderLaan&Wellner95}.
For any two functions $F,Z\in D[0,\tau]$ with $\pl F\pl_v^*<\infty$ and $\pl Z\pl_v^*<\infty$, we have the following integration by parts formula:
\[
\int_{[0,\tau]} F(x)dZ(x)=F(0)\bar{Z}(0) +\sum_s \int_{u_s} \bar{Z}(u_s,0_{-s})dF_s(u_s).\]
This implies 
\[
\int_{[0,\tau]} F(x)dZ(x)\leq \pl \bar{Z}\pl_{\infty}\pl F\pl_v^* .\]
\end{lemma}
{\bf Proof:}
The representation of $F(x)$ is presented in \citep{Gill&vanderLaan&Wellner95,vanderLaan15}. Using this representation yields the presented integration by parts formula as follows:
\begin{eqnarray*}
\int F dZ&=&\int \{F(0)+\sum_s \int_{(0_s,x_s]} dF_s(u)\} dZ(x)\\
&=&F(0) Z([0,\tau])+\sum_s \int_x\int_{u_s} I_{x_s\geq u_s} dF_s(u_s)dZ(x)\\
&=& F(0)Z([0,\tau])+\sum_s \int_{u_s} Z([u_s,\tau_s]\times [0_{-s},\tau_{-s}]) dF_s(u_s)\\
&\leq & \max_s \sup_{u_s\in [0_s,\tau_s]}\mid Z ([u_s,\tau_s]\times [0_{-s},\tau_{-s}])\mid \pl F\pl_v^*\\
&=& \pl Z\pl_{\infty} \pl F\pl_v^*.\Box
\end{eqnarray*}

For a $P\in {\cal M}$ and $P=P_n$ we define
\[
\bar{P}(u)=P([u,\tau])=\int_{[u,\tau]} dP(s).\]

By Lemma \ref{lemmaip}, we have
\begin{eqnarray*}
d_{01}(Q_n,Q_0)&\leq & \pl \bar{P}_n-\bar{P}_0\pl_{\infty}\pl L_1(Q_n,Q_0)\pl_v^* \\
d_{02}(G_n,G_0)&\leq &\pl \bar{P}_n-\bar{P}_0\pl_{\infty}\pl L_2(G_n,G_0)\pl_v^* .
\end{eqnarray*}
By \citep{vanderVaart&Wellner11}, we can bound the expectation of the  supremum norm of an empirical process over a  class of functions with uniformly bounded envelope  by the entropy integral:
\[
E\pl \sqrt{n}(\bar{P}_n-\bar{P}_0)\pl_{\infty}\lesssim J(1,{\cal F}_I)\equiv \sup_Q \int_{0}^1 \sqrt{\log N(\epsilon,L^2(Q),{\cal F}_I)} d\epsilon .\]
The covering number $N(\epsilon,L^2(Q),{\cal F}_I)$ for the class of indicators ${\cal F}_I=\{I_{[u,\tau]}:u\in [0,\tau]\}$ behaves as $\epsilon^{-d}$.   
This proves that
$E\pl \sqrt{n}(\bar{P}_n-\bar{P}_0)\pl_{\infty}=O(d^{1/2})$,
and thus
\begin{eqnarray*}
Ed_{01}(Q_n,Q_0)&=& O(d^{1/2}n^{-1/2}M_1)\\
Ed_{02}(G_n,G_0)&=& O(d^{1/2}n^{-1/2}M_2).
\end{eqnarray*}
In particular, this shows that the exact second-order remainder (\ref{exactremainder}) can be bounded in expectation as follows:
\[
E\mid \tilde{R}_{2n} \mid =O(n^{-1/2}d^{1/2} \sqrt{M_1M_2}).\]
Even though these bounds are overly conservative, these bounds provide a clear indication how the size of $d_{01}(Q_n,Q_0)$ and $d_{02}(G_n,G_0)$, and thereby the second-order remainder is  potentially affected by the dimension $d$ (i.e., for nonparametric models) and the allowed complexity of the model as measured by the bounds $M_1,M_2$.

One can thus conclude that there are many settings in which the exact second-order remainder $\tilde{R}_{2n}$ will dominate the leading linear term $(P_n-P_0)D^*(P_0)$ in finite samples.
Therefore, for the sake of accurate inference we will need methods that estimate the actual finite sample sampling distribution of the HAL-TMLE.


%In fact, we have that the (Corollary 2.2.5, van der Vaart, Wellner, 1996) the $\psi_1$-orlics norm $\pl\cdot\pl_{\psi_1}$ of $\pl \sqrt{n}(P_n-P_0)\pl_{\infty}$ is bounded by $J(1,{\cal F})$, which shows that
%\[\pl \pl n^{1/2}/d^{1/2}(\bar{P}_n-\bar{P}_0)\pl_{\infty} \pl_{\psi_1}=O(1),\]where $\psi_p(x)=\exp(x^p)-1$.This bound on the orlics norm of the supremum implies a bound on its tail probability \citep{vanderVaart&Wellner96}:\[P(\pl n^{1/2}/d^{1/2}(\bar{P}_n-\bar{P}_0)\pl_{\infty}>x)\leq \exp(-C x)\]for some $C<\infty$.Thus, this proves the following lemma.\begin{lemma}For some $C<\infty$, \[P(n^{1/2}d_{01}(Q_n,Q_0)>x)\leq P( \pl n^{1/2}/d^{1/2}(\bar{P}_n-\bar{P}_0)\pl_{\infty}M_1>x/d^{1/2})\leq \exp(-C x/(d^{1/2}M_1) ).\]Similarly, \[P(n^{1/2}d_{02}(G_n,G_0)>x)\leq P( \pl n^{1/2}/d^{1/2}(\bar{P}_n-\bar{P}_0)\pl_{\infty}M_2>x/d^{1/2})\leq \exp(-C x/(d^{1/2}M_2) ).\]\end{lemma}
%Similarly,\begin{eqnarray*}P(\mid \sqrt{n}R_{2n}\mid >x)&\leq& P(\delta^{-1} \pl \sqrt{n}(P_n-P_0)\pl_{\infty,1} \sqrt{M_1M_2} >x)\\&=& P(\pl \sqrt{n}(P_n-P_0)\pl_{\infty,1}> x\delta/\sqrt{M_1M_2})\\&\leq& \exp(-C\delta x/\sqrt{M_1M_2}).\end{eqnarray*}
%These bounds are of theoretical interest since they demonstrate the impact of the bounds $M_1,M_2$ on the sectional variation norm of $L_1(Q_n,Q_0)$ and $L_2(G_n,G_0)$ and of the dimension $d$ of the data $O$. 


%General point. we need to work with bound $\sup_P \max_{\epsilon}\pl L_1(P_{\epsilon})\pl_v^*$ so that this bound applies to $Q_n^*$!So our bounds $M_1,M_3$ need to take this into account! May be we can keep the $M_1,M_2$ as earlier and then denote these bounds with $M_1^*$ and $M_3^*$.

\subsection*{A very conservative finite sample confidence interval}
Consider the case that $r_n=0$.
Let ${\bf M}_1^*=\sup_{P\in {\cal M}}\max_{\epsilon}\pl {\bf L}_1(Q(P)_{\epsilon})\pl_v^*$ and ${\bf M}_2=\sup_{P\in {\cal M}}\pl {\bf L}_2(G(P))\pl_v^*$ be the  deterministic upper bound on the sectional variation norms of  ${\bf L}_1(Q_n^*)$ and ${\bf L}_2(G_n)$. 
 Let $\bar{Z}_n=n^{1/2}(\bar{P}_n-\bar{P}_0)$. The integration by parts bound applied to (\ref{exactexpansiontmle}) yields the following bound:
 \begin{eqnarray*}
\mid n^{1/2}(\Psi(Q_n^*)-\Psi(Q_0))\mid&\leq& \pl D^*(Q_n^*,G_n)\pl_v^*\pl \bar{Z}_n\pl_{\infty}\\
&&\hspace*{-2cm}
+f(\pl {\bf L}_1(Q_n^*,Q_0)\pl_v^{*1/2}\pl \bar{Z}_n\pl_{\infty}^{1/2},\pl {\bf L}_2(G_n,G_0)\pl_v^{*1/2}\pl\bar{Z}_n\pl_{\infty}^{1/2}) .\end{eqnarray*}
Let $M_3^*\equiv \sup_{P\in {\cal M}}\max_{\epsilon}\pl D^*(Q(P)_{\epsilon},G)\pl_v^*$. Then, we obtain the following bound:
\begin{equation}\mid n^{1/2}(\Psi(Q_n^*)-\Psi(Q_0))\mid\leq \left\{ M_3^*+f({\bf M}_1^{*1/2},{\bf M}_2^{1/2})\right\} \pl \bar{Z}_n\pl_{\infty}.\label{consbound}
\end{equation}
 Let $q_{n,0.95}$ be the $0.95$-quantile of $\pl \bar{Z}_n\pl_{\infty}$. A conservative finite sample $0.95$-confidence interval is then given by:
 \[
 \Psi(Q_n^*)\pm C({\bf M}_1^*,{\bf M}_2,M_3^*)q_{n,0..95}/n^{1/2},\]
where $C({\bf M}_1,{\bf M}_2,M_3)= M_3+f({\bf M}_1^{1/2},{\bf M}_2^{1/2})$.
One could estimate the distribution of $\bar{Z}_n$ with the nonparametric bootstrap and thereby obtain an bootstrap-estimate $q_{n,0.95}^{\#}$ of $q_{n,0.95}$.
One could push the conservative nature of this confidence interval further by using theoretical bounds for the tail-probability $P(\pl \bar{Z}_n\pl_{\infty}>x)$
and define the quantile $q_{n,0.95}$ in terms of this theoretical upper bound (such exponential bounds are available in (e.g.) \citep{vanderVaart&Wellner96}, but the constants in these exponential bounds appear to not  be concretely specified).



 The bound (\ref{consbound}) simplifies if we focus on the sampling distribution of the one-step estimator $\psi_n^1=\Psi(Q_n)+P_n D^*(Q_n,G_n)$ by being able to replace the targeted version $Q_n^*$ by $Q_n$.
 For the one-step estimator we have
 \[
 \psi_n^1-\psi_0=(P_n-P_0)D^*(Q_n,G_n)+R_{20}(Q_n,G_n,Q_0,G_0) .\]
 Let ${\bf M_1}=\sup_{P\in {\cal M}}\pl {\bf L}_1(Q(P))\pl_v^*$ and ${\bf M}_2=\sup_{P\in {\cal M}}\pl {\bf L}_2(G(P))\pl_v^*$ be the upper bound on the sectional variation norms of ${\bf L}_1(Q_n)$ and ${\bf L}_2(G_n)$.
% Let $\bar{Z}_n=n^{1/2}(\bar{P}_n-\bar{P}_0)$. The integration by parts bound applied to (\ref{exactexpansiontmle}) yields the following bound:
Analogue to above, we obtain
 \begin{eqnarray*}
\mid n^{1/2}(\psi_n^1-\Psi(Q_0))\mid&\leq& \pl D^*(Q_n,G_n)\pl_v^*\pl \bar{Z}_n\pl_{\infty}\\
&&\hspace*{-2cm}
+f(\pl {\bf L}_1(Q_n,Q_0)\pl_v^{*1/2}\pl \bar{Z}_n\pl_{\infty}^{1/2},\pl {\bf L}_2(G_n,G_0)\pl_v^{*1/2}\pl\bar{Z}_n\pl_{\infty}^{1/2}) .\end{eqnarray*}
Recall $M_3\equiv \sup_{P\in {\cal M}}\pl D^*(P)\pl_v^*$. Then, we obtain the following conservative sampling distribution:
\begin{equation}
Z_n^+\equiv \mid n^{1/2}(\psi_n^1-\Psi(Q_0))\mid\leq \left\{ M_3+f({\bf M}_1^{1/2},{\bf M}_2^{1/2})\right\} \pl \bar{Z}_n\pl_{\infty},\label{consbound1}
\end{equation}
% Let $q_{n,0.95}$ be the $0.95$-quantile of $\pl \bar{Z}_n\pl_{\infty}$. 
and  conservative finite sample $0.95$-confidence interval 
 \[
 \psi_n^1\pm C({\bf M}_1,{\bf M}_2,M_3)q_{n,0..95}/n^{1/2},\]
where $C({\bf M}_1,{\bf M}_2,M_3)= M_3+f({\bf M}_1^{1/2},{\bf M}_2^{1/2})$. Clearly, this same confidence interval can be applied to the TMLE  since the TMLE is asymptotically equivalent with the one-step estimator and generally performs better in finite samples by being a substitution estimator. 
%rarely worse in finite samples than the one-step estimator, but potentially significantly better. 
 
 Above, we pointed out that  $\pl \bar{Z}_n\pl_{\infty}=O_P((n/d)^{-1/2})$, which shows that this confidence interval has a width of order $(n/d)^{-1/2}$.
 This confidence interval is not only finite sample conservative but is also not  asymptotically sharp. 
 %Nonetheless, it demonstrates the effect of the dimension $d$ and of the sectional variation norm bounds $M_1,M_2,M_3$ on the finite sample width of the confidence interval.
Nonetheless, this formula appears to demonstrate  that the dimension $d$ of the data $O$ enters directly into the rate of convergence as $(n/d)^{1/2}$. In addition, it shows  and that the actual bounds $(C_1^u,C_2^u)$ on the sectional  variation norms of $Q$ and $G$ are directly affecting the width of the confidence interval (essentially linearly).
 In addition, the dimension $d$ itself naturally affects the chosen upper bounds $(C_1^u,C_2^u)$ and thereby ${\bf M}_1,{\bf M}_2,M_3$, so that the dimension $d$ may also affect the width of the finite sample confidence interval through the constant $C({\bf M}_1,{\bf M}_2,M_3)$. 
 
 Though interesting,  we suggest that in most applications this bound is much too conservative for practical use. This motivates us to construct much more accurate estimators of the actual sampling distribution of the HAL-TMLE.
 
 The above finite sample bound could also be applied to choices $M_{1n},M_{2n},M_{3n}$ implied by the cross-validation selector $(C_{1n},C_{2n})$ of $(C_1,C_2)$. We suggest that this would make the resulting confidence interval more reasonable, by not being so conservative (by being forced to select conservative upper bounds $C^u=(C_1^u,C_2^u)$). 
%\subsection{Conservative bound}Show here most conservative approach.


%I THINK WE MIGHT MOVE THE BOOTSTRAP FOR HAL-MLE TO APPENDIX AND FOCUS ON PRESENTIN GTHEOREM FOR HAL-TMLE. THEN DO NOT HAVE TO REPEAT THE LOSS FUNCTIN ASSUMPTIONS, CAN REVIEW OUR FORMAL RESULT FOR HAL-MLE AFTER HAVING DEFINED LOSS FUNCTION ASSUMPTIONS.

%do also the np bootstrap theorem at $C_n$ instead of fixed $C$.
% ==================================================================

\paragraph{Remark regarding robustness in underlying data distribution}
Consider the exact second order remainder $R_{20}$  for the HAL-TMLE $\Psi(Q_n^*)-\Psi(Q_0)=(P_n-P_0)D^*(Q_0,G_0)+R_{20}(Q_n^*,G_n,Q_0,G_0)$
and the exact second order remainder $R_{2n}^{\#}$  for the bootstrapped HAL-TMLE $\Psi(Q_n^{\#*})-\Psi(Q_n^*)=(P_n^{\#}-P_n)D^*(Q_n,G_n)+R_{2n}^{\#}$, as specified in the above proof. Under our model assumptions, the bounding of these two remainders only concern empirical processes $(P_n-P_0)$ and $(P_n^{\#}-P_n)$ indexed by a uniform Donsker class. As shown in \citep{vanderVaart&Wellner96}, such empirical processes converge and satisfy exact finite sample bounds that apply uniformly in all possible data distributions. 
Therefore, it follows that we can also establish that the nonparametric bootstrap is consistent for the normal limit distribution of the HAL-TMLE, {\em uniformly in all $P_0\in {\cal M}$}. This would mean that there exist sufficient sample sizes to obtain a particular level of precision in approximating  the normal limit distribution, uniformly in all $P_0\in {\cal M}$. This further demonstrates the robustness of the HAL-MLE, HAL-TMLE, and its bootstrap distribution in statistical models that have uniform model bounds $(M_1,M_2,M_3)$.

% ==================================================================

\subsection{The nonparametric bootstrap for the exact second-order expansion of the HAL-TMLE}
Recall the exact second-order expansion of the HAL-TMLE:
\begin{equation}\label{displ}
n^{1/2}(\Psi(Q_n^*)-\Psi(Q_0))=n^{1/2}(P_n-P_0)D^*(Q_n^*,G_n)+n^{1/2}R_{20}(Q_n^*,G_n,Q_0,G_0).\end{equation}
Recall that $R_{20}(Q,G,Q_0,G_0)=R_{2P_0}(Q,G,Q_0,G_0)$ potentially depends on $P_0$ beyond $(Q_0,G_0)$. 
Typically, we have 
\begin{equation}
R_{2P_0}(Q,G,Q_0,G_0)=P_0 R_2(Q,G,Q_0,G_0)\mbox{ for some $R_2(Q,G,Q_0,G_0)$.}\label{P0repR2}
\end{equation}
Let $R_{2n}()=R_{2P_n}()$ be obtained by replacing the $P_0$ by the empirical measure $P_n$. Thus, if we have (\ref{P0repR2}), then 
$R_{2n}(Q,G,Q_n,G_n)=P_n R_2(Q,G,Q_n,G_n)$.
 We assume the analogue of the bound (\ref{boundingR2}) on $R_{20}$ for $R_{2n}$:
\begin{equation}\label{boundingR2n}
\mid R_{2n}(Q,G,Q_n,G_n)\mid \leq f({\bf d}_{n1}^{1/2}(Q,Q_n),{\bf d}_{n2}^{1/2}(G,G_n))\end{equation}
for some function $f:\openr^K_{\geq 0}\rightarrow\openr_{\geq 0}$, $K=K_1+K_2$ of the form $f(x)=\sum_{i,j} a_{ij} x_ix_j$, a quadratic polynomial with positive coefficients $a_{ij}\geq 0$. 

Consider the nonparametric bootstrap analogue of the right-hand side of (\ref{displ}):
\[
Z_n^{2,\#}=n^{1/2}(P_n^{\#}-P_n)D^*(Q_n^{\#*},G_n^{\#})+n^{1/2}R_{2n}(Q_n^{\#*},G_n^{\#},Q_n^*,G_n).\]
This bootstrap sampling distribution $Z_n^{\#*}$ provides a very direct estimate of the sampling distribution of $n^{1/2}(\Psi(Q_n^*)-\Psi(Q_0))$.

Let $\Phi_n^{\#}(x)=P(Z_n^{2,\#}\leq x\mid P_n)$  be the cumulative distribution of this bootstrap sampling distribution.
So a bootstrap based 0.95-confidence interval for $\psi_0$ is given by \begin{equation}\label{ciexactexp}
[\psi_n^{*}+q_{0.025,n}^{\#}/n^{1/2},\psi_n^*+q_{0.975,n}^{\#}/n^{1/2} ],\end{equation}
 where 
$q_{\alpha,n}^{\#}=\Phi_n^{\#-1}(\alpha)$ is the $\alpha$-quantile of this bootstrap distribution. 



\begin{theorem}\label{thnpbootexactexp}
Under the same conditions as Theorem \ref{thnpboothaltmle} and condition (\ref{boundingR2n}), we have 
$Z_n^{2,\#}=n^{1/2}(P_n^{\#}-P_n)D^*(Q_n,G_n)+O_P(n^{-1/2-\alpha(d)})$, and thereby
\[
Z_n^{2,\#}\Rightarrow_d N(0,\sigma^2_0)\mbox{ conditional on $(P_n:n\geq 1)$}.\]
In particular the above confidence interval (\ref{ciexactexp}) contains $\psi_0$ with probability tending to 0.95 as $n\rightarrow\infty$.
\end{theorem}

One might simplify $Z_n^{2\#}$  by replacing the targeted versions by their initial estimators:
\begin{equation}\label{simplified}
Z_n^{2a,\#}=n^{1/2}(P_n^{\#}-P_n)D^*(Q_n^{\#},G_n^{\#})+n^{1/2}R_{2n}(Q_n^{\#},G_n^{\#},Q_n,G_n).\end{equation}
In this case $Z_n^{2a,\#}$ is the bootstrap sampling distribution of the exact second-order expansion 
\[
n^{1/2}(\psi_n^1-\Psi(Q_0))=n^{1/2}(P_n-P_0)D^*(Q_n,G_n)+R_{20}(Q_n,G_n,Q_0,G_0)\]
of the HAL-one-step estimator $\psi_n^1=\Psi(Q_n)+P_n D^*(Q_n,G_n)$.  The latter bootstrap sampling distribution can also  be used for the HAL-TMLE.


As above, let $\Phi_n^{a\#}(x)=P(Z_n^{2a,\#}\leq x\mid P_n)$  be the cumulative distribution of $Z_n^{2a,\#}$, conditional on $P_n$.
A corresponding bootstrap based 0.95-confidence interval for $\psi_0$ is given by \begin{equation}\label{ciexactexpa}
[\psi_n^1+q_{0.025,n}^{a\#}/n^{1/2},\psi_n^1+q_{0.975,n}^{a\#}/n^{1/2} ],\end{equation}
 where 
$q_{\alpha,n}^{a\#}=\Phi_n^{a\#-1}(\alpha)$. 
We have the analogue of the above theorem for the bootstrap distribution $Z_n^{2a,\#}$ of the one-step estimator, where we can remove the specific conditions needed for the TMLE
$Q_n^*$.
Since the proof is remarkably simple and demonstrates that $Z_n^{2,\#}$ and $Z_n^{2a,\#}$ provide very direct approximations of the sampling distributions of the HAL-TMLE and HAL-one-step estimator,  we show here its proof.

\begin{theorem}\label{thnpbootexactexpa}
Assume the conditions of Theorem \ref{thefftmle}; (\ref{boundb}); (\ref{dn1bounding}); and (\ref{contDstaremp}).

Then, $Z_n^{2a,\#}=n^{1/2}(P_n^{\#}-P_n)D^*(Q_n,G_n)+O_P(n^{-1/2-\alpha(d)})$, and thereby
\[
Z_n^{2a,\#}\Rightarrow_d N(0,\sigma^2_0)\mbox{ conditional on $(P_n:n\geq 1)$}.\]
In particular the above confidence interval (\ref{ciexactexpa}) contains $\psi_0$ with probability tending to 0.95 as $n\rightarrow\infty$.
\end{theorem}
{\bf Proof:}
%Let's do the proof for (\ref{simplified}) with $\psi_n^*$ replaced by the one-step estimator $\psi_n^1$.
Consider (\ref{simplified}).
By Theorem \ref{thnpbootmle} we have that $d_{n1}(Q_n^{\#},Q_n)$ and $d_{n2}(G_n^{\#},G_n)$ are $O_P(n^{-1/2-\alpha(d)})$.
Using the bound (\ref{boundingR2n}) implies now that $R_{2n}(Q_n^{\#},G_n^{\#},Q_n,G_n)=O_P(n^{-1/2-\alpha(d)})$. 
Regarding the leading term in $Z_n^{2a,\#}$ we write is as 
\[
n^{1/2}(P_n^{\#}-P_n)\{D^*(Q_n^{\#},G_n^{\#})-D^*(Q_n,G_n)\}+n^{1/2}(P_n^{\#}-P_n)D^*(Q_n,G_n).\]
In the proof of Theorem \ref{thnpboothaltmle} we showed that the first term is $O_P(n^{-1/2-\alpha(d)})$. This completes the proof of Theorem \ref{thnpbootexactexp}.
$\Box$


The above bootstrap distribution  $Z_n^{2,\#}$ is different from the  sampling distribution of $Z_n^{1,\#}=n^{1/2}(\Psi(Q_n^{\#*})-\Psi(Q_n^*))$ used in the previous subsection (and similarly, $Z_n^{2a,\#}$ is different from the bootstrap distribution of the standardized one-step estimator). The advantage of $Z_n^{1\#}$ is that it is an actual sampling distribution of our HAL-TMLE and thereby fully respects that our estimator is a substitution estimator. On the other hand, 
its asymptotic expansion as analyzed in the proof of Theorem \ref{thnpboothaltmle} and the remarkable direct and simple proof of Theorem \ref{thnpbootexactexp} suggests that the sampling distribution $Z_n^{1,\#}$  is more different from the desired sampling distribution 
of $n^{1/2}(\psi_n^*-\psi_0)$ than $Z_n^{2,\#}$. Therefore it will be of interest to compare both bootstrap methods through a simulation study.

As in our previous theorems, the above theorems also apply to the setting in which we replace $C^u$ by the  cross-validation selector $C_n$.

% ==================================================================
\section{The nonparametric bootstrap for a conservative finite sample bound of exact second-order expansion of HAL-TMLE or HAL-one-step-estimator}\label{sectupperb}

%Do here both direclty bootstrapping $d_{01}(Q_n^*,Q_0)$, $d_{02}(G_n,G_0)$ as well as doing it to their upper bound $-(P_n-P_0)L_1(Q_n,Q_0)$ and $-(P_n-P_0)L_2(G_n,G_0)$.
%Let's consider the case that $r_n$ is negligible and thereby treated as $0$.
We have the following finite sample upper bound for our HAL-TMLE relative to its target $\Psi(Q_0)$:
\begin{eqnarray*}
 n^{1/2}\mid \Psi(Q_n^*)-\Psi(Q_0)\mid&\leq & \mid  n^{1/2}(P_n-P_0)D^*(Q_n^*,G_n) \mid \\
 &&+
%\mid n^{1/2}(P_n-P_0)(D^*(Q_n^*,G_n)-D^*(Q_0,G_0))\mid\\
 f({\bf d}_{01}(Q_n^*,Q_0),{\bf d}_{02}(G_n,G_0)) +n^{1/2}r_n\\
 &\equiv&X_n(Q_n^*,G_n)+n^{1/2}r_n,
\end{eqnarray*}
where we defined a process $X_n(Q,G)$ (suppressing its dependence on $P_0$).
Similarly, we have this upper bound for the HAL one-step estimator $\psi_n^1=\Psi(Q_n)+P_n D^*(Q_n,G_n)$:
\[
n^{1/2}\mid \psi_n^1-\Psi(Q_0)\mid \leq  X_n(Q_n,G_n).\]
Let's focus on the latter, which could just as well be used for the sampling distribution of the HAL-TMLE as well.

{\bf How is this upper bound conservative?}
This upper bound is conservative from various points of view. Firstly, the true second-order remainder $R_{20}(Q_n,G_n,Q_0,G_0)$ could have both negative and positive values  that could cancel out a positive or negative value of $(P_n-P_0)D^*(Q_n,G_n)$. For example, in many models $R_{20}$ has a double robust structure
$\int (H_1(Q_n)-H_1(Q_0))(H_2(G_n)-H_2(G_0)) H_3(P_0,P_n) dP_0$.
In these double robust problems $Q_n$ and $G_n$ are based on different factors of the likelihood so that $H_1(Q_n)-H_1(Q_0))$ is generally almost uncorrelated with $H_2(G_n)-H_2(G_0))$, so that such a second order term could be reasonably symmetric  distributed around zero. The above upper bound does not allow any cancelation making it particularly conservative for double robust estimation problems. Secondly, the actual size  of $R_{20}(Q_n,G_n,Q_0,G_0)$ could be significantly smaller than our upper bound. For example, if we have the double robust structure, then the upper bound  bounds a term $\int (H_1(Q_n)-H_1(Q_0))(H_2(G_n)-H_2(G_0)) H_3(P_0,P_n)dP_0$ by Cauchy-Schwarz while bounding $H_3$ by its supremum norm. Since $Q_0$ and $G_0$ are very different functions, the Cauchy-Schwarz bound is very conservative itself, and, the supremum norm bound on $H_3$ will involve replacing a denominator by its smallest value. 
Therefore,  this bound is highly conservative for double robust estimation problems. 

If the second-order remainder has the form $\int (H_1(Q_n)-H_1(Q_0))^2 H_3(P_n,P_0)dP_0$, then this bound is more reasonable by  only being conservative due to the bounding of $H_3$ by its supremum norm and that we do not allow cancelation of  
 a mean zero centered $n^{1/2}(P_n-P_0)D^*(Q_n,G_n)$ with $R_{20}(P_n^*,P_0)$.
 Finally, the sampling distribution of this upper bound is not incorporating the known bounds for $n^{1/2}(\Psi(Q_n^*)-\Psi(Q_0))$ such as, for example, that $\Psi(P_0)$. The first nonparametric bootstrap method of the previous section is a sampling distribution of a substitution estimator thereby respects all the global bounds of the model and target parameter (e.g., $\Psi(P)$ is a probability). Respecting global constraints is particularly important when the target parameter is weakly supported by the data and asymptotics has not kicked in for the given sample size. 
 
 \ 
 \newline
We estimate the distribution of this upper bound with the nonparametric bootstrap. That is, we (conservatively) approximate the sampling distribution of 
$Z_n=\mid n^{1/2}(\Psi(Q_n^*)-\Psi(Q_0)\mid$ or $\mid n^{1/2}(\psi_n^1-\Psi(Q_0))\mid$ with
\[
Z_n^{3,\#}=\mid  n^{1/2}(P_n^{\#}-P_n)D^*(Q_n^{\#},G_n^{\#})\mid +
%\mid n^{1/2}(P_n-P_0)(D^*(Q_n^*,G_n)-D^*(Q_0,G_0))\mid\\
 f({\bf d}_{n1}(Q_n^{\#},Q_n),{\bf d}_{n2}(G_n^{\#},G_n)) \mid \]
 conditional on $(P_n:n\geq 1)$.
% Again, we could simplify this sampling distribution by replacing the targeted estimator $Q_n^{\#*}$ by $Q_n^{\#}$ and $Q_n^*$ by $Q_n$ in which case it corresponds with applying the above bounds to the sampling distribution of the one-step estimator $\psi_n^1$.
This distribution can now be used to construct an $0.95$-confidence interval. Let $F_n^{\#}(x)=P(Z_n^{3,\#}\leq x\mid (P_n:n\geq 1))$ and 
$q_{n,0.95}^{\#}=F_n^{\#  -1}(0.95)$ be its $0.95$-quantile. Then, $\Psi(Q_n^*)\pm q_{n,0.95}^{\#}/n^{1/2}$ is the resulting $0.95$-confidence interval.
 
% One could also apply this method to $n^{1/2}\mid \Psi(Q_n^*)-\Psi(Q_0)\mid/\sigma_n$, where $\sigma_n^2$ is an estimator of the variance of $D^*(Q_0,G_0)$, by just dividing the above upper bound by $\sigma_n$.  In that case, $Z_n^{\#}$ also involves $\sigma_n^{\#}$. It is not clear if this has any advantage, beyond that the confidence interval is now of the form $\Psi(Q_n^*)\pm q_{n,0.95}^{\#}\sigma_n/n^{1/2}$ imitating the Wald-type confidence interval.
{\bf Alternative reasonable upper-bound:}
 It appears to also be reasonable to use as upper-bound of $X_{n1}(Q_n,G_n)\equiv \mid  n^{1/2}(P_n-P_0)D^*(Q_n^*,G_n)  +
%\mid n^{1/2}(P_n-P_0)(D^*(Q_n^*,G_n)-D^*(Q_0,G_0))\mid\\
 f(d_{01}(Q_n^*,Q_0),d_{02}(G_n,G_0))\mid $. Note that  $X_{n1}(Q_n,G_n)$ is different from $X_n(Q_n,G_n)$, by putting the absolute value outside the sum of the two terms. This is not a deterministic upper bound in the sense that $\mid n^{1/2}(\psi_n^1-\Psi(Q_0))\mid $ is smaller than this bound with probability 1, but we certainly expect this to be a conservative distribution since we are adding a positive bias to a mean zero centered symmetric empirical process at $D^*(Q_n,G_n)$.


In spite of the conservative nature of our upper bound it is still asymptotically sharp.
Again,  not surprisingly, asymptotic consistency of the above conservative sampling distribution  is an immediately corollary of our analysis of the nonparametric bootstrap for the HAL-TMLE. 
\begin{theorem}\label{thupperbound}
Under the same conditions as Theorem \ref{thnpboothaltmle}, $Z_n^{3,\#}=n^{1/2}(P_n^{\#}-P_n)D^*(Q_n,G_n)+O_P(n^{-1/2-\alpha(d)})$, and thereby
\[
Z_n^{3,\#}\Rightarrow_d N(0,\sigma^2_0)\mbox{ conditional on $(P_n:n\geq 1)$}.\]
In particular the above confidence interval (\ref{ciexactexp}) contains $\psi_0$ with probability tending to 0.95 as $n\rightarrow\infty$.
%  In particular, $q_{n,0.95}^{\#}$ converges to $\sigma_0 1.96$. 
 \end{theorem}
 
\paragraph{More conservative asymptotically sharp sampling distribution and corresponding bootstrap method:}
In the Appendix \ref{sectsupupperb} we propose an even more conservative sampling distribution for $n^{1/2}(\psi_n^1-\psi_0)$ (or $n^{1/2}(\psi_n^*-\psi_0)$) by replacing $X_n(Q_n,G_n)$ by   the supremum of $X_n(Q,G)$ over all $(Q,G)$ in the parameter space for which $d_{01}(Q,Q_0)$ and $d_{02}(G,G_0)$ are smaller than specified constants $x_{1n} $ and $x_{2n}$ chosen so that the probability that $d_{01}(Q_n,Q_0)$ and $d_{02}(G_n,G_0)$ are smaller than these constants are known to be larger than $1-\bar{\alpha}_{n}$ for some small number $\bar{\alpha}_n\rightarrow 0$. We propose a concrete method that expresses $(x_{1n},x_{2n})$  in terms of  a quantile of the supremum norm of a standard empirical cumulative survival function process $n^{1/2}(\bar{P}_n-\bar{P}_0)$. Bootstrapping this latter process provides now an estimator $(x_{1n}^{\#},x_{2n}^{\#})$ of $(x_{1n},x_{2n})$. The distribution of the corresponding supremum of $X_n(Q,G)$  is then estimated with the nonparametric bootstrap as well. The same method could be applied to $X_{n1}(Q,G)$.
Since this supremum might be cumbersome to compute in practice, in Appendix \ref{sectsupupperb} we proceed with proposing a simplified conservative approximation of this supremum in which the second-order remainder is separately maximized by plugging in the values $(x_{1n},x_{2n})$, resulting in an easy to compute sampling distribution. Again, we show that both of these methods are still asymptotically sharp.  
% ==================================================================

 {\bf Finite sample conservative confidence interval:}
 Let's first consider the exact finite sample conservative confidence interval presented in (\ref{consbound1}).
 For this we need bounds $M_3$, $M_{12}$ and $M_2$ on the sectional variation norm of $D^*(Q,G)$, $L_{12}(\bar{Q})$ and $L_2(G)$, respectively.
 These can be expressed in terms of the sectional variation norm bounds $(C_{12}^u,C_2^u)$ on $(\bar{Q}, G)$ and the lower bound $\delta$ of $\min_a g(a\mid W)$ and $\bar{Q}$.
 Here one can use that the sectional variation norm of $1/g(a\mid W)$ can be bounded in terms of $\delta$ and $\pl w\rightarrow g(a\mid w)\pl_v^*$. 
 (\ref{consbound1}) tells us that $\mid n^{1/2}(\psi_n^1-\Psi(Q_0))\mid $ is dominated by the distribution of 
 $Z_n^+=(M_3+f(M_{12}^{1/2},M_2^{1/2}))\pl n^{1/2}(\bar{P}_n-\bar{P}_0)\pl_{\infty}$, where
$f$ is defined by (\ref{r2upperboundexample1}), and 
$\bar{P}(u)=P([u,\tau])=\int_{[u,\tau]} dP(s)$ is the probability that $O\in [u,\tau]$ under $P$. Estimation of the sampling distribution of
$n^{1/2}(\bar{P}_n-\bar{P}_0)$ with $n^{1/2}(\bar{P}_n^{\#}-\bar{P}_n)$ results then in the estimate $Z_n^{+,\#}$ of $Z_n^+$ and corresponding finite sample conservative $0.95$-confidence interval.
(Similarly, we have this bound for the TMLE $\Psi(Q_n^*)$ with $M_3$  and $M_{12}$ replaced by $M_3^*$ and $M_{12}^*$, respectively.)
 However, as we argued in general, this conservative confidence interval will generally be of little practical use by being much too conservative, although these confidence intervals will still have a width or order $n^{-1/2}$. 
% ==================================================================

{\bf Consistency of nonparametric bootstrap for exact expansion of HAL-TMLE/HAL-one-step:}
Recall the exact second-order remainder of $\Psi(Q_n^*)-\Psi(Q_0)$ defined by $R_{20}(Q_n^*,G_n,Q_0,G_0)=(R_{20}^1-R_{20}^0)(Q_n^*,G_n,Q_0,G_0)$.
Let $R_{2n}(Q_n^{\#*},G_n^{\#},Q_n^*,G_n)$ be the nonparametric bootstrap analogue.
Thus,
\[
R_{2n}^a(Q_n^{\#*},G_n^{\#},Q_n^*,G_n)=\int \frac{(g_n^{\#}-g_n)(a\mid w)}{g_n^{\#}(a\mid w)}(\bar{Q}_n^{\#*}-\bar{Q}_n^*)(a,w) dP_n(w).\] 
Let 
\[
Z_n^{2,\#}=n^{1/2}(P_n^{\#}-P_n)D^*(Q_n^{\#*},G_n^{\#})+n^{1/2}R_{2n}(Q_n^{\#*},G_n^{\#},Q_n^*,G_n).\]

Consider also the conservative version
\[
Z_n^{3,\#}=\mid n^{1/2}(P_n^{\#}-P_n)D^*(Q_n^{\#*},G_n^{\#})\mid + f(d_{n12}(\bar{Q}_n^{\#*},\bar{Q}_n^*),d_{n2}(G_n^{\#},G_n)) \mid .\]
 where the upper bound $f()$ for the remainder is defined in  (\ref{r2upperboundexample1}).
 Application of Theorems \ref{thnpbootexactexp} and \ref{thupperbound} prove the asymptotic consistency of these two nonparametric bootstrap distributions.
 
 \begin{theorem}
 We have $Z_n^{2,\#}\Rightarrow_d N(0,\sigma^2_0)$ and $Z_n^{3,\#}\Rightarrow_d \mid N(0,\sigma^2_0)\mid$, conditional on $(P_n:n\geq 1)$.
 As a consequence, an $0.95$-confidence interval for $\psi_0$ based on $Z_n^{2,\#}$ and $Z_n^{3,\#}$ have asymptotic coverage 0.95 of $\psi_0$.
 This also applies to the setting in which $C^u$ is replaced by the cross-validation selector $C_n$.
 \end{theorem}
 Finally, we remark that our HAL-MLE is really indexed by the  model bounds $(C_{12}^u,C_2^u,\delta)$ and these might all three be unknown to the user. So in that case, we recommend to select
 all three with the cross-validation selector $(C_{12n},C_{2n},\delta_)$ and define the HAL-TMLE and bootstrap of the HAL-TMLE at this fixed  choice $(C_n,\delta_n,M_n)$.

 
   
%   do the very conserative finie sampe bound ujsing IP as shown in section 2!! first and state confidene inteval
  

% define nonpaarmetric bootstrap of TMLE
 %check conditions on hte loss functions we needed, differentiability second-order andthe P_n R_2 bounding as stated.
  %Then staet the np bootstrap results for $Q_n,G_n$ itself.

%State asymptotic consistency of bootstrap result. say why so important since DR structrue of R_2 is preserved isntead of upper bounding

%define np bootstrap of upper bound method and CI. just do bootstrap of L^2(P_0) norms, not d_{01}. easier and sharper.
%proof is all same sincew we can use the upper bound in terms of d_0 for that implies result for L2norms remainder

%define np bootstrap of supremum method. Define process X_n(Q,G).
%validity immediately applies sicne our theorems are all about empirical process, othign to do with particular target parameter.

% ======================================================
{\bf Finite sample conservative confidence interval:}
Let's first consider the exact finite sample conservative confidence interval presented in (\ref{consbound1}).
 For this we need bounds $M_3$, $M_{1}$ on the sectional variation norm of $D^*(P)=2p-\Psi(p)$ and $L(p)=-2p+\Psi(p)$, respectively. These bounds will thus be identical: $M_3=M_1$. We have that $M_1=\sup_{p\in {\cal M}} \pl L(p)\pl_v^*=2 C^u$.
 %One would now have to establish a bound on \pl p_{\epsilon}\pl_v^*$ in terms of $\pl p\pl_v^*$.
%Let's for now denote this bound with $M_1^*$.
 (\ref{consbound1}) tells us that $\mid n^{1/2}(\psi_n^1-\Psi(P_0))\mid $ is dominated by the distribution of 
 $Z_n^+=4C^u\pl n^{1/2}(\bar{P}_n-\bar{P}_0)\pl_{\infty}$, where 
$\bar{P}(u)=P([u,\tau])=\int_{[u,\tau]} dP(s)$ is the probability that $O\in [u,\tau]$ under $P$. Estimation of the sampling distribution of 
$n^{1/2}(\bar{P}_n-\bar{P}_0)$ with the bootstrap distribution $n^{1/2}(\bar{P}_n^{\#}-\bar{P}_n)$ results then in $Z_n^{+,\#}$ and  corresponding finite sample conservative $0.95$-confidence interval, which can also be used for $\Psi(P_n^*)$.
 In the previous example, this confidence interval appeared to be much too conservative to be practically useful, but in this example, since our bound on $R_{20}(P,P_0)$ is sharp and the sectional variation norm bounds $M_1=M_3=2C^u$ are easily determined in terms of the sectional variation norm bound $C^u$ of the model, this appears to be an interesting finite sample conservative confidence interval. We propose to apply this confidence interval to $C^u=C_n$ and the corresponding bounds $M_{1n}=M_{3n}=2C_n$.
 
% Regarding determining $M_1^*$ note that for an infinitesimal $d\epsilon>0$$p_{d\epsilon}=p(1+d\epsilon(2p-\Psi(p)))=p+ d\epsilon (2p^2-p\Psi(p)) Say $O$ is univariate. \int \mid p_{d\epsilon}(dx)\mid\leq \int \mid p(dx)\mid+ d\epsilon \int 4 \mid p(dx)\mid+\Psi(p)
 
  %However, as we argued in general, this results in much too conservative confidence intervals for practical use, although they will still have a width or order $n^{-1/2}$. 

% ======================================================
 
{\bf Asymptotic consistency of the bootstrap for the exact second-order expansion of HAL-TMLE:}
We have $n^{1/2}(\Psi(P_n^*)-\Psi(P_0))=n^{1/2}(P_n-P_0)D^*(P_n^*)-n^{1/2}\int (p_n^*-p_0)^2 d\mu$.
Let  $Z_n^{2,\#}$ be the nonparametric bootstrap estimator of this exact second-order expansion:
\[
Z_n^{2,\#}=n^{1/2}(P_n^{\#}-P_n)D^*(P_n^{\#*})-n^{1/2}\int (p_n^{\#*}-p_n^*)^2 d\mu.\]
In addition, consider the upper bound:
\[
\mid n^{1/2}(\Psi(P_n^*)-\Psi(P_0))\mid\leq \mid n^{1/2}(P_n-P_0)D^*(P_n^*)\mid +\int (p_n^*-p_0)^2 d\mu .\]
Let $Z_n^{3,\#}$ be the nonparametric bootstrap estimator of this conservative sampling distribution:
\[
Z_n^{3,\#}\equiv \mid n^{1/2}(P_n^{\#}-P_n)D^*(P_n^{\#*})\mid +n^{1/2}\int (p_n^{\#*}-p_n^*)^2 d\mu .\]
Application of Theorems \ref{thnpbootexactexp} and \ref{thupperbound} prove the asymptotic consistency of these two nonparametric bootstrap distributions.

\begin{theorem}
We have that conditional on $(P_n:n\geq 1)$, $Z_n^{j,\#}\Rightarrow_d N(0,\sigma^2_0)$ as $n\rightarrow\infty$, $j=2,3$. 
 As a consequence, an $0.95$-confidence interval for $\psi_0$ based on $Z_n^{2,\#}$ and $Z_n^{3,\#}$ have asymptotic coverage 0.95 of $\psi_0$.
 This theorem can also be applied to setting in which $C^u=C_n$.
 \end{theorem}
 
 Finally, we remark that our HAL-MLE is really indexed by the hypothesized model bounds $(C^u,\delta,M)$ and these might all three be unknown to the user. So in that case, we recommend to select
 all three with the cross-validation selector $(C_n,\delta_n,M_n)$ and define the HAL TMLE and bootstrap of the HAL-TMLE at this fixed choice $(C_n,\delta_n,M_n)$.

%I am tempted to only do the NP bootsrtap and NP boostrap of upper bound, bu tnot supremum for both examples.
%D*, R2, R2 bound L2 norms.
%loglik loss for f.
%how to define family of densities with sectional varioatnnorm bounded how to do HALMLE.
%HAL MLE results.
%universasl lfm. verify condition for preserved for this immpliciti model! eps-n-eps_0n =n^{-1/2} and eps_{0n}=O(d^{05}(Q_n,Q_0))
%then state efficiency of TMLE.

%state bootstrap. verify conditions on loss for bootstrap second-order expansion etc.
%state result.

%do bootsrap of upper bound R2, just L2 norms!, pretty close to bootsraP TMLE IN THIS CASE.
%do supnorm, state X_N(Q) state method, state result.

%
% ======================================================
\section{Nonparametric bootstrap to estimate a supremum norm of the upper-bound of exact second order expansion of HAL-one-step estimator}\label{sectsupupperb}
 

%Define the process $(X_{I,n}(Q,G):(Q,G)\in {\cal F})$ where ${\cal F}={\cal F}_1\times {\cal F}_2)\[X_{I,n}(Q,G)\equiv n^{1/2}(P_n-P_0)D^*(Q_{\epsilon_n},G) +
%\mid n^{1/2}(P_n-P_0)(D^*(Q_n^*,G_n)-D^*(Q_0,G_0))\mid\\ f(d_{01}(Q_{\epsilon_n},Q_0),d_{02}(G,G_0)). \] A user  might decide to use the slightly simpler stochastic process as a good approximation: \[ X_{I,n,a}(Q,G)=n^{1/2}(P_n-P_0)D^*(Q,G) +
%\mid n^{1/2}(P_n-P_0)(D^*(Q_n^*,G_n)-D^*(Q_0,G_0))\mid\\ f(d_{01}(Q,Q_0),d_{02}(G,G_0)).\] The following lemma is trivially true. \begin{lemma}$ X_{I,n}$ is weakly convergence in $\ell^{\infty}({\cal F})$.The nonparametric bootstrap is consistent for $X_{I,n}$.\end{lemma}

%We can use directly empirical process bound for $d_{01}(Q_n^*,Q_0)$, see lemma preserve we now have. No need to replace $Q_n^*$ by $Q_n$.So we can then get rid of $\sim \leq$ and get true inequalities. we can replace $\epsilon_{0n}$ by $\epsilon_n$ giving the $1/n$ error. So that is perfect.This will be much cleaner.

 
 By Lemma \ref{lemma2} for the HAL-MLEs we have ${\bf d}_{01}(Q_n,Q_0)\leq -(P_n-P_0){\bf L}_1(Q_n,Q_0)$ and ${\bf d}_{02}(G_n,G_0)\leq -(P_n-P_0){\bf L}_2(G_n,G_0)$.
 % Since $d_{01}(Q_n^*,Q_0)$ behaves at least as well as  $d_{01}(Q_n,Q_0)$ and is of the same order, we suggest using the same bound for $d_{01}(Q_n^*,Q_0)$. By the same argument, replacing $(P_n-P_0)D^*(Q_n^*,G_n)$ by $(P_n-P_0)D^*(Q_n,G_n)$ should also not be a problem for preserving the conservative nature of our bound. 
  Applying these two upper bounds for ${\bf d}_{01}(Q_n,Q_0)$ and ${\bf d}_{02}(G_n,G_0)$ to our upper bound for the exact second-order remainder 
  in the expansion $\psi_n^1-\psi_0=(P_n-P_0)D^*(Q_n,G_n)+R_{20}(Q_n,G_n,Q_0,G_0)$ yields the following conservative bound for the HAL-one-step estimator $\psi_n^1=\Psi(Q_n)+P_n D^*(Q_n,G_n)$:
\begin{eqnarray*}
 n^{1/2}\mid \psi_n^1-\Psi(Q_0)\mid& \leq & \mid  n^{1/2}(P_n-P_0)D^*(Q_n^*,G_n) \mid \\
 &&\hspace*{-5cm}
 +
%\mid n^{1/2}(P_n-P_0)(D^*(Q_n^*,G_n)-D^*(Q_0,G_0))\mid\\
 f(\sqrt{\mid n^{1/2}(P_n-P_0){\bf L}_1(Q_n,Q_0)\mid},\sqrt{ \mid n^{1/2}(P_n-P_0){\bf L}_2(G_n,G_0)\mid})\mid .
\end{eqnarray*}
Suppose that $\sup_{P,P_1\in {\cal M}}P \{{\bf L}_1(Q(P_1))-{\bf L}_1(Q(P))\}\leq c_1\in \openr^{K_1}_{\geq 0}$ and $\sup_{P,P_1\in {\cal M}}P\{{\bf L}_2(G(P_1))-{\bf L}_2(G(P))\}<c_2\in \openr^{K_2}_{\geq 0}$, then we also know that $R_2(Q_n^*,G_n,Q_0,G_0)\leq f(c)$, where $c=(c_1,c_2)$. Therefore, we assume that $f$ is chosen so that these global bounds on the loss-based dissimilarities ${\bf d}_{01}$ and ${\bf d}_{02}$ are respected even when $f$ is applied to an $x\in\openr^{K}_{\geq 0}$ with $x\geq c$ that is outside these bounds: i.e., 
$f(x)=f(\min(x,c))$.


%We use the notation $\sim\leq$ instead of $\leq$ since it is formally known to hold up till the 2 substitutions of $Q_n$ for $Q_n^*$ mentioned above.
%We could simplify this upper bound by replacing $Q_n^*$ by $Q_n$ in which case it corresponds with an upper bound for the centered one-step estimator $n^{1/2}(\psi_n^1-\psi_0)$.
Define the following process $X_n=(X_n(Q,G): (Q,G)\in {\cal F})$:
\begin{eqnarray*}
X_n(Q,G)&=&\mid  n^{1/2}(P_n-P_0)D^*(Q,G) \mid \\
&&+
%\mid n^{1/2}(P_n-P_0)(D^*(Q_n^*,G_n)-D^*(Q_0,G_0))\mid\\
 f(\sqrt{\mid n^{1/2}(P_n-P_0){\bf L}_1(Q,Q_0)\mid},\sqrt{ \mid n^{1/2}(P_n-P_0){\bf L}_2(G,G_0)\mid})\mid .\end{eqnarray*}
{\bf Finite sample bound:}
 Thus, we can state that \[
 \mid n^{1/2}(\psi_n^1-\psi_0)\mid \leq \mid X_n(Q_n,G_n)\mid .\]
 %+O_P(n^{-1/2})+n^{1/2}\mid P_n D^*(Q_n,G_n)\mid.\]
 %Let $\tilde{r}_n=O_P(n^{-1/2})+r_n$, and let's assume that $\tilde{r}_n$ is negligible relative to $X_n(Q_n^*,G_n)$ so that we can ignore this term.
 It remains to upper bound $X_n(Q_n,G_n)$.\nl
{\bf Proposed method of inference:}
 This finite sample bound in terms of a stochastic process evaluated at our HAL-MLEs suggests the following method for inference:
 \begin{itemize}
 \item For user supplied $\alpha_n=(\alpha_{1n},\alpha_{2n})$, determine an $x_n=(x_{1n},x_{2n})$  so that $P(d_{01}(Q_n,Q_0)>x_{1n})\leq \alpha_{1n}$ and $P(d_{02}(G_n,G_0)>x_{2n})\leq \alpha_{2n}$. For example, $x_n$ could be defined so that  $\mid (P_n-P_0)L_1(Q_n,Q_0)\mid >x_{1n}$ with probability $\alpha_{1n}$ and 
 $\mid (P_n-P_0)L_2(G_n,G_0)\mid >x_{2n}$ with probability $\alpha_{2n}$.
  \item Define
 \[ {\cal F}(x_n)=\{(Q,G)\in {\cal F}: d_{01}(Q,Q_0)<x_{1n},d_{02}(G,G_0)<x_{2n}\},\]
 and note that $P((Q_n,G_n)\in {\cal F}(x_n))\geq 1-\bar{\alpha}_n$, where $\bar{\alpha}_n\equiv \alpha_{1n}+\alpha_{2n}$.
 \item We have 
 \[
P(\mid X_n(Q_n,G_n)\mid > x)\leq  P(\pl X_n\pl_{{\cal F}(x_n)}>x)+\bar{\alpha}_n ,\]
where $\pl X\pl_{{\cal F}}=\sup_{f\in {\cal F}}\mid X(f)\mid$.
Let 
\[
F_{n,x_1}(x)=P(\pl  X_n \pl_{{\cal F}(x_1)} \leq x),\]
and
\[
q_{n,0.95}=F_{n,x_n}^{-1}(0.95+\bar{\alpha}_n) .\]
We have  $\psi_n^1\pm q_{n,0.95}/n^{1/2}$ contains $\psi_0$ with probability at least $0.95$.
\item Let $X_n^{\#}$ be the nonparametric bootstrap estimate of $X_n$:
\begin{eqnarray*}
X_n^{\#}(Q,G)&=&\mid  n^{1/2}(P_n^{\#}-P_n)D^*(Q,G) \mid \\
&&\hspace*{-2cm} +
%\mid n^{1/2}(P_n-P_0)(D^*(Q_n^*,G_n)-D^*(Q_0,G_0))\mid\\
 f(\sqrt{\mid n^{1/2}(P_n^{\#}-P_n){\bf L}_1(Q,Q_n)\mid}, \sqrt{\mid n^{1/2}(P_n^{\#}-P_n){\bf L}_2(G,G_n)\mid}) .\end{eqnarray*}
 \item Let $x_n^{\#}$ be an estimator of $x_n$ using the nonparametric bootstrap. A highly conservative method is presented below. Alternatively, one could determine $x_n^{\#}$ based on the  conservative sampling distributions $n^{1/2}(P_n^{\#}-P_n)L_1(Q_n^{\#},Q_n)$ for $d_{01}(Q_n,Q_0)$ and $n^{1/2}(P_n^{\#}-P_n)L_2(G_n^{\#},G_n)$ for $d_{02}(G_n,G_0)$. 
%\item We use $\pl  X_n^{\#}\pl_{{\cal F}(x_n)}$ as a conservative sampling distribution estimator of the sampling distribution of $\mid n^{1/2}(\psi_n^*-\psi_0)\mid$.
\item Let  \[ {\cal F}_n(x_n^{\#})=\{(Q,G)\in {\cal F}: d_{n1}(Q,Q_n)<x_{1n}^{\#},d_{n2}(G,G_n)<x_{2n}^{\#}\}\] be the nonparametric bootstrap version of ${\cal F}(x_n)$.
Let 
\[
F_{n,x_1}^{\#}(x)=P(\pl  X_n^{\#} \pl_{{\cal F}_n(x_1)} \leq x\mid (P_n:n\geq 1)).\]
Let 
\[
q_{n,0.95}^{\#}=F_{n,x_n^{\#}}^{\#-1}(0.95+\bar{\alpha}_n) .\]
\item The proposed 0.95-confidence interval is given by:
\[
\psi_n^1\pm q_{n,0.95}^{\#}/n^{1/2} .\]
\end{itemize}
{\bf Method for determining cut-offs $x_n$ for loss-based dissimilarities of HAL-MLEs:}
In order to implement the above confidence interval we  need to derive a method for determining $x_n$ and its bootstrap version $x_n^{\#}$.
We will now present a conservative definition of $x_n$ and its bootstrap estimate $x_n^{\#}$.
By our integration by parts lemma, we have
\begin{eqnarray*}
d_{01}(Q_n,Q_0)&\leq & \pl \bar{P}_n-\bar{P}_0\pl_{\infty}\pl L_1(Q_n,Q_0)\pl_v^*  \\
&\leq & 2M_1\pl \bar{P}_n-\bar{P}_0\pl_{\infty},\\
d_{02}(G_n,G_0)&\leq &\pl \bar{P}_n-\bar{P}_0\pl_{\infty}\pl L_2(G_n,G_0)\pl_v^* \\
&\leq& 2M_2\pl \bar{P}_n-\bar{P}_0\pl_{\infty}.
\end{eqnarray*}
Let  $T_{n}(x)\equiv P(\pl n^{1/2}(\bar{P}_n-\bar{P}_0)\pl_{\infty}>x)$ so that
\[
P(d_{01}(Q_n,Q_0)>x)\leq T_n( 1/2 n^{1/2}M_1^{-1} x).\]
Given $\alpha_{1n},\alpha_{2n}$ we can select $x_{1n}=2M_1n^{-1/2}T_n^{-1}(\alpha_{1n})$ and $x_{2n}=2M_2n^{-1/2}T_n^{-1}(\alpha_{2n})$.
Then, we have that $P(d_{01}(Q_n,Q_0)>x_{1n})\leq \alpha_{1n}$ and $P(d_{02}(G_n,G_0)>x_{2n})\leq \alpha_{2n}$.
We also know from empirical process theory that the supremum norm of $n^{1/2}(\bar{P}_n-\bar{P}_0)$ has an exponential tail $\exp(-C x)$ so that
$T_n^{-1}(\alpha_{1n})$ behaves as $\log \alpha_{1n}^{-1}$, and the same applies to $T_n^{-1}(\alpha_{2n})$. This shows that one can select $\alpha_{1n}$ and $\alpha_{2n}$ as numbers that converge to zero at a polynomial rate (e.g. $\alpha_{1n}=n^{-1}$), while still preserving that $\max(x_{1n},x_{2n})\rightarrow 0$ at rate $\log n/n^{1/2}$. 
Since $n^{1/2}(\bar{P}_n-\bar{P}_0)$ is an empirical process indexed by a class of indicators, we can consistently and robustly estimate the distribution of $\pl n^{1/2}(\bar{P}_n-\bar{P}_0)\pl_{\infty}$  with the nonparametric bootstrap \citep{vanderVaart&Wellner96}, which, for completeness,  is  stated in the following lemma.
\begin{lemma}
We have that (uniformly in $x$) $T_{n}(x)\rightarrow T_0(x)$, where $T_0(x)=P(\pl \bar{X}_0\pl_{\infty}>x)$, and 
$\bar{X}_0$ is the limit Gaussian process of $\bar{X}_n=n^{1/2}(\bar{P}_n-\bar{P}_0)$.
We have
\begin{eqnarray*}
P(n^{1/2}d_{01}(Q_n,Q_0)>x)&\leq& T_{n}(1/2n^{1/2}x/M_1)\\
P(n^{1/2}d_{02}(G_n,G_0)>x)&\leq & T_{n}(1/2n^{1/2}x/M_2).
\end{eqnarray*}
Let $T_n^{\#}(x)=P(\pl n^{1/2}(\bar{P}_n^{\#}-\bar{P}_n)\pl_{\infty}>x\mid (P_n:n\geq 1))$. Then, uniformly in $x$,
$T_n^{\#}(x)\rightarrow T_0(x)$ as $n\rightarrow\infty$.
\end{lemma}
We estimate $x_n$ with its nonparametric bootstrap analogue: 
\begin{eqnarray*}
x_{1n}^{\#}&=&2M_1 n^{-1/2}T_n^{\#-1}(\alpha_{1n})\\
x_{2n}^{\#}&=&2M_2n^{-1/2}T_n^{\#-1}(\alpha_{2n}).
\end{eqnarray*}
%Now optimize w.r.t. choice $x_n$
%Let $T_n^{\#}$ be the estimator of the survivor function $T_{0,n}$ of $\pl n^{1/2}(\bar{P}_n-\bar{P}_0)\pl_{\infty}$ based on the nonparametric bootstrap. 


We note that our nonparametric bootstrap estimator of the sampling distribution of $X_n$ and $x_n$ only relies on how well the nonparametric bootstrapped empirical process indexed by Donsker class (functions with uniformly bounded sectional variation norm) and class of indicators approximates the sampling distribution of the empirical process. Therefore, the asymptotic consistency of this nonparametric bootstrap method  follows straightforwardly from the asymptotic consistency of the nonparametric bootstrap for these empirical processes. This is presented in the following theorem. 

 \begin{theorem}
 Consider definitions $X_n$,
 $x_{1n}=2M_1n^{-1/2}T_n^{-1}(\alpha_{1n})$ and $x_{2n}=2M_2n^{-1/2}T_n^{-1}(\alpha_{2n})$. 
 Let $\alpha_n$ converge to zero at a rate $n^{-p}$ for some finite $p$. Then, $x_n$ converges to zero at rate $\log n/n^{1/2}$.
 
{\bf Finite sample oracle confidence interval:} We have
 \[
 \mid n^{1/2}(\psi_n^1-\psi_0)\mid \leq \mid X_n(Q_n,G_n)\mid,\]
 and
 \[
P(\mid X_n(Q_n,G_n)\mid > x)\leq  P(\pl X_n\pl_{{\cal F}(x_n)}>x)+\bar{\alpha}_n .\]
Let 
\[
F_{n,x_1}(x)=P(\pl  X_n \pl_{{\cal F}(x_1)} \leq x),\]
and
\[
q_{n,0.95}=F_{n,x_n}^{-1}(0.95+\bar{\alpha}_n) .\]
Then,  $\psi_n^1\pm q_{n,0.95}/n^{1/2}$ contains $\psi_0$ with probability at least $0.95$. 

{\bf Weak convergence of process $X_n$:}
  Let $Z_n$ be the empirical process $n^{1/2}(P_n-P_0)$ indexed by the class of functions 
 \begin{equation}\label{calf1}
 {\cal F}_1\equiv \{D^*(Q,G),L_1(Q,Q_0),L_2(G,G_0): (Q,G)\in {\cal F}\}.
 \end{equation}
  $X_n$ is a continuous function of $Z_n$:
\[
X_n(Q,G)=g(Z_n)\equiv \mid Z_n(D^*(Q,G))\mid +f(\mid Z_n(L_1(Q,Q_0))\mid,\mid Z_n(L_2(G,G_0))\mid) .\]
We know that $Z_n\Rightarrow_d Z_0$ for a Gaussian process in $\ell^{\infty}({\cal F}_1)$.
The continuous mapping theorem shows that $X_n\Rightarrow_d X_0=g(Z_0)$ , where 
$X_0$ is a simple function of $Z_0$ defined by
\[
X_0(Q,G)= \mid Z_0(D^*(Q,G))\mid +f( \mid Z_0(L_1(Q,Q_0))\mid, \mid Z_0(L_2(G,G_0))\mid) .\] 
Therefore, $\pl X_n\pl_{{\cal F}(x)}\Rightarrow \pl X_0\pl_{{\cal F}(x)}$, uniformly in $x$.
In particular, uniformly in $x$
\[
P(\pl X_n\pl_{{\cal F}(x_n)}>x)\rightarrow P(N(0,\sigma^2_0)>x).\]


{\bf Weak convergence of nonparametric bootstrap process $X_n^{\#}$:}
Let $X_n^{\#}$, $x_n^{\#}$, ${\cal F}_n(x_n^{\#})$ be the nonparametric bootstrap version of $X_n$, $x_n$ and ${\cal F}(x_n)$ defined above.
 We have that uniformly in $x$,  conditional on $(P_n:n\geq 1)$, $\pl X_n^{\#}\pl_{{\cal F}(x)}\Rightarrow_d \pl X_0\pl_{{\cal F}(x)}$.
 In particular,
 \[
 P(\pl X_n^{\#}\pl_{{\cal F}(x_n^{\#})}>x\mid (P_n:n\geq 1))+\bar{\alpha}_n\rightarrow P(\mid N(0,\sigma^2_0)\mid >x).\]
 
 {\bf Nonparametric bootstrap estimate of finite sample confidence interval and its asymptotic consistency:}
 Let 
\[
F_{n,x_1}^{\#}(x)=P(\pl  X_n^{\#} \pl_{{\cal F}_n(x_1)} \leq x\mid (P_n:n\geq 1)).\,\]
and
\[
q_{n,0.95}^{\#}=F_{n,x_n^{\#}}^{\#-1}(0.95+\bar{\alpha}_n) .\]

 Then,  $q_{0.95,n}^{\#}(x_n)\rightarrow 1.96$ so that the confidence interval $\psi_n^*\pm q_{0.95,n}^{\#}/n^{1/2}$ is an asymptotic $0.95$-confidence interval.
 \end{theorem}
 
 The width of this proposed confidence interval is a function of the user supplied $\alpha_n=(\alpha_{1n},\alpha_{2n})$. To remove this choice from consideration, one might determine the $\alpha_n$ that minimizes $q_{n,0.95}^{\#}=F_{n,x_n^{\#}}^{\#-1}(0.95+\bar{\alpha}_n) $, where we note that $x_n^{\#}$ depends on $(\alpha_{1n},\alpha_{2n})$. 
 
 
 \subsection{Simplified conservative version}
 The implementation of the computation of the supremum over $(Q,G)$ of $X_n(Q,G)$ can be computationally challenging.
 Therefore, here we pursue an easy to compute and robust conservative version of this approach. Consider a sequence of cut-offs  $x_n=(x_{1n},x_{2n})$ for which  $P(d_{01}(Q_n,Q_0)\leq x_{1n}, d_{02}(G_n,G_0)\leq x_{2n})\geq 1-\bar{\alpha}_{n}$, where $\bar{\alpha}_n\rightarrow 0$.
 Here one could conservatively replace $d_{01}(Q_n,Q_0)$ and $d_{02}(G_n,G_0$ by their empirical process bounds
 $\mid (P_n-P_0)L_1(Q_n,Q_0)\mid $ and $\mid (P_n-P_0)L_2(G_n,G_0)\mid$, respectively.
 
  The basic idea is to replace the second-order remainder
 by the upper bound $n^{1/2}(f(x_n^{1/2})$ (which holds with probability at least $1-\bar{\alpha}_n$), while keeping the leading term $\mid n^{1/2}(P_n-P_0)D^*(Q_n,G_n)\mid$ for what it is. We think the latter makes sense since we suspect that the supremum of $\mid n^{1/2}(P_n-P_0)D^*(Q,G)\mid $ over all $(Q,G)\in {\cal F}_{x_n}$ will be close to its evaluation at $Q_n,G_n$.
 
 Let $I_n$ be the indicator that $(Q_n,G_n)\in {\cal F}_{x_n}$ so that $P(I_n=1)\geq 1-\bar{\alpha}_n$, and let $\tilde{Z}_n\equiv \mid n^{1/2}(P_n-P_0)D^*(Q_n,G_n)\mid$.
 %Then, \[ P( X_n(Q_n,G_n)\leq \mid n^{1/2}(P_n-P_0)D^*(Q_n,G_n)\mid +n^{1/2} f(x_{1n}^{1/2},x_{2n}^{1/2}))\geq 1-\bar{\alpha}_n.\]
We have the following bounding for the tail probability of $\mid n^{1/2}(\psi_n^1-\psi_0)\mid$:
\begin{eqnarray*}
P(\mid n^{1/2}(\psi_n^1-\psi_0)\mid >x)&\leq&P( \tilde{Z}_n +n^{1/2} f(x_{1n}^{1/2},x_{2n}^{1/2})>x,I_n=1)\\
&&\hspace*{-4cm}+
P(\tilde{Z}_n +n^{1/2} f(d_{01}(Q_n,Q_0)^{1/2},d_{02}(G_n,G_0)^{1/2})>x,I_n=0)\\
&\leq& P( \tilde{Z}_n +n^{1/2} f(x_{1n}^{1/2},x_{2n}^{1/2})>x)+\bar{\alpha}_n\\
&=&
P( \tilde{Z}_n>x-n^{1/2} f(x_{1n}^{1/2},x_{2n}^{1/2}))+\bar{\alpha}_n.
\end{eqnarray*}
 Let $\Phi_n(x)=P(\tilde{Z}_n>x)$.
Let $\tilde{q}_{n,0.05} $ be the solution in $x$ of 
\[
\Phi_n(x-n^{1/2}f(x_{1n}^{1/2},x_{2n}^{1/2}))+\bar{\alpha}_n=0.05.\]
Thus,
\[
\tilde{q}_{n,0.05}=n^{1/2}f(x_n^{1/2})+\Phi_n^{-1}(0.05-\bar{\alpha}_n).\]
For this choice we have $P(\mid n^{1/2}(\psi_n^1-\psi_0)\mid > \tilde{q}_{n,0.05})\leq 0.05$ so that 
\[
\psi_n^1\pm \tilde{q}_{n,0.05}/n^{1/2}\]
is a finite sample $>0.95$-confidence interval.

Let $x_n^{\#}$ be the above presented bootstrap estimator of $x_n$, $\tilde{Z}_n^{\#}=\mid n^{1/2}(P_n^{\#}-P_n)D^*(Q_n^{\#},G_n^{\#})\mid$, and 
$\Phi_n^{\#}(x)=P(\tilde{Z}_n^{\#}>x\mid (P_n:n\geq 1))$ be the bootstrap estimator of $\Phi_n$.
Then, our bootstrap estimator of this confidence interval is given by:
\[
\psi_n^1\pm \tilde{q}_{n,0.05}^{\#}/n^{1/2},\]
where 
\[
\tilde{q}_{n,0.05}^{\#}=n^{1/2}f(x_n^{\#1/2})+\Phi_n^{\#-1}(0.05-\bar{\alpha}_n).\]

 In order for this confidence interval to be asymptotically sharp one will need to make sure that $x_n$ converges to zero faster than $n^{-1/2}$. Our conservative bound for $x_n^{\#}$  in the previous subsection is too large. Instead, we might estimate $x_n^{\#}$ so that 
 \[
 P( A_{1}(P_n^{\#},P_n)<x_{1n}^{\#},A_2(P_n^{\#},P_n)<x_{2n}^{\#}\mid (P_n:n\geq 1))\geq 1-\bar{\alpha}_n,\]
 where $A_1(P_n^{\#},P_n)\equiv \mid (P_n^{\#}-P_n)L_1(Q_n^{\#},Q_n)\mid$ and $A_2(P_n^{\#},P_n)\equiv \mid (P_n^{\#}-P_n)L_2(G_n^{\#},G_n)\mid$.
 Then, $x_n^{\#}$ converges to zero at a rate faster than $n^{-1/2}$ for slowly converging $\bar{\alpha}_n$.
 
 

%This proves the weak convergence of $X_n$, and, similarly, it follows that the nonparametric bootstrap yields a consistent estimator of this limit distribution $X_0$.We also have that the asymptotic equicontinuity of $Z_n$ w.r.t. variance dissimilarity $d(f_1,f_2)=P_0(f_1-f_2)^2$, and the continuity of $D^*(Q,G)$, $L_1(Q,Q_0)$ and $L_2(G,G_0)$ w.r.t. $d_{01}(Q,Q_0)+d_{02}(G,G_0)$ implies that  $X_n$ is asymptotically equicontinuous w.r.t. $d((Q,G),(Q_0,G_0))=d_{01}(Q,Q_0)+d_{02}(G,G_0)$.Thus, the consistency of $Q_n,G_n$ w.r.t. $d_{01}$ and $d_{02}$ implies that $X_n(Q_n,G_n)-X_n(Q_0,G_0)\rightarrow_p 0$, where we note that $X_n(Q_0,G_0)=n^{1/2}(P_n-P_0)D^*(Q_0,G_0)$. This proves then also that $X_n(Q_n,G_n)\Rightarrow_d N(0,\sigma^2_0)$.Since the nonparametric bootstrap is consistent, it also follows that  $X_n^{\#}(Q_n^{\#},G_n^{\#})-X_n^{\#}(Q_n,G_n)\rightarrow_p 0$ and $X_n^{\#}(Q_n^{\#},G_n^{\#})\Rightarrow_d N(0,\sigma^2_0)$, conditional on $(P_n:n\geq 1)$.\begin{lemma}\label{lemmaXnweakconv}We have that $X_n=g(Z_n)$, where $Z_n=(n^{1/2}(P_n-P_0)f:f\in {\cal F}_1)$ is the empirical process indexed by class ${\cal F}_1$ (\ref{calf1}) contained in class of cadlag functions with sectional variation norm bounded by some $M<\infty$.Thus,$X_n=(X_n(f):f\in {\cal F})\Rightarrow_d X_0=g(Z_0)$ in $\ell^{\infty}({\cal F})$.In particular, $\pl X_n\pl_{\cal F}\equiv \sup_{f\in {\cal F}}\mid X_n(f)\mid\Rightarrow_d \pl X_0\pl_{\cal F}$.Let $X_n^{\#}=g(Z_n^{\#})$, where $Z_n^{\#}=(n^{1/2}(P_n^{\#}-P_n):f\in {\cal F}_1)$ be the nonparametric bootstrapped version of $X_n$.We have \[X_n^{\#}\Rightarrow_d X_0\mbox{ conditional on $(P_n:n\geq 1)$}.\]We also have $X_n(Q_n,G_n)-XLogic in this theorem, including selection of x_n.\pl X_n^{\#}\pl_{{\cal F}(x_n)}\Rightarrow_d \mid N(0,\sigma^2_0)\mid$, conditional on $(P_n:n\geq 1)$.For a fixed $x$, $\pl X_n^{\#}\pl_{{\cal F}(x)}\Rightarrow_d \pl X_0\pl_{{\cal F}(x)}$, conditional on $(P_n:n\geq 1)$.We have $\mid n^{1/2}(\psi_n^*-\psi_0)\mid\sim\leq \mid X_n(Q_n,G_n)\mid $, while $P(\mid X_n(Q_n,G_n)\mid >x)\leq P(\pl X_n\pl_{{\cal F}(x_n)}>x)+\alpha_n$, where$x_n$ and $\alpha_n$ are  chosen so that $P(d_{01}(Q_n,Q_0)<x_{1n},d_{02}(G_n,G_0)<x_{2n})\geq 1-\alpha_n$, $\alpha_n\rightarrow 0$.\end{theorem}

% sampling distribution for $\mid n^{1/2}(\psi_n^*-\psi_0)\mid$, for a sequence
%We can consistently estimate the limit distribution on the right-hand side. Let $S_{x_0,0}(\cdot)$ be the survivor function of $\sigma_0^{-1}\pl X_0\pl_{{\cal F}(x_0)$. Let $S_{x_0,n}$ be a consistent estimator of this survivor function. We estimate $P( \sigma_n^{-1}\pl X_n\pl_{{\cal F}(x_n)}>x)$with $S_{x_n,n}(x)$. We also define $S^n_{x_0,0}(\cdot)$ as the survivor function of $\sigma_n^{-1}\pl X_n\pl_{{\cal F}(x_0)}$.


%Let $q_{0.95,n}^{\#}$ be defined as $F^{-1}_{x_n,n}(0.95+\alpha_n)$, the $0.95+\alpha_n$-quantile of the cumulative distribution function $F_{x_n,n}^{\#}$.
%\[S_{x_n,n}^{\#}(q_{0.95,n}^{\#})= 0.05-\alpha_n .\]The resulting $0.95$-confidence interval is given by\[\psi_n^*\pm q_{0.95,n}^{\#}/n^{1/2} .\]
%By the asymptotic equicontinuity of $X_n$, we have  $\pl X_n\pl_{{\cal F}(x_n)}\Rightarrow_d N(0,\sigma^2_0)$, and similarly that $\pl X_n^{\#}\pl_{{\cal F}(x_n)}\Rightarrow_d N(0,\sigma^2_0)$, conditional on $(P_n:n\geq 1)$. As a consequence,  $q_{0.95,n}^{\#}\rightarrow 1.96$ converges to the $0.975$-quantile of the standard normal distribution.This confidence interval converges to the Wald-type confidence interval $\psi_n^*\pm 1.96\sigma_0/n^{1/2}$.
%Now find a $T_{1n}$, $T_{2n}$.

%The proposed confidence interval is given by $\psi_n^*\pm q_{0.95,n}^{\#}(x_n)/n^{1/2}$.


 


%The optimal choice $x_n$ minimizing the width of the confidence interval would thus be given by:\[x_n^*\equiv \arg\min_{x}F_{x,n}^{\#,-1}(0.95+(T_{n}^{\#}(x_{1}/M_1)+T_{n}^{\#}(x_{2}/M_2)) ).\]It seems reasonable to set $x_1=c$ and $x_2=c M_2/M_1$ so that $T_{n}^{\#}(x_1/M_1)=T_{n}^{\#}(x_2/M_2)$.Then, the optimal $c$ is given by\[c_n^*\equiv  \arg\min_{c}S_{x(c),n}^{\#,-1}(0.05-2T_{n}^{\#}(c/M_1) ) ,\]where $x(c)=(c,c M_2/M_1)$.

%\subsection{Practical implementation}The implementation of this method requires determining a supremum  $\sup_{f\in {\cal F}_n(x_n^{\#})}\mid X_n^{\#}(f)\mid$ of the bootstrapped process $X_n^{\#}$ over $(Q,G) $ in the $x_n^{\#}$-neighborhood${\cal F}_n(x_n^{\#})$  of  $(Q_n,G_n)$. It appears reasonable to assume that the supremum will be attained at the edge of ${\cal F}_n(x_n^{\#})$. One might aim to approximate this supremum by randomly sampling elements $Q$ and $G$ on the $x_n$-edge of this neighborhood.For example, suppose that $d_{n1}(Q,Q_n)=\pl Q-Q_n\pl^2$ is an $L^2$-norm. Suppose we determine a scheme that allows us to sample functions $e$ such that $\pl e\pl^2=x_{1n}^{\#}$. Each such a draw determines a draw $Q=Q_n+e$.Similarly, one samples $G=G_n+e$ resulting in a sample $f_1,\ldots,f_J$ of size $J$ on the $x_n$-edge of ${\cal F}_n(x_n^{\#})$ The maximum  $\max_j \mid X_n^{\#}(f_j)\mid$ provides then an approximation of the desired supremum $\sup_{f\in {\cal F}_n(x_n^{\#})}\mid X_n^{\#}(f)\mid$.Implementation of the supremum $\pl n^{1/2}(\bar{P}_n^{\#}-\bar{P}_n)\pl_{\infty}$ for the sake of determining $x_n^{\#}$ is significantly easier but could also be carried out by taking a random sample from its domain $[0,\tau]$. The other components of this method are straightforward to implement.
 


 



==> archive_mark.tex <==

\section{The nonparametric bootstrap applied to highly conservative finite sample bound on exact second-order expansion of HAL-TMLE}
Obtaining $S_{x,n}^{\#,-1}$ can be highly computer intensive. Therefore we also propose a conservative method that is not asymptotically optimal but is easier to implement.

Consider the CV-TMLE. Then
\begin{eqnarray*}
\psi_n^*-\psi_0&\leq&\mid E_{B_n}(P_{n,B_n}^1-P_0)D^*(Q_{n,B_n}^*,G_{n,B_n})+E_{B_n}f(\pl \bar{P}_{n,B_n}-\bar{P}_0\pl_{\infty}M_1,\pl \bar{P}_{n,B_n}-\bar{P}_0\pl_{\infty}M_2).
\end{eqnarray*}
Select $x_n$ so that $n^{1/2}\pl \bar{P}_{n,B_n}-\bar{P}_0\pl_{\infty}<x_n$ with probability at least $1-\alpha_n$.
Let $A_n$ be the indicator that $n^{1/2}\pl \bar{P}_{n,B_n}-\bar{P}_0\pl_{\infty}<x_n$ so that $P(A_n=1)\leq \alpha_n$.
Let $Z_n=n^{1/2}E_{B_n}(P_{n,B_n}^1-P_0)D^*(Q_{n,B_n}^*,G_{n,B_n})$.
We have
\begin{eqnarray*}
n^{1/2}\mid \psi_n^*-\psi_0\mid&\leq &Z_n+I_{A_n}
f(x_nM_1,x_nM_2)\\
&& +I_{A_n^c}E_{B_n}f(n^{1/2}\pl \bar{P}_{n,B_n}-\bar{P}_0\pl_{\infty}M_1,n^{1/2}\pl \bar{P}_{n,B_n}-\bar{P}_0\pl_{\infty}M_2).
\end{eqnarray*}
So
\begin{eqnarray*}
P(n^{1/2}\mid \psi_n^*-\psi_0\mid >x)&\leq & P (Z_n+f(x_nM_1,x_nM_2)>x)+\alpha_n .
\end{eqnarray*}
We have the following normal approximation:
\[
Z_n+f(x_nM_1,x_nM_2)\sim N(f(x_nM_1,x_nM_2),\sigma^2_n),\]
where
\[
\sigma^2_n=E_{B_n}P_{n,B_n}^1 \{ D^*(Q_{n,B_n}^*,G_{n,B_n})\}^2.\]
Let $q_{n,0.95}$ be the $1-(0.05-\alpha_n)$ quantile of $N(f(x_nM_1,x_nM_2),\sigma^2_n)$: i.e.,
$q_{n,0.95}=Z_{1-0.05-\alpha_n} \sigma_n+f(x_nM_1,x_nM_2)$, where $Z_{q}$ is the $q$-quantile of the standard normal $N(0,1)$. Then our proposed confidence interval is given by $\psi_n^*\pm q_{n,0.95}/n^{1/2}$.
One could aim to select $\alpha_n$ to minimize $q_{n,0.95}$ in order to minimize the width of this conservative confidence interval.
This confidence interval only relies on having to estimate the survivor distribution of the supremum norm of $\bar{P}_n-\bar{P}_0$. In the above method we use the nonparametric bootstrap to estimate this distribution, but we could also have based it on the Gaussian limit process of $n^{1/2}(\bar{P}_n-\bar{P}_0)$ by estimating the covariance structure of this process and then simulating many replicates from this Gaussian process and each time evaluating its supremum.
Note also that this confidence interval shrinks at a rate slower than $n^{-1/2}$, so that asymptotically it has coverage $1$.








\section{Some fundamental results}
%HAL MLE analysis, Integration by parts
\begin{lemma}
Let $F,Z\in D[0,\tau]$. For a $F\in D[0,\tau]$ define the supremum norm $\pl F\pl_{\infty}=\sup_{x\in [0,\tau]}\mid F(x)\mid$ and its sectional variation norm as follows:
 \[
 \pl F\pl_v^*=F(0)+\sum_{s\subset\{1,\ldots,d\}}\int_{(0_s,x_s]} dF_s(u_s),\] where
$F_s(u_s)=F(u_s,0_{-s})$ is the $s$-specific section of $F$ that sets the coordinates in the complement of $s$ equal to 0.
For any cadlag function $F\in D[0,\tau]$ with $\pl F\pl_v^*<\infty$, we have
\[
F(x)=F(0)+\sum_{s\subset\{1,\ldots,d\}}\int_{(0_s,x_s]} dF_s(u_s).\]
For a given function $Z\in D[0,\tau]$ we define
\[
\bar{Z}(u)=Z([u,\tau]).\]
For any two functions $F,Z\in D[0,\tau]$ with $\pl F\pl_v^*<\infty$ and $\pl Z\pl_v^*<\infty$, we have the following integration by parts formula:
\[
\int_{[0,\tau]} F(x)dZ(x)=F(0)\bar{Z}(0) +\sum_s \int_{u_s} \bar{Z}(u_s,0_{-s})dF_s(u_s).\]
This implies
\]
\int_{[0,\tau]} F(x)dZ(x)\leq \pl \bar{Z}\pl_{\infty}\pl F\pl_v^* .\]
\end{lemma}
{\bf Proof:}
The representation of $F(x)$ is presented in \citep{Gill&vanderLaan&Wellner94,vanderLaan15}. Using this representation yields the presented integration by parts formula as follows:
\begin{eqnarray*}
\int F dZ&=&\int \{F(0)+\sum_s \int_{(0_s,x_s]} dF_s(u)\} dZ(x)\\
&=&F(0) Z([0,\tau])+\sum_s \int_x\int_{u_s} I_{x_s\geq u_s} dF_s(u_s),dZ(x)\\
&=& F(0)Z([0,\tau])+\sum_s \int_{u_s} Z([u_s,\tau_s]\times [0_{-s},\tau_{-s}]) dF_s(u_s)\\
&\leq & \max_s \sup_{u_s\in [0_s,\tau_s]}\mid Z ([u_s,\tau_s]\times [0_{-s},\tau_{-s}])\mid \pl F\pl_v^*\\
&=& \pl Z\pl_{\infty} \pl F\pl_v^*.\Box
\end{eqnarray*}

\begin{lemma}\label{lemma2}
Let $O\sim P_0\in {\cal M}$. Let $Q:{\cal M}\rightarrow Q({\cal M})$ be a function valued parameter and let $L:Q({\cal M})\rightarrow D[0,\tau]$ be a loss function so that $Q_0\equiv Q(P_0)=\arg\min_{Q\in Q({\cal M})}P_0L(Q)=\arg\min_{Q\in Q({\cal M})} \int L(Q)(o)dP_0(o)$.
 Let $\hat{Q}:{\cal M}_{NP}\rightarrow Q({\cal M})$ be an estimator  $Q_n\equiv \hat{Q}(P_n)$ so that $P_n L_1(Q_n)=\min_{Q\in Q({\cal M})}P_n L(Q)$.
 Let $d_0(Q,Q_0)=P_0L(Q)-P_0L(Q_0)$ be the loss-based dissimilarity.
 Then,
 \[
 d_0(Q_n,Q_0)\leq -(P_n-P_0)\{L(Q_n)-L(Q_0)\}.
 \]
 If for each $Q\in Q({\cal M})$ we have $\pl L(Q)\pl_v^*<M_1$ for some $M_1<\infty$, then
 \[
E_0 d_0(Q_n,Q_0)=O(n^{-1/2-\alpha(d)},\]
where $\alpha(d)=1/(2d+4)$.
 \end{lemma}




\section{General approach for finite sample inference}
Let $O_1,\ldots,O_n$ be $n$ i.i.d. copies of a random variable $O\sim P_0\in {\cal M}$.
Let $\Psi:{\cal M}\rightarrow\openr$ be a real valued parameter that is pathwise differentiable at each $P\in {\cal M}$ with
canonical gradient $D^*(P)\in L^2_0(P)$.
Define the second-order remainder
\[
R_2(P,P_0)=\Psi(P)-\Psi(P_0)+(P-P_0)D^*(P),\]
where $(P-P_0)D^*(P)=-P_0D^*(P)$.
Let $Q:{\cal M}\rightarrow Q({\cal M})$ be a function valued parameter so that $\Psi(P)=\Psi_1(Q(P))$ for some $\Psi_1$.
For notational convenience, we will abuse  notation  by referring to the target parameter with $\Psi(Q)$ and $\Psi(P)$ interchangeably.
Let $G:{\cal M}\rightarrow G({\cal M})$ be a function valued parameter so that $D^*(P)=D^*_1(Q(P),G(P))$ for some $D^*_1$. Again, we will use the notation $D^*(P)$ and $D^*(Q,G)$ interchangeably.
Let $L_1:Q({\cal M})\rightarrow D[0,\tau]$ and $L_2:G({\cal M})\rightarrow D[0,\tau]$ be loss functions so that $P_0L_1(Q_0)=\min_{Q\in Q({\cal M})}P_0L_1(Q)$ and
$P_0L_2(G_0)=\min_{G\in G({\cal M})} P_0L_2(G)$. Let $d_{01}(Q,Q_0)=P_0L_1(Q)-P_0L_1(Q_0)$ and $d_{02}(G,G_0)=P_0L_2(G)-P_0L_2(G_0)$ be the loss-based dissimilarities for these two parameters.
We assume that these loss function map into functions in $D[0,\tau]$ with a sectional variation norm bounded by some universal finite constant:
\begin{eqnarray}
M_1\equiv \sup_{P\in {\cal M}}\pl L_1(Q(P))\pl_v^* &<&\infty\\
 M_2\equiv \sup_{P\in {\cal M}}\pl L_2(G(P))\pl_v^*&<& \infty.
 \end{eqnarray*}
Let \[
R_2(P,P_0)=R_{20}(Q,G,Q_0,G_0)\]
for some mapping $R_{20}()$ possibly indexed by $P_0$. We often have that
$R_{20}(Q,G,Q_0,G_0)$ is a sum of term of second-order term of the types $\int (H_1(Q)-H_1(Q_0))^2 f(P,P_0)dP_0$, $\int (H_2(G)-H_2(G_0))^2 f(P,P_0)dP_0$ and
$\int (H_1(Q)-H_1(Q_0))(H_2(G)-H_2(G_0))f(P,P_0) dP_0$ for certain specifications of $H_1, H_2 $ and $f()$.
We assume the following:
\begin{equation}\label{boundingR2}
\mid R_2(P,P_0)\mid =\mid R_{20}(Q,G,Q_0,G_0)\mid \leq f(d_{01}^{1/2}(Q,Q_0),d_{02}^{1/2}(G,G_0))\end{equation}
for some function $f:\openr^2_{\geq 0}\rightarrow\openr_{\geq 0}$ that is differentiable, and is monotone increasing so that $f(x_1,x_2)\leq f(y_1,y_2)$ if $y_1\geq x_1$ and $y_2\geq x_2$. In addition, we assume that $c f(x_1,x_2)=f(c^{1/2}x_1,c^{1/2}x_2)$.
A typical choice of function will be of the form $ax_1^2+bx_2^2+c \mid x_1x_2\mid$ for some positive constants $a,b,c$.
Suppose that $\sup_{P,P_1\in {\cal M}}P \{L_1(Q(P_1))-L_1(Q(P))\}\leq c_1$ and $\sup_{P,P_1\in {\cal M}}P\{L_2(G(P_1))-L_2(G(P))\}<c_2$, then we also know that
$R_2(Q_n^*,G_n,Q_0,G_0)\leq f(c_1,c_2)$. Therefore, we assume that $f$ is chosen so that these global bounds are respected:
$f(x_1,x_2)=f(\min(x_1,c_1),\min(x_2,c_2))$.



We estimate $Q_0,G_0$ with MLEs satisfying
\begin{eqnarray*}
P_n L_1(Q_n)&=&\min_{Q\in Q({\cal M})} P_n L_1(Q)\\
P_n L_2(G_n)&=& \min_{G\in G({\cal M})}P_n L_2(G).
\end{eqnarray*}
By Lemma \ref{lemma2}, we have that $d_{01}(Q_n,Q_0)=O_P(n^{-1/2-\alpha(d)})$ and $d_{02}(G_n,G_0)=O_P(n^{-1/2-\alpha(d)})$ even for a nonparametric model.
More importantly for this article is that we have upper bounds:
\begin{eqnarray*}
d_{01}(Q_n,Q_0)&\leq&-(P_n-P_0)L_1(Q_n,Q_0)\\
d_{02}(G_n,G_0)&\leq&-(P_n-P_0)L_2(G_n,G_0),
\end{eqnarray*}
where we defined $L_1(Q,Q_0)=L_1(Q)-L_1(Q_0)$ and $L_2(G,G_0)=L_2(G)-L_2(G_0)$.
If we estimate $Q_0$ and $G_0$ instead with super-learners $\tilde{Q}_n,\tilde{G}_n$  in which the library contains this HAL-MLE $Q_n$ and $G_n$, then, by the oracle inequality for the super-learner, $we know that
$d_{01}(\tilde{Q}_n,Q_0)$ and $d_{02}(\tilde{G}_n,G_0)$ will be asymptotically equivalent with the oracle selected estimator, so that $d_{01}(Q_n,Q_0)$ and $d_{02}(G_n,G_0)$ represent upper bounds.  Therefore, assuming that each estimator in the library of the super-learners for $Q_0$ and $G_0$  falls it the parameter space of $Q$ and $G$, respectively, our proposed  confidence interval can also be used for the super-learner, although they might be overly conservative.

Let $Q_n^*=Q_{n,\epsilon_n}$ for an $\epsilon_n=\arg\min_{\epsilon}P_n L_1(Q_{n,\epsilon})$ and local or universal least favorable submodel $\{Q_{\epsilon}:\epsilon\}\subset Q({\cal M})$. We assume that the TMLE  $Q_n^*$ satisfies
\begin{equation}\label{efficeqn}
P_n D^*(Q_n^*,G_n)=r_n,\end{equation}
where $r_n=o_P(n^{-1/2})$. By using a universal least favorable submodel we have $r_n=0$.
We now want to obtain a similar bound for $d_{01}(Q_n^*,Q_0)$.
\begin{lemma}
Assume $\epsilon\rightarrow L(Q_{n,\epsilon})$ is differentiable with a uniformly bounded derivative on an interval $\epsilon \in (-\delta,\delta)$ for some $\delta>0$.
Then,
\[
d_{01}(Q_n^*,Q_0)\leq -(P_n-P_0)L(Q_n,Q_0)+O_P(n^{-1}).\]
\end{lemma}
This also proves that the iterative TMLE using a {\em finite} (uniform in $n$) number of iterations satisfies $d_{01}(Q_n^*,Q_0)\leq -(P_n-P_0)L(Q_n,Q_0)+O_P(n^{-1})$. So  if needed  one can iterate the TMLE to guarantee that $r_n$ is small enough to be neglected.
\newline
{\bf Proof:}
Define $\epsilon_{0n}=\arg\min_{\epsilon}P_0 L_1(Q_{n,\epsilon})$.
We have
\begin{eqnarray*}
P_0L(Q_n^*)-P_0L(Q_0)&=&\{ P_0L(Q_{n,\epsilon_n}-P_0L(Q_{n,\epsilon_{0n}})\}
+\{P_0L(Q_{n,\epsilon_{0n}})-P_0L(Q_n)\}\\
&&+\{P_0L(Q_n)-P_0L(Q_0)\}\\
&\leq& -(P_n-P_0)L(Q_{n,\epsilon_n},Q_{n,\epsilon_{0n} })-(P_n-P_0)L(Q_n,Q_0).
\end{eqnarray*}
Since $\epsilon_n$ is a MLE of $\epsilon_{0,n}$ based on a 1-dimensional parametric model, under weak regularity condition we have
$\mid \epsilon_n-\epsilon_{0n}\mid =O_P(n^{-1/2})$. In addition, an exact first order Tailor expansion $f(\epsilon_n)-f(\epsilon_{0n})=\frac{d}{d\xi}f(\xi)(\epsilon_n-\epsilon_{0n})$ for a $\xi$ between $\epsilon_n$ and $\epsilon_{0n}$, we obtain
\[
L(Q_{n,\epsilon_n})-L(Q_{n,\epsilon_0})=(\epsilon_n-\epsilon_0)\frac{d}{d\epsilon_{n,1}}L(Q_{n,\epsilon_{n,1}}).\]
It then follows that $(P_n-P_0)L(Q_{n,\epsilon_n},Q_{n,\epsilon_{0n} })=O_P(n^{-1})$. Therefore, we will ignore the contribution of this term.
So we have
\[
d_{01}(Q_n^*,Q_0)\leq -(P_n-P_0)L(Q_n,Q_0)+O_P(n^{-1}) \Box .\]

By (\ref{boundingR2}) we have  established the following upper bound for the second-order remainder $R_2(P_n^*,P_0)$.

\begin{lemma}
We have
\[
n^{1/2}\mid R_2(Q_n^*,G_n,Q_0,G_0)\mid \leq f(\mid n^{1/2}(P_n-P_0)L_1(Q_n,Q_0)\mid^{1/2},\mid n^{1/2}(P_n-P_0)L_2(G_n,G_0)\mid^{1/2})+O_P(n^{-1/2}).
\]

\end{lemma}

We have the following identity for the TMLE:
\begin{eqnarray*}
\Psi(Q_n^*)-\Psi(Q_0)&=&(P_n-P_0)D^*(Q_n^*,G_n)+R_{20}(Q_n^*,G_n,Q_0,G_0)+r_n\\
&=&(P_n-P_0)D^*(Q_0,G_0)+(P_n-P_0)\{D(Q_n^*,G_n)-D^*(Q_0,G_0)\}+R_{20}(Q_n^*,G_n,Q_0,G_0)+r_n.
\end{eqnarray*}
Combined with our upper bound for $R_2(P_n^*,P_0)$ this yields:
\begin{eqnarray*}
 n^{1/2}\mid \Psi(Q_n^*)-\Psi(Q_0)\mid&\leq & \mid  n^{1/2}(P_n-P_0)D^*(Q_n^*,G_n) +
%\mid n^{1/2}(P_n-P_0)(D^*(Q_n^*,G_n)-D^*(Q_0,G_0))\mid\\
 f(\mid n^{1/2}(P_n-P_0)L(Q_n,Q_0)\mid, \mid n^{1/2}(P_n-P_0)L(G_n,G_0)\mid)\mid  +O_P(n^{-1/2})+r_n
\end{eqnarray*}
We have
\[
n^{1/2}(P_n-P_0D^*(Q_n^*,G_n)=n^{1/2}(P_n-P_0)D^*(Q_n,G_n)+r_{1n},\]
where
\[
r_{1n}=n^{1/2}(P_n-P_0)\{D^*(Q_{n,\epsilon_n},G_n)-D^*(Q_n,G_n)\}.\]
As shown above, under a weak regularity condition, this can be bounded by $\epsilon_n=o_P(n^{-1/4})$ times an empirical process indexed by a Donsker class, so that this term will be at least
$O_P(n^{-1/4})$. Therefore, one might decide to neglect this remainder $r_{1n}$ for inference.
Define
\begin{eqnarray*}
N_{0n}&\equiv& n^{1/2}(P_n-P_0)D^*(Q_0,G_0)\\
X_{0,n}(Q,G)&=&  n^{1/2}(P_n-P_0)D^*(Q_{\tilde{\epsilon}_n},G)
+
f(\mid n^{1/2}(P_n-P_0)L(Q,Q_0)\mid, \mid n^{1/2}(P_n-P_0)L(G,G_0)\mid),
\end{eqnarray*}
where $\tilde{\epsilon}_n=\arg\min_{\epsilon}P_n L(Q_{\epsilon})$ is the MLE for the least favorable submodel through $Q$.
As mentioned above, one can simplify this process $X_{0,n}(Q,G)$ by setting $\tilde{\epsilon}_n=0$ while introducing an $o_P(n^{-1/4})$.

Of course, $N_{0n}$ is an absolute value of a  simple empirical mean and thus converges to the absolute value of the  optimal (most concentrated) normal limit distribution $N(0,\sigma^2_0=P_0D^*(P_0)^2)$.
For notational convenience, let ${\cal F}=Q({\cal M})\times G({\cal M})$ be the parameter space for $(Q,G)$.
$X_{0,n}=(X_{0n}:f\in {\cal F})$ is a process indexed by ${\cal F}$ and can thus be viewed as a random element of $\ell^{\infty}({\cal F})$.
We view $(N_{0,n},X_{0,n})$ as a random element of $\openr\times \ell^{\infty}({\cal F})$.
$X_{0,n}$  is a simple function of three empirical processes indexed by classes of functions ${\cal F}_1=\{L(Q,Q_0):Q\in Q({\cal M})\}$, ${\cal F}_2=\{L(G,G_0):G\in G({\cal M})\}$ and
${\cal F}_3=\{D^*(Q,G):(Q,G)\in {\cal F}\}$ that are contained in the Donsker class of cadlag functions with sectional variation norm bounded by some $M<\infty$. Consider the empirical process $Z_{n,4}=(\sqrt{n}(P_n-P_0)(f):f\in {\cal F}_4)$ indexed by the union ${\cal F}_4=\cup_{j=1}^3 {\cal F}_j$ which is a subset of the Donsker class ${\cal F}_v^*$ of cadlag functions with sectional variation bounded by universal constant. Thus, $Z_{n,4}\Rightarrow_d Z_{0,4}$ in $\ell^{\infty}({\cal F}_4)$ for a uniquely defined Gaussian process $Z_0$. Note that $X_{0,n}$ is a function of $Z_{n,4}$: $X_{0,n}=g(Z_{n,4})$ for a well defined function $g$. By the continuous mapping theorem and the continuity of this function $g$, we have that $X_{0,n}\Rightarrow_d X_0\equiv g(Z_{0,4}), converges in distribution to a function $g$ of this Gaussian process $Z_{0,4}$.
%check this more carefully, i.e. continuity.
More generally, $(N_{0,n},X_{0,n})$ converges jointly in distribution to $(N_0,X_0)$ in $\openr\times \ell^{\infty}({\cal F})$.

This proves the following lemma.
\begin{lemma}\label{weakconvergencesupnorm}
We have $(N_{0,n},X_{0,n})\Rightarrow_d (N_0,X_0)$ in $\openr\times \ell^{\infty}({\cal F})$, where $X_0$ is  a simple function $g()$ of the Gaussian limit process $Z_{0,4}$ of the empirical process $Z_{n,4}=(\sqrt{n}(P_n-P_0)(f):f\in {\cal F}_4)$:
\[
X_0(Q,G)= Z_{04}(D^*(Q_{\tilde{\epsilon}_0},G))\mid +
f(\mid Z_{04}(L(Q,Q_0))\mid, \mid Z_{04}(L(G,G_0))\mid).\]
%This implies also that\[(N_{0,n}+\pl X_{0,n}\pl_{\cal F} \Rightarrow_d (N_0+\pl X_0\pl_{{\cal F}} .\]
\end{lemma}


Each of the three empirical processes indexed by the classes ${\cal F}_j$, $j=1,2,3$, is asymptotically equicontinuous w.r.t. variance dissimilarity $d(f_1,f_2)=P_0(f_1-f_2)^2$.
We assume that convergence of $(Q_n,G_n)$ to $(Q_0,G_0)$ w.r.t. $d_{01}(Q_n,Q_0)+d_{02}(G_n,G_0)$ implies
\begin{eqnarray}\label{continuityD*}
P_0 \{D^*(Q_n,G_n)-D^*(Q_0,G_0)\}^2&\rightarrow_p& 0\\
P_0\{L_1(Q_n,Q_0)\}^2&\rightarrow_p& 0\nonumber \\
P_0\{L_2(G_n,G_0)\}^2&\rightarrow_p& 0.\nonumber
\end{eqnarray}
Then it follows that $X_{0,n}(Q_n,G_n)\rightarrow_d N(0,\sigma^2_0)$.
This proves the following lemma.
\begin{lemma}
We have that $X_{0,n}(Q_n,G_n)\Rightarrow_d N(0,\sigma^2_0)$.
\end{lemma}


We claim that we can consistently estimate the limit distribution of $X_{0,n}(Q_n,G_n)$ with the nonparametric bootstrap $X_{n}^{\#}(Q_n^{\#},G_n^{\#})$.
\begin{lemma}
Let $P_n^{\#}$ be the empirical probability measure of an i.i.d. sample $O_1^{\#},\ldots,O_n^{\#}\sim P_n$ and let $Q_n^{\#}=\arg\min_{Q\in Q({\cal M})}P_n^{\#}L_1(Q)$ and
$G_n^{\#}=\arg\min_{G\in G({\cal M})}P_n^{\#}L_2(G)$ be the corresponding HAL-MLEs based on these bootstrap samples.
Let
\[
X_{n}^{\#}(Q_n^{\#},G_n^{\#})=n^{1/2}(P_n^{\#}-P_n)D^*(Q_n^{\#},G_n^{\#})
+
f(\mid n^{1/2}(P_n^{\#}-P_n)L(Q_n^{\#},Q_n)\mid, \mid n^{1/2}(P_n^{\#}-P_n)L(G_n^{\#},G_n)\mid).\]
Suppose that \begin{eqnarray}\label{continuityD*Pn}
P_n \{D^*(Q_n^{\#},G_n^{\#})-D^*(Q_n,G_n)\}^2&\rightarrow_p& 0\\
P_n\{L_1(Q_n^{\#},Q_n)\}^2&\rightarrow_p& 0\nonumber \\
P_n\{L_2(G_n^{\#},G_n)\}^2&\rightarrow_p& 0.\nonumber
\end{eqnarray}
Then, $X_n^{\#}(Q_n^{\#},G_n^{\#})$ converges in distribution to $N_0=N(0,\sigma^2_0), conditional on $(P_n:n\geq 1)$.

Regarding verification of (\ref{continuityD*Pn}, we note the following. We have
\[
d_{n1}(Q_n^{\#},Q_n)\equiv P_n\{ L_1(Q_n^{\#})-L_1(Q_n)\}\leq -(P_n^{\#}-P_n)\{L_1(Q_n^{\#})-L_1(Q_n)\},\]
and similarly $d_{n2}(G_n^{\#},G_n)\leq -(P_n^{\#}-P_n)L_2(G_n^{\#},G_n)$.
As a consequence, we have that $d_{n1}(Q_n^{\#},Q_n)=P_n L_1(Q_n^{\#})-P_nL_1(Q_n)$ and $d_{n2}(G_n^{\#},G_n)=P_n L_2(G_n^{\#})-P_nL_2(G_n)$ are both $O_P(n^{-1/2})$.
In addition, if  $d_{n1}(Q_n^{\#},Q_n)\rightarrow 0$ and $d_{n2}(G_n^{\#},G_n)\rightarrow 0$ implies that $P_n \{L_1(Q_n^{\#})-L_1(Q_n)\}^2\rightarrow 0$ and
$P_n \{L_2(G_n^{\#})-L_2(G_n)\}^2\rightarrow 0$, then we have $d_{n1}(Q_n^{\#},Q_n)=o_P(n^{-1/2})$ and $d_{n2}(G_n^{\#},G_n)=o_P(n^{-1/2})$.
If these dissimilarities are equivalent in the sense that  $\pl L_1(Q_n^{\#})-L_1(Q_n)\pl_{P_n}^2\lesssim d_{n1}(Q_n^{\#},Q_n)$ and $\pl L_2(G_n^{\#})-L_2(G_n)\pl_{P_n}^2\lesssim d_{n2}(G_n^{\#},G_n)$, then we have
$d_{n1}(Q_n^{\#},Q_n)=O_P(n^{-1/2-\alpha(d)})$ and $d_{n2}(G_n^{\#},G_n)=O_P(n^{-1/2-\alpha(d)})$.

If $L_1(Q)(O)=(Y-Q(X))^2$ is the squared error loss function, then $d_{n1}(Q_n^{\#},Q_n)=P_n (Q_n^{\#}-Q_n)^2$. Thus, $P_n  \{L_1(Q_n^{\#})-L_1(Q_n)\}^2\leq C P_n \{L_1(Q_n^{\#})-L_1(Q_n)\}=O_P(n^{-1/2})$ for some $C<\infty$, and thereby
\[
d_{n1}(Q_n^{\#},Q_n)=P_n (Q_n^{\#})-Q_n)^2=O_P(n^{-1/2-\alpha(d)}).\]
\end{lemma}
{\bf Proof:}
Firstly, the nonparametric bootstrap is consistent for an empirical process indexed by a uniform Donsker class so that
$Z_{n,4}^{\#}=(\sqrt{n}(P_n^{\#}-P_n)f:f\in {\cal F}_4)\Rightarrow_d Z_{0,4}$ conditional on $(P_n:n\geq 1)$.
Each of the three empirical processes indexed by the classes ${\cal F}_j$, $j=1,2,3$, is asymptotically equicontinuous w.r.t. variance dissimilarity $d_n(f_1,f_2)=P_n(f_1-f_2)^2$ uniformly in $(P_n:n\geq 1)$.
Therefore, if (\ref{continuityD*Pb}) holds, then we obtain the stated weak convergence of the bootstrapped process $X_n^{\#}(Q_n^{\#},G_n^{\#})$ to $N(0,\sigma^2_0)$.
%\begin{eqnarray}\label{continuityD*Pn}P_n \{D^*(Q_n^{\#},G_n^{\#})-D^*(Q_n,G_n)\}^2&\rightarrow_p& 0\\P_n\{L_1(Q_n^{\#},Q_n)\}^2&\rightarrow_p& 0\nonumber \\P_n\{L_2(G_n^{\#},G_n)\}^2&\rightarrow_p& 0.\nonumber\end{eqnarray}
%This shows that the conditional probability distribution of $X_n^{\#}(Q_n^{\#},G_n^{\#})$, conditional on $(P_n:n\geq 1)$ approximately equals the probability distribution of \[X_{0,n}(Q_n^{\#},G_n^{\#})=n^{1/2}(P_n-P_0)D^*(Q_n^{\#},G_n^{\#})+f(\mid n^{1/2}(P_n-P_0)L(Q_n^{\#},Q_n)\mid, \mid n^{1/2}(P_n-P_0)L(G_n^{\#},G_n)\mid).\]To prove that the latter converges weakly to $N(0,\sigma^2_0)$ we need to show that $P_0 \{D^*(Q_n^{\#},G_n^{\#})-D^*(Q_0,G_0)\}^2\rightarrow_p 0$ and$P_0 L_1(Q_n^{\#},Q_n)\rightarrow_p 0$ and $P_0 L_2(G_n^{\#},G_n)\rightarrow_p 0$.
Thus, it remains to analyze the estimator $Q_n^{\#}$ and $G_n^{\#}$ as estimators of $Q_n,G_n$, conditional on $(P_n:n\geq 1)$.
Let's consider the HAL-MLE $Q_n^{\#}$ of $Q_n$ based on $P_n^{\#}$.
We can analyze the HAL-MLE $Q_n^{\#}$ of $Q_n$ in an analogue manner as we analyze $Q_n$.
We have
\[
P_n\{ L_1(Q_n^{\#})-L_1(Q_n)\}\leq -(P_n^{\#}-P_n)\{L_1(Q_n^{\#})-L_1(Q_n)\}.\]
From this it follows that $0\leq d_{n,1}(Q_n^{\#},Q_n)\equiv P_n\{L_1(Q_n^{\#})-L_1(Q_n)\}=O_P(n^{-1/2})$.
We now like to show that $P_n \{L_1(Q_n^{\#})-L_1(Q_n)\}^2\lessim P_n \{L_1(Q_n^{\#})-L_1(Q_n)\}$.
Let's first aim to establish this  in general. Subsequently, we explicitly verify that it holds for the squared error loss.

Consider a path $Q_{n,\epsilon}(x)=(1+\epsilon h(0))Q_n(0)+\sum_s \int_{(0_s,x_s]}(1+\epsilon h_s(u_s)) dQ_{n,s}(u_s))$, where $r(h,Q_n)\equiv  h(0)Q_n(0)+\sum_s \int_{(0_s,\tau_s]} h_s(u_s)\mid dQ_{n,s}(u_s)\mid \leq 0$ and $h$ is uniformly bounded. Let ${\cal H}$ be the set of $h$ functions (i.e., functions of $s,u_s$).
Note that  for $\epsilon\geq 0$, we have
\begin{eqnarray*}
\pl Q_{n,\epsilon}\pl_v^*&=&(1+\epsilon h(0))\mid Q_n(0))+\sum_s \int_{(0_s,\tau_s]}(1+\epsilon h_s(u_s))\mid dQ_{n,s}(u_s)\mid \\
&=& \pl Q_n\pl_v^*+\epsilon\left\{ h(0)Q_n(0)+\sum_s \int_{(0_s,\tau_s]}h_s(u_s) \mid dQ_{n,s}(u_s)\mid \\
&\geq & \pl Q_n\pl_v^*,
\end{eqnarray*}
by assumption on $h$.
Thus, this represents a path of cadlag functions with sectional variation norm is smaller equal than $M=\pl Q_n\pl_v^*$.
We also have that
 \[
 Q_{n,\epsilon}-Q_n=\epsilon\left\{ Q_n(0)h(0)+ \sum_s \int_{(0_s,x_s]} h_s(u_s)dQ_{n,s}(u_s))\right\} .\]
 Thus,
 \[
 \frac{d}{d\epsilon}Q_{n,\epsilon}=f(h,Q_n)\equiv Q_n(0)h(0)+ \sum_s \int_{(0_s,x_s]} h_s(u_s)dQ_{n,s}(u_s)) .\]
 Note that $f(h,Q_n)$ represents a difference of two cadlag functions.
 Let ${\cal S}\equiv \{f(h,Q_n): h\in {\cal H}\}$.
 By definition of the MLE $Q_n$, we also have that $\epsilon \rightarrow P_n L_1(Q_{n,\epsilon})$ is minimal over $[0,\delta)$ at $\epsilon =0$.
This shows that the right-derivative $\frac{d}{d\epsilon+ }P_n L_1(Q_{n,\epsilon })\geq 0$ at $\epsilon =0$ and thus for each $h\in {\cal H}$, we have
\[
P_n \frac{d}{dQ_n}L_1(Q_n)(f(h,Q_n)) \geq 0 .\]
Suppose that $Q_n^{\#}-Q_n\in {\cal S}=\{f(h,Q_n):h\in {\cal H}\}$. Since $\pl Q_n^\#}\pl_v^*=\pl Q_n\pl_v^*=M$ will both achieve the maximal allowed variation norm,
and  $Q_{n,s}^{\#}\ll Q_{n,s}$ for all subset $s$ (i.e., the support of $Q_{n,s}^{\#}$ is a subset of the support of $Q_{n,s}$ due to the support of $P_n^{\#}$ being  a subset of support of $P_n$),
one would generally expect that indeed this difference $Q_n^{\#}-Q_n$ is included in ${\cal S}$.
To make this concrete, let's solve explicitly for $h$ so that $Q_n^{\#}-Q_n=f(h,Q_n)$.
We have
\begin{eqnarray*}
Q_n^{\#}-Q_n&=&Q_n^{\#}(0)-Q_n(0)+\sum_s\int_{(0_s,x_s]} d(Q_{n,s}^{\#}-dQ_{n,s})(u_s)\\
&=& Q_n^{\#}(0)-Q_n(0)+\sum_s \int_{(0_s,x_s]} \frac{d(Q_{n,s}^{\#}-dQ_{n,s})}{dQ_{n,s}} dQ_{n,s}(u_s),
\end{eqnarray*}
where we used that $Q_{n,s}^{\#}\ll Q_{n,s}$ for each subset $s$.
Define for each $s$
\begin{eqnarray*}
h(Q_n^{\#},Q_n)(0)&=&(Q_n^{\#}(0)-Q_n(0))/Q_n(0)\\
h_s(Q_n^{\#},Q_n)&=&\frac{d(Q_{n,s}^{\#}-dQ_{n,s})}{dQ_{n,s}} .
\end{eqnarray*}
For this choice $h(Q_n^{\#},Q_n)$, we have $f(h,Q_n)=Q_n^{\#}-Q_n$.
Let's now check if we have that for this choice of $h$ $r(h,Q_n)\leq 0$.
We have
\begin{eqnarray*}
r(h,Q_n)&=&Q_n^{\#}(0)-Q_n(0)+\int_{(0_s,\tau_s]}\frac{dQ_{n,s}^{\#}-dQ_{n,s}}{dQ_{n,s}}\mid dQ_{n,s}\mid\\
&=&Q_n^{\#}(0)-Q_n(0)+\int_{(0_s,\tau_s]}I(dQ_{n,s}\geq 0) d(Q_{n,s}^{\#}-dQ_{n,s})+I(dQ_{n,s}<0)d(Q_{n,s}-Q_{n,s}^{\#})\\
&=&-\pl Q_n\pl_v^*+Q_n^{\#}(0)+\int_{(0_s,\tau_s]}I(dQ_{n,s}\geq 0) dQ_{n,s}^{\#}-I(dQ_{n,s}<0)dQ_{n,s}^{\#})\\
&\leq&-\pl Q_n\pl_v^*+\pl Q_n^{\#}\pl_v^*\\
&\leq &0,
\end{eqnarray*}
since $\pl Q_n^{\#}\pl_v^*\leq M=\pl Q_n\pl_v^*$.
Thus, this proves that indeed $Q_n^{\#}-Q_n\in {\cal S}$.
 Then, we have
\[
P_n \frac{d}{dQ_n}L_1(Q_n)(Q_n^\#}-Q_n)\geq 0.\]
Suppose that $L_1(Q)$ is differentiable at $Q=Q_n$ so that
\[
P_n \{L_1(Q_n^{\#})-L_1(Q_n)\}=P_n \frac{d}{dQ_n}L_1(Q_n)(Q_n^{\#}-Q_n)+R_2(Q_n^{\#},Q_n)\]
for some second-order remainder involving square differences between $Q_n^{\#}$ and $Q_n$. Thus we have
\[
0\leq P_n\{L_1(Q_n^{\#})-L_1(Q_n)\}\geq R_2(Q_n^{\#},Q_n).\]
This shows that the second-order remainder $R_2(Q_n^{\#},Q_n)\geq 0$ while it is also a square of $Q_n^{\#}-Q_n$.
Therefore, this can be expected to imply
\]
P_n \{L_1(Q_n^{\#})-L_1(Q_n)\}^2\lesssim P_n\{L_1(Q_n^{\#})-L_1(Q_n)\}.\]

HERE I AM, COrrECt THIS LEMMA. VERY IMPORTANT LEMMA ALLOWING US NP BOOTSTRAP WORKS
This proves the following lemma for general loss functions.
\begin{lemma}
Consider the collection of paths  $Q_{n,\epsilon}(x)=(1+\epsilon h(0))Q_n(0)+\sum_s \int_{(0_s,x_s]}(1+\epsilon h_s(u_s)) dQ_{n,s}(u_s))$, where $h(0)Q_n(0)+\sum_s \int_{(0_s,\tau_s]} h_s(u_s)\mid dQ_{n,s}(u_s)\mid =0$ and $h$ is uniformly bounded.
Suppose that for local neighborhoods of $\epsilon $ at $0$ these are submodels of the parameter space of $Q:{\cal M}\rightarrow Q({\cal M})$.
Then, there exists a $\delta>0$ so that $\epsilon\rightarrow \pl Q_{n,\epsilon}\pl_v^*=\pl Q_n\pl_v^*$ is constant in $\epsilon\in (-\delta,\delta)$.
In addition, we have for each of these paths
\[
\left . \frac{d}{d\epsilon} P_n L_1(Q_{n,\epsilon})\right |_{\epsilon =0}=0 .\]
Therefore, we have that for each $h\in {\cal H}$,
\[
0=P_n \frac{d}{dQ_n}L_1(Q_n)(f(h,Q_n)).\]
\end{lemma}



%Therefore we have $0=\sum_i f(h)(X_i)(Y_i-Q_n(X_i))=0$ for all $h$ satisfying the condition $h(0)\mid Q_n(0)\mid +\sum_s \int_{(0_s,\tau_s]} h_s(u_s)\mid dQ_{n,s}(u_s)\mid =0$. Since $Q_{n,s}^{\#}\ll Q_{n,s}$ for all subset $s$ (i.e. support of $Q_{n,s}^{\#}$ is a subset of support of $Q_{n,s}$ due to the support of $P_n^{\#}$ being  a subset of support of $P_n$. Therefore, we there exists a $h$ such that $f(h)=(Q_n^{\#}-Q_n)$.


Consider the squared error loss $L_1(Q)=(Y-Q(X))^2$. Then,
\begin{eqnarray*}
P_n L_1(Q_n^{\#})-P_nL_1(Q_n)&=&\frac{1}{n}\sum_i \{2Y_iQ_n(X_i)-2Y_i Q_n^{\#}(X_i)+Q_n^{\#2}(X_i)-Q_n^2(X_i)\}\\
&=& \frac{1}{n}\sum_i\{2Y_i(Q_n-Q_n^{\#})(X_i)+Q_n^{\#2}(X_i)-Q_n^2(X_i)\}\\
&=&\frac{1}{n}\sum_i \{2(Y_i-Q_n(X_i))(Q_n-Q_n^{\#})(X_i)+2Q_n(X_i)(Q_n-Q_n^{\#})(X_i)+Q_n^{\#2}(X_i)-Q_n^2(X_i)\}
&=&\frac{1}{n}\sun_i (Q_n-Q_n^{\#})^2(X_i)+\frac{1}{n}\sum_i 2(Q_n-Q_n^{\#})(X_i)(Y_i-Q_n(X_i)).
\end{eqnarray*}
We want to show that $ \frac{1}{n}\sum_i 2(Q_n-Q_n^{\#})(X_i)(Y_i-Q_n(X_i))\geq 0$.
The general equation above $P_n \frac{d}{dQ_n}L_1(Q_n)(f(h,Q_n)) \geq 0$ corresponds for the squared error loss with:
\[
2 P_n -f(h,Q_n)(Y-Q_n(X)) \geq 0.\]
As above shown, we have $f(h,Q_n)$ can be chosen to be equal to $Q_n^{\#}-Q_n$.
So this proves that $P_n (Q_n^{\#}-Q_n)(Y-Q_n)\leq 0$. This proves the desired result.

%This shows that $\sum_i (Q_n^{\#}-Q_n)(X_i)(Y_i-Q_n(X_i))=0$.
Thus, this proves that
\[
d_{n1}(Q_n^{\#},Q_n)=P_n \{L_1(Q_n^{\#})-L_1(Q_n)\}\geq P_n (Q_n-Q_n^{\#})^2.\]
Thus, $P_n  \{L_1(Q_n^{\#})-L_1(Q_n)\}^2\leq C P_n \{L_1(Q_n^{\#})-L_1(Q_n)\}=O_P(n^{-1/2})$ for some $C<\infty$.
As a consequence, using empirical process results (van der Vaart, Wellner), it follows that $(P_n^{\#}-P_n)\{L_1(Q_n^{\#})-L_1(Q_n)\}=O_P(n^{-1/2-\alpha(d)})$, and thus that
\[
d_{n1}(Q_n^{\#},Q_n)=P_n (Q_n^{\#})-Q_n)^2=P_n \{L_1(Q_n^{\#})-L_1(Q_n)\}=O_P(n^{-1/2-\alpha(d)}).\]
%Given the weak convergence of $Z_{n,4}^{\#}$ and this latter consistency of $Q_n^{\#}$ to $Q_n$, it follows that $X_n^{\#}(Q_n^{\#},G_n^{\#})$ converges weakly $N_0=N(0,\sigma^2_0)$, conditional on $(P_n:n\geq 1)$.


Given that the $Z_{n,4}^{\#}$ is a good robust approximation of  $Z_{n,4}$ (i.e., there  are empirical process results available providing bounds on this approximation) and that the bootstrapped HAL-MLEs $Q_n^{\#}$ and $G_n^{\#}$ converge at the same rate to $Q_n$ and $G_n$ as $Q_n,G_n$ converge to $Q_0,G_0$, this lemma strongly suggest that $X_n^{\#}(Q_n^{\#},G_n^{\#})$ represents a robust approximation of the finite sample distribution $X_{0,n}(Q_n,G_n)$. Therefore, we suggest using this bootstrapped random variable as a finite sample approximation of the finite sample distribution of $X_{0,n}(Q_n,G_n)$.

Let $q_{n,0.95}^{\#}$ be the $0.95$-quantile of $\mid X_n^{\#}(Q_n^{\#},G_n^{\#})\mid$.
Then, a higher order $0.95$-confidence interval is given by:
\[
\psi_n^*\pm q_{n,0.95}^{\#}/n^{1/2} .\]
We could also replace the process $X_{0,n}$ by its normalized version:
\begin{eqnarray*}
X_{0,n}^I(Q,G)=  \sigma_n(Q,G)^{-1}n^{1/2}(P_n-P_0)D^*(Q,G)
+\sigma_n(Q,G)^{-1}f(\mid n^{1/2}(P_n-P_0)L_1(Q,Q_0)\mid, \mid n^{1/2}(P_n-P_0)L_2(G,G_0)\mid),
\end{eqnarray*}
where $\sigma_n^2(Q,G)=P_n D^*(Q_n,G_n)^2$.
Let $X_n^{I,\#}$ be the bootstrapped version of $X_{0,n}^I$ and let $q_{n,0.95}^{I,\#}$ be the $0.95$-quantile of
$\mid X_n^{I,\#}(Q_n^{\#},G_n^{\#})$. In that case the proposed $0.95$-confidence interval is given by:
\[
\psi_n^*\pm q_{n,0.95}^{I,\#}\sigma_n/n^{1/2}.\]
It is not clear if this normalization provides a finite sample improvement.



%to do, finsih nonparametric bootstrap proposal, if works. Then do conservative supremum norm bounding. Then do root-n based confidence interval, and possibly shrining by ration J(delta_n)/J(1).
We will now consider a more conservative approach in which we bound $X_{0,n}(Q_n,G_n)$ by a supremum norm of $X_{0,n}$ over a set that will contain $(Q_n,G_n)$ with probability tending to 1, and then use the nonparametric bootstrap to estimate the distribution of the supremum.

Let $x_n=(x_{1n},x_{2n})$ and ${\cal F}(x_n)=\{(Q,G): d_{01}(Q,Q_0)\leq x_{1n},d_{02}(G,G_0)\leq x_{2n}\}$.
The analogue of Lemma \ref{weakconvergencesupnorm} is given by the following lemma.
\begin{lemma}
For each fixed $x=(x_1,x_2)$, we have
\[
\pl X_{0,n}\pl_{{\cal F}(x)}\Rightarrow_d \pl X_0\pl_{{\cal F}(x)} .\]
\end{lemma}

Suppose that $(Q_n,G_n)\in {\cal F}(x)$ for some $x$. Then we have the following bound:
\[
\mid n^{1/2}(\psi_n^*-\psi_0)\mid\leq\mid \pl X_{0,n}\pl_{{\cal F}(x)}+O_P(n^{-1/2})+r_n .\]
Let $T_{1n}$ and $T_{2n}$ be tail probabilities that dominate the survivor distribution of $d_{01}(Q_n,Q_0)$ and $d_{02}(G_n,G_0)$, respectively:
\begin{eqnarray*}
P(d_{01}(Q_n,Q_0)>x)&\leq & T_{1n}(x)\\
P(d_{02}(G_n,G_0)>x)&\leq & T_{2n}(x).
\end{eqnarray*}
Let $x_n=(x_{1n},x_{2n})$ be a given sequence and define $\alpha_{1n}=T_{1n}(x_{1n})$ and $\alpha_{2n}=T_{2n}(x_{2n})$.
Let $\alpha_n=\alpha_{1n}+\alpha_{2n}$.
Let $B_n$ be the indicator that both $d_{01}(Q_n,Q_0)\leq x_{1n}$ and $d_{02}(G_n,G_0)\leq x_{2n}$.
Then, it follows that $P(B_n=1)\geq 1-\alpha_n$.
We have
\begin{eqnarray*}
\mid \sqrt{n}(\psi_n^*-\psi_0)\mid& \leq& X_n(Q_n,G_n)+r_n+O_P(n^{-1/2})\\
&=& N_{0n}+I(B_n=1)X_n(Q_n,G_n)+I(B_n=0)X_n(Q_n,G_n)+r_n+O_P(n^{-1/2})\\
&\leq& N_{0n} +I(B_n=1) \pl X_n\pl_{{\cal F}(x_n)}+I(B_n=0)\pl X_n\pl_{{\cal F}}+r_n+O_P(n^{-1/2}).
\end{eqnarray*}
Let $\tilde{r}_n=r_n+O_P(n^{-1/2})$.
Thus,
\begin{eqnarray*}
P(\mid \sqrt{n}(\psi_n^*-\psi_0)\mid >x)&\leq& P( \pl X_n\pl_{{\cal F}(x_n)}B_n+\pl X_n\pl_{\cal F}(1-B_n)+\tilde{r}_n>x)\\
&=& P(\pl X_n\pl_{{\cal F}(x_n)}+\tilde{r}_n>x,B_n=1)\\
&&+ P(\pl X_n\pl_{\cal F}+\tilde{r}_n>x,B_n=0)\\
&\leq&P(\pl X_n\pl_{{\cal F}(x_n)}+\tilde{r}_n>x,B_n=1)+ \alpha_n \\
&\leq& P(\pl X_n\pl_{{\cal F}(x_n)}+\tilde{r}_n>x)+ \alpha_n \\
\end{eqnarray*}
Thus, we have the following lemma.
\begin{lemma}
P(\mid n^{1/2}(\psi_n^*-\psi_0)\mid>x)\leq P(\pl X_n\pl_{{\cal F}(x_n)}+\tilde{r}_n>x)+\alpha_n .\]
\end{lemma}
%Similarly, it follows that we have the following lemma.\begin{lemma}\[P(\sigma_n^{-1}\mid n^{1/2}(\psi_n^*-\psi_0)\mid>x)\leq P(\sigma_n^{-1}\pl X_n\pl_{{\cal F}(x_n)}+\sigma_n^{-1}\tilde{r}_n>x)+ \alpha_n .\]\end{lemma}

%Now derive confidence interval
For a given $x_n=x_0$, we have
\[
P(\pl X_n\pl_{{\cal F}(x_0)}+\tilde{r}_n>x)\rightarrow P(\pl X_0\pl_{{\cal F}(x_0)}>x),
\]
or more generally,
\[ \pl X_n\pl_{{\cal F}(x_0)}+\tilde{r}_n\Rightarrow_d  \mid \pl X_0\pl_{{\cal F}(x_0)} .\]
We can consistently estimate the distribution of $\pl X_n\pl_{{\cal F}(x)}$ with the nonparametric bootstrap version
$\pl X_n^{\#}\pl_{{\cal F}(x)}$, where
\[
X_n^{\#}(Q,G)=n^{1/2}(P_n^{\#}-P_n)D^*(Q,G)+f(n^{1/2}(P_n^{\#}-P_n)L_1(Q,Q_n),n^{1/2}(P_n^{\#}-P_n)L_2(G,G_n)).\]
Let $S_{x_0,n}^{\#}$ be the survivor function of $\pl X_n^{\#}\pl_{{\cal F}(x_0)}$.
%We can consistently estimate the limit distribution on the right-hand side. Let $S_{x_0,0}(\cdot)$ be the survivor function of $\sigma_0^{-1}\pl X_0\pl_{{\cal F}(x_0)$. Let $S_{x_0,n}$ be a consistent estimator of this survivor function. We estimate $P( \sigma_n^{-1}\pl X_n\pl_{{\cal F}(x_n)}>x)$with $S_{x_n,n}(x)$. We also define $S^n_{x_0,0}(\cdot)$ as the survivor function of $\sigma_n^{-1}\pl X_n\pl_{{\cal F}(x_0)}$.


Let $q_{0.95,n}^{\#}$ be defined by
\[
S_{x_n,n}^{\#}(q_{0.95,n}^{\#})= 0.05-\alpha_n .\]
Our proposed higher order $0.95$-confidence interval is given by
\[
\psi_n\pm q_{0.95,n}^{\#}/n^{1/2} .\]
By the asymptotic equicontinuity of $X_n$, we have  $\pl X_n\pl_{{\cal F}(x_n)}\Rightarrow_d N(0,\sigma^2_0)$, and similarly that $\pl X_n^{\#}\pl_{{\cal F}(x_n)}\Rightarrow_d N(0,\sigma^2_0)$, conditional on $(P_n:n\geq 1)$. As a consequence,
 $q_{0.95,n}^{\#}\rightarrow 1.96$ converges to the $0.975$-quantile of the standard normal distribution.
 Thus our higher order 0.95-confidence interval converges to the Wald-type confidence interval $\psi_n\pm 1.96\sigma_0/n^{1/2}$.
%Now find a $T_{1n}$, $T_{2n}$.

In order to implement the above confidence interval we  need to derive a method for determining $x_n$.
By our integration by parts lemma, we have
\begin{eqnarray*}
d_{01}(Q_n,Q_0)&\leq & \pl \bar{P}_n-\bar{P}_0\pl_{\infty}\pl L_1(Q_n,Q_0)\pl_v^* \\
d_{02}(G_n,G_0)&\leq &\pl \bar{P}_n-\bar{P}_0\pl_{\infty}\pl L_2(G_n,G_0)\pl_v^* .
\end{eqnarray*}
Since the covering number $N(\epsilon,L^2(Q),{\cal F}_I)$ for the class of indicators ${\cal F}_I=\{I_{[u,\tau]}:u\in [0,\tau]\}$ behaves as $\epsilon^{-d}$ and
$E\pl \sqrt{n}(\bar{P}_n-\bar{P}_0)\pl_{\infty}\lesssim J(1,{\cal F}_I)\equiv \sup_Q \int_{0}^1 \sqrt{\log N(\epsilon,L^2(Q),{\cal F}_I)} d\epsilon$, it follows that
$E\pl \sqrt{n}(\bar{P}_n-\bar{P}_0)\pl_{\infty}=O(d^{1/2})$.
So this shows that
\begin{eqnarray*}
Ed_{01}(Q_n,Q_0)&=& O(d^{1/2}n^{-1/2}M_1)\\
Ed_{02}(G_n,G_0)&=& O(d^{1/2}n^{-1/2}M_2).
\end{eqnarray*}
In particular, this shows that
\[
E\mid R_{2n}\mid =O(n^{-1/2}d^{1/2} \sqrt{M_1M_2}).\]
In fact, we have that the (Corollary 2.2.5, van der Vaart, Wellner, 1996) the $\psi_1$-orlics norm $\pl\cdot\pl_{\psi_1}$ of $\pl \sqrt{n}(P_n-P_0)\pl_{\infty}$ is bounded by $J(1,{\cal F})$, which shows that
\[
\pl \pl n^{1/2}/d^{1/2}(\bar{P}_n-\bar{P}_0)\pl_{\infty} \pl_{\psi_1}=O(1),\]
where $\psi_p(x)=\exp(x^p)-1$, $p=1,,2$.
This bound on the orlics norm of the supremum implies a bound on its tail probability:
\[
P(\pl n^{1/2}/d^{1/2}(\bar{P}_n-\bar{P}_0)\pl_{\infty}>x)\leq \exp(-C x)\]
for some $C<\infty$.
Thus, this proves the following lemma.
\begin{lemma}
For some $C<\infty$,
\[
P(n^{1/2}d_{01}(Q_n,Q_0)>x)\leq P( \pl n^{1/2}/d^{1/2}(\bar{P}_n-\bar{P}_0)\pl_{\infty}M_1>x/d^{1/2})\leq \exp(-C x/(d^{1/2}M_1) ).\]
Similarly,
\[
P(n^{1/2}d_{01}(G_n,G_0)>x)\leq P( \pl n^{1/2}/d^{1/2}(\bar{P}_n-\bar{P}_0)\pl_{\infty}M_2>x/d^{1/2})\leq \exp(-C x/(d^{1/2}M_2) ).\]
\end{lemma}
%Similarly,\begin{eqnarray*}P(\mid \sqrt{n}R_{2n}\mid >x)&\leq& P(\delta^{-1} \pl \sqrt{n}(P_n-P_0)\pl_{\infty,1} \sqrt{M_1M_2} >x)\\&=& P(\pl \sqrt{n}(P_n-P_0)\pl_{\infty,1}> x\delta/\sqrt{M_1M_2})\\&\leq& \exp(-C\delta x/\sqrt{M_1M_2}).\end{eqnarray*}
These bounds are of theoretical interest since they demonstrate the impact of the bounds $M_1,M_2$ on the sectional variation norm of $L_1(Q_n,Q_0)$ and $L_2(G_n,G_0)$ and of the dimension $d$ of the data $O$.

For practical purposes, we would need to know $C$ for these bounds to become useful. However, we can consistently estimate the distribution of $\pl n^{1/2}(\bar{P}_n-\bar{P}_0)\pl_{\infty}$ (e.g.) with the nonparametric bootstrap), so that we do not need to use a conservative finite sample bound.
Therefore, we just use the following lemma.
\begin{lemma}
Let  $T_{0,n}(x)\equiv P(\pl n^{1/2}(\bar{P}_n-\bar{P}_0)\pl_{\infty}>x)$.
Then, we have
\begin{eqnarray*}
P(n^{1/2}d_{01}(Q_n,Q_0)>x)&\leq& T_{0,n}(x/M_1)\\
P(n^{1/2}d_{02}(G_n,G_0)>x)&\leq & T_{0,n}(x/M_2).
\end{eqnarray*}
Let $\bar{N}_0$ be the Gaussian limit process of $n^{1/2}(\bar{P}_n-\bar{P}_0)$.
$T_{0,n}$ converges to the survivor function $T_0$ of $\pl \bar{N}_0\pl_{\infty}$.
Let $T_n^{\#}(x)=P(\pl n^{1/2}(\bar{P}_n^{\#}-\bar{P}_n)\pl_{\infty}>x)$. Then, conditional on $(P_n:n\geq 1)$,
$T_n^{\#}(x)\rightarrow T_0(x)$ for all $x\in \openr$.
\end{lemma}
%Now optimize w.r.t. choice $x_n$
%Let $T_n^{\#}$ be the estimator of the survivor function $T_{0,n}$ of $\pl n^{1/2}(\bar{P}_n-\bar{P}_0)\pl_{\infty}$ based on the nonparametric bootstrap.
For a given $x$, let $S_{x,n}^{\#}$ be an estimator of the survivor function  of $\pl X_n\pl_{{\cal F}(x_n)} based on the nonparametric bootstrap.
For a given $x_n=(x_{1n},x_{2n})$, let
\[
q_{0.95,n}^{\#}(x_n)=S_{x_n,n}^{\#,-1}(0.05-(T_{n}^{\#}(x_{1n}/M_1)-T_{n}^{\#}(x_{2n}/M_2)) ).\]
The proposed confidence interval is given by $\psi_n^*\pm q_{0.95,n}^{\#}(x_n)/n^{1/2}$.

The optimal choice $x_n$ minimizing the width of our higher order confidence interval would thus be given by:
\[
x_n^*\equiv \arg\min_{x}S_{x,n}^{\#,-1}(0.05-(T_{n}^{\#}(x_{1}/M_1)-T_{n}^{\#}(x_{2}/M_2)) ).\]
It seems reasonable to set $x_1=c$ and $x_2=c M_2/M_1$ so that $T_{n}^{\#}(x_1/M_1)=T_{n}^{\#}(x_2/M_2)$.
Then, the optimal $c$ is given by
\[
c_n^*\equiv  \arg\min_{c}S_{x(c),n}^{\#,-1}(0.05-2T_{n}^{\#}(c/M_1) ) ,\]
where $x(c)=(c,c M_2/M_1)$.

Obtaining $S_{x,n}^{\#,-1}$ can be highly computer intensive. Therefore we also propose a conservative method that is not asymptotically optimal but is easier to implement.

Consider the CV-TMLE. Then
\begin{eqnarray*}
\psi_n^*-\psi_0&\leq&\mid E_{B_n}(P_{n,B_n}^1-P_0)D^*(Q_{n,B_n}^*,G_{n,B_n})+E_{B_n}f(\pl \bar{P}_{n,B_n}-\bar{P}_0\pl_{\infty}M_1,\pl \bar{P}_{n,B_n}-\bar{P}_0\pl_{\infty}M_2).
\end{eqnarray*}
Select $x_n$ so that $n^{1/2}\pl \bar{P}_{n,B_n}-\bar{P}_0\pl_{\infty}<x_n$ with probability at least $1-\alpha_n$.
Let $A_n$ be the indicator that $n^{1/2}\pl \bar{P}_{n,B_n}-\bar{P}_0\pl_{\infty}<x_n$ so that $P(A_n=1)\leq \alpha_n$.
Let $Z_n=n^{1/2}E_{B_n}(P_{n,B_n}^1-P_0)D^*(Q_{n,B_n}^*,G_{n,B_n})$.
We have
\begin{eqnarray*}
n^{1/2}\mid \psi_n^*-\psi_0\mid&\leq &Z_n+I_{A_n}
f(x_nM_1,x_nM_2)\\
&& +I_{A_n^c}E_{B_n}f(n^{1/2}\pl \bar{P}_{n,B_n}-\bar{P}_0\pl_{\infty}M_1,n^{1/2}\pl \bar{P}_{n,B_n}-\bar{P}_0\pl_{\infty}M_2).
\end{eqnarray*}
So
\begin{eqnarray*}
P(n^{1/2}\mid \psi_n^*-\psi_0\mid >x)&\leq & P (Z_n+f(x_nM_1,x_nM_2)>x)+\alpha_n .
\end{eqnarray*}
We have the following normal approximation:
\[
Z_n+f(x_nM_1,x_nM_2)\sim N(f(x_nM_1,x_nM_2),\sigma^2_n),\]
where
\[
\sigma^2_n=E_{B_n}P_{n,B_n}^1 \{ D^*(Q_{n,B_n}^*,G_{n,B_n})\}^2.\]
Let $q_{n,0.95}$ be the $1-(0.05-\alpha_n)$ quantile of $N(f(x_nM_1,x_nM_2),\sigma^2_n)$: i.e.,
$q_{n,0.95}=Z_{1-0.05-\alpha_n} \sigma_n+f(x_nM_1,x_nM_2)$, where $Z_{q}$ is the $q$-quantile of the standard normal $N(0,1)$. Then our proposed confidence interval is given by $\psi_n^*\pm q_{n,0.95}/n^{1/2}$.
One could aim to select $\alpha_n$ to minimize $q_{n,0.95}$ in order to minimize the width of this conservative confidence interval.
This confidence interval only relies on having to estimate the survivor distribution of the supremum norm of $\bar{P}_n-\bar{P}_0$. In the above method we use the nonparametric bootstrap to estimate this distribution, but we could also have based it on the Gaussian limit process of $n^{1/2}(\bar{P}_n-\bar{P}_0)$ by estimating the covariance structure of this process and then simulating many replicates from this Gaussian process and each time evaluating its supremum.
Note also that this confidence interval shrinks at a rate slower than $n^{-1/2}$, so that asymptotically it has coverage $1$.

We can prove that the nonparametric bootstrap works for $Q_n$  and $G_n$ itself. SO I think we can prove that the NP bootstrap is consistent for the TMLE based on HAL.
Let's prove that results since that is a non conservativ method of interest clearly.



Write paper: A) NP bootstrap works for HAL-TMLE !!
B)  directly NP bootstrap $\pl Q_n-Q_0\pl $ and $\pl G_n-G_0\pl$ in this upper bound
C) NP bootstrap of upper bound of second-order term to get conservative inference
further bounding by (P_n-P)L_1(Q_n,Q) etc.
D)  bounding by supremum over set that shrinks to get more conservative result, still sharp in limit, cumbersome to implement
E) conservative bound, not even root -n rate but only relying on estimation of quantile of sup norm of indicator empirical process.

 \end{document}



\section{Idea I}
The general idea is to write $\psi_n-\psi_0=(P_n-P_0)f_n$ exact or $\mid \psi_n-\psi_0\mid \leq (P_n-P_0)f_n$, where $f_n\in {\cal F}$ with probability tending to 1.
We then estimate the $0.95$-quantile $q_{0.95}$ of $\pl G_n\pl_{\cal F}$, where $G_nf=\sqrt{n}(P_n-P_0)f$.
Our choice will be that ${\cal F}$ is class of cadlag functions with sectional variation norm bounded by a $M<\infty$.
Our confidence interval is then $\psi_n\pm q_{0.95,n}/\sqrt{n}$.
We can probably improve this by writing $\sqrt{n}(\psi_n-\psi_0)/\sigma_n=\sqrt{n}(P_n-P_0)f_n/\sigma_n$, and $\sigma_n=P_n (f_n-P_nf_n)^2$.
Then the confidence interval becomes $\psi_n\pm \sigma_n q_{0.95,n}/\sqrt{n}$.

{\bf Stochastic Domination of Remainder:}
We have
\[
R_{2n}=\int (Q_n-Q)(G_n-G)/G_n dP\leq \frac{1}{\delta}\pl Q_n-Q\pl_{P_0}\pl G_n-G\pl_{P_0}.\]
Let $L_1(Q)=(Y-Q(W))^2A$ and $L_2(G)=(A-G(W))^2$. We have
\begin{eqnarray*}
\pl Q_n-Q\pl_{P_0}&\leq& \sqrt{ -(P_n-P_0)\{L_1(Q_n)-L_1(Q)\}}\\
\pl G_n-G\pl_{P_0}&\leq &\sqrt{-(P_n-P_0)\{L_2(G_n)-L_2(G)\}.
\end{eqnarray*}
Let $f_1(Q)=L_1(Q)-L_1(Q_0)$ and $f_2(G)=L(G)-L(G_0)$.
Define also $f(Q,G)=D^*(Q,G)-D^*(Q_0,G_0)$.
So we have
\begin{eqnarray*}
\mid \sqrt{n}(\psi_n-\psi_0)\mid &\leq&\mid \sqrt{n}(P_n-P_0)D^*(Q_0,G_0)\mid +\mid  \sqrt{n}(P_n-P_0)f(Q_n,G_n)\mid \\
 &&+\frac{1}{\delta} \sqrt{\mid  \sqrt{n}(P_n-P_0) f_1(Q_n)\mid \mid \sqrt{n}(P_n-P_0)f_2(G_n)\mid }.
\end{eqnarray*}
Let ${\cal F}_1=\{f\in D[0,\tau]:\pl f\pl_v^*<M_1\}$ and ${\cal F}_2=\{f\in D[0,\tau]:\pl f\pl_v^*<M_2\}$ so that $(Q,G)\in{\cal F}= {\cal F}_1\times {\cal F}_2$.
Let $Z_n(f)=\sqrt{n}(P_n-P_0)f$ be the empirical process at a function $f$.
Let $N_{0n}=Z_n(D^*(Q_0,G_0))$, $Z_{n1}(Q,G)=Z_n(f(Q,G))$, $Z_{n2}(Q)=Z_n(f_1(Q))$, $Z_{n3}(G)=Z_n(f_2(G))$.
The process $Z_{n1}=(Z_{n1}(Q,G):(Q,G)\in {\cal F})$ is asymptotically equicontinuous at $(Q_0,G_0)$ w.r.t. $d_1((Q,G),(Q_0,G_0))=P_0 (D^*(Q,G)-D^*(Q_0,G_0))^2$.
The process $Z_{n2}=(Z_{n2}(Q):Q\in {\cal F}_1)$ is asymptotically equicontinuous at $(Q_0,G_0)$  w.r.t. $d_2(Q,Q_0)=P_0(L_1(Q)-L_1(Q_0))^2$.
The process $Z_{n3}=(Z_{n3}(G):G\in {\cal F}_2)$ is asymptotically equicontinuous at $(Q_0,G_0)$ w.r.t. $d_3(G,G_0)=P_0(L_2(G)-L_2(G_0))^2$.
We also have that the finite dimensional distributions of $(N_{0n},Z_{n1},Z_{n2},Z_{n3})$ converge to their corresponding multivariate normal distributions.
Thus, $(N_{0n},(Z_{n1},Z_{n2},Z_{n3}))\Rightarrow_d (N_0,(Z_{01},Z_{01},Z_{03}))$ in the  space $\openr\times \ell^{\infty,3}(\cal F})$, where $\ell^{\infty,3}({\cal F})$  consists of  functions $g=(g_1,g_2,g_3):{\cal F}\rightarrow\openr^3$ endowed with the supremum norm $\pl g\pl_{\cal F}=\sup_{f\in {\cal F}\max(\mid g_1(f)\mid ,\mid g_2(f)\mid ,\mid g_3(f)\mid )$.
For $f=(Q,G)$ and $f_0=(Q_0,G_0)$, let $d(f,g)=d_1(f,f_0)+d_2(f,f_0)+d_3(f,f_0)$.
Define the process $X_n=(X_n(Q,G):(Q,G)\in {\cal F})$:
\[
X_n(Q,G)=\mid Z_{n1}(Q,G)\mid +\frac{1}{\delta}\sqrt{ \mid Z_{n2}(Q)\mid Z_{n3}(G)\mid }.\]
By the continuous mapping theorem we have that $(N_{0n},X_n)\Rightarrow_d (N_0,X_0)$ in $\openr\times \ell^{\infty}(\cal F}$, where
$X_0=\mid Z_{01}\mid +\frac{1}{\delta}\sqrt{Z_{02}Z_{03}}$. In addition, $X_n$ is asymptotically equicontinuous w.r.t. $d((Q,G),(Q_0,G_0))=\pl Q-Q_0\pl_{P_0}^2+\pl G-G_0\pl_{P_0}^2$.
The continuous mapping theorem then also shows that $(N_{0n},\pl X_n\pl_{\cal F})\Rightarrow_d (N_0,\pl X_0\pl_{\cal F})$.
So we have the following stochastic domination result for the HAL-TMLE:
\begin{eqnarray*}
\mid \sqrt{n}(\psi_n-\psi_0)\mid &\leq &\mid N_{0n}\mid +\pl X_n\pl_{\cal F} \\
&\Rightarrow_d& \mid N_0\mid +\pl X_0\pl_{\cal F}.
\end{eqnarray*}
Let $q_{0.95}$ be the $0.95$-quantile of $\mid N_0+\pl X_0\pl_{\cal F}$. Then, $\psi_n\pm q_{0.95}/\sqrt{n}$ is an asymptotically valid $0.95$-confidence internal.
Let $\sigma^2_n=P_n D^*(Q_n,G_n)^2$, where we know that $\sigma^2_n\rightarrow_p \sigma^2_0=P_0 D^*(Q_0,G_0)^2$. Similarly,
\begin{eqnarray*}
\sigma_n^{-1}\mid \sqrt{n}(\psi_n-\psi_0)\mid &\leq &\mid \sigma_n^{-1} N_{0n}\mid +\pl \sigma_n^{-1}X_n\pl_{\cal F} \\
&\Rightarrow_d& \mid \sigma_0^{-1} N_0\mid +\sigma_0^{-1}\pl X_0\pl_{\cal F}.
\end{eqnarray*}
Let $q_{0.95}$
be the $0.95$-quantile of $\mid N(0,1)\mid +\sigma_0^{-1} \pl X_0\pl_{\cal F}$. Then, $\psi_n\pm q_{0.95}\sigma_n/\sqrt{n}$ is an asymptotically valid $0.95$-confidence internal.

This confidence interval does not shrink towards its asymptotic distribution based confidence interval.
We have
\[
\pl Q_n-Q_0\pl^2_{P_0}\leq \mid (P_n-P_0)f_1(Q_n)\mid .\]
By integration by parts we have
\begin{eqnarray*}
\int F dZ&=&\int \{F(0)+\sum_s \int_{(0_s,x_s]} dF_s(u)\} dZ(x)\\
&=&F(0) Z([0,\tau])+\sum_s \int_x\int_{u_s} I_{x_s\geq u_s} dF_s(u_s),dZ(x)\\
&=& F(0)Z([0,\tau])+\sum_s \int_{u_s} Z([u_s,\tau_s]\times [0_{-s},\tau_{-s}]) dF_s(u_s)\\
&\leq & \max_s \sup_{u_s\in [0_s,\tau_s]}\mid Z ([u_s,\tau_s]\times [0_{-s},\tau_{-s}])\mid \pl F\pl_v^*\\
&=& \pl Z\pl_{\infty,1} \pl F\pl_v^*,
\end{eqnarray*}
where
\[
\pl Z\pl_{\infty,1}=\sup_{u\in [0,\tau]}\mid Z([u,\tau])\mid .\]
Therefore, we have
\begin{eqnarray*}
\pl Q_n-Q_0\pl^2_{P_0}&\leq & \pl P_n-P_0\pl_{\infty,1}\pl f_1(Q_n)\pl_v^* \\
\pl G_n-G_0\pl^2_{P_0}&\leq &\pl P_n-P_0\pl_{\infty,1}\pl f_2(G_n)\pl_v^* .
\end{eqnarray*}
Since the covering number $N(\epsilon,L^2(Q),{\cal F}_I)$ for the class of indicators ${\cal F}_I=\{I_{[u,\tau]}:u\in [0,\tau]\}$ behaves as $\epsilon^{-d}$ and
$E\pl \sqrt{n}(P_n-P_0)\pl_{\infty,1}\lesssim J(1,{\cal F}_I)\equiv \sup_Q \int_{0}^1 \sqrt{\log N(\epsilon,L^2(Q),{\cal F}_I)} d\epsilon$, it follows that
$E\pl \sqrt{n}(P_n-P_0)\pl_{\infty,1}=O(d^{1/2})$.
So this shows that
\begin{eqnarray*}
E\pl Q_n-Q_0\pl^2_{P_0}&=& O(d^{1/2}n^{-1/2}M_1)\\
E\pl G_n-G_0\pl^2_{P_0}&=& O(d^{1/2}n^{-1/2}M_2).
\end{eqnarray*}
In particular, this shows that
\[
E\mid R_{2n}\mid =O(n^{-1/2}d^{1/2} \sqrt{M_1M_2}).\]
In fact, we have that the (Corollary 2.2.5, van der Vaart, Wellner, 1996) the $\psi_1$-orlics norm of $\pl \sqrt{n}(P_n-P_0)\pl_{\infty}$ is bounded by $J(1,{\cal F})$, which shows that
\[
\pl \pl \sqrt{n}(P_n-P_0)\pl_{\infty,1} \pl_{\psi_1}=O(d^{1/2}),\]
where $\psi_p(x)=\exp(x^p)-1$, $p=1,,2$.
This bound on the orlics norm of the supremum implies a bound on its tail probability:
\[
P(\pl \sqrt{n}(P_n-P_0)\pl_{\infty,1}>x)\leq \exp(-C x)\]
for some $C<\infty$.
Thus, this shows that
\[
P(n^{1/2}\pl Q_n-Q_0\pl^2_{P_0}>x)\leq P( \pl n^{1/2}(P_n-P_0)\pl_{\infty,1}M_1>x)\leq \exp(-C x/M_1).\]
Similarly,
\[
P(n^{1/2}\pl G_n-G_0\pl^2_{P_0}>x)\leq P( \pl n^{1/2}(P_n-P_0)\pl_{\infty,1}M_2>x)\leq \exp(-C x/M_2).\]
Similarly,
\begin{eqnarray*}
P(\mid \sqrt{n}R_{2n}\mid >x)&\leq& P(\delta^{-1} \pl \sqrt{n}(P_n-P_0)\pl_{\infty,1} \sqrt{M_1M_2} >x)\\
&=& P(\pl \sqrt{n}(P_n-P_0)\pl_{\infty,1}> x\delta/\sqrt{M_1M_2})\\
&\leq& \exp(-C\delta x/\sqrt{M_1M_2}).
\end{eqnarray*}
More importantly, we can consistently estimate the distribution of $\pl n^{1/2}(P_n-P_0)\pl_{\infty,1}$, so that we do not need to use a conservative finite sample bound.
Let's denote this distribution with $T_n(x)\equiv P(\pl n^{1/2}(P_n-P_0)\pl_{\infty,1}>x)$.
Then, we have
\begin{eqnarray*}
P(n^{1/2}\pl Q_n-Q_0\pl^2_{P_0}>x)&\leq& T_n(x/M_1)\\
P(n^{1/2}\pl G_n-G_0\pl^2_{P_0}>x)&\leq & T_n(x/M_2).
\end{eqnarray*}
Let $x_{1n}$ be a sequence so that $\alpha_{1n}\equiv T_n(x_{1n}/M_1)\rightarrow 0$ and similarly, let $x_{2n} be such that $\alpha_{2n}\equiv T_n(x_{2n}/M_2)\rightarrow 0$. Let $\alpha_n=\alpha_{1n}+\alpha_{2n}$.
Then
\[
P(\pl Q_n-Q_0\pl_{P_0}^2<x_{1n}/n^{1/2}\mbox{ and } \pl G_n-G_0\pl_{P_0}^2<x_{2n}/n^{1/2})> 1-\alpha_{n}.\]
For notational convenience, let $B(Q_n,G_n)$ be defined as the indicator on the event in the latter probability, so that $P(B(Q_n,G_n)=1)>1-\alpha_n$.
Define \[
{\cal F}(x_n)\equiv \{(Q,G): B(Q,G)=1\}.\]
Note that $P((Q_n,G_n)\in {\cal F}(x_n))> 1-\alpha_n$.
We have
\begin{eqnarray*}
\mid \sqrt{n}(\psi_n-\psi_0)\mid& \leq& N_{0n}+X_n(Q_n,G_n)\\
&=& N_{0n}+I((Q_n,G_n)\in {\cal F}(x_n))X_n(Q_n,G_n)+I((Q_n,G_n)\not\in {\cal F}(x_n))X_n(Q_n,G_n)\\
&\leq& N_{0n} +I(Q_n,G_n)\in {\cal F}(x_n) \pl X_n\pl_{{\cal F}(x_n)}+I(Q_n,G_n)\not \in {\cal F}(x_n) \pl X_n\pl_{{\cal F}}.
\end{eqnarray*}
Thus,
\begin{eqnarray*}
P(\mid \sqrt{n}(\psi_n-\psi_0)\mid >x)&\leq& P(\mid N_{0n}\mid+\pl X_n\pl_{{\cal F}(x_n)}B(Q_n,G_n)+\pl X_n\pl_{\cal F}(1-B(Q_n,G_n)>x)\\
&=& P(\mid N_{0n}\mid+\pl X_n\pl_{{\cal F}(x_n)}>x,B(Q_n,G_n)=1)\\
&&+ P(\mid N_{0n}\mid++\pl X_n\pl_{\cal F}>x,B(Q_n,G_n)=0)\\
&\leq&P(\mid N_{0n}\mid+\pl X_n\pl_{{\cal F}(x_n)}>x,B(Q_n,G_n)=1)+ \alpha_n \\
&\leq& P(\mid N_{0n}\mid+\pl X_n\pl_{{\cal F}(x_n)}>x)+ \alpha_n \\
\end{eqnarray*}
Similarly,
\begin{eqnarray*}
P(\sigma_n^{-1}\mid \sqrt{n}(\psi_n-\psi_0)\mid >x)&\leq& P(\mid \sigma_n^{-1}N_{0n}\mid+\sigma_n^{-1}\pl X_n\pl_{{\cal F}(x_n)}B(Q_n,G_n)+\sigma_n^{-1}\pl X_n\pl_{\cal F}(1-B(Q_n,G_n)>x)\\
&=& P(\mid \sigma_n^{-1}N_{0n}\mid+\sigma_n^{-1}\pl X_n\pl_{{\cal F}(x_n)}>x,B(Q_n,G_n)=1)\\
&&+ P(\mid \sigma_n^{-1}N_{0n}\mid+\sigma_n^{-1}\pl X_n\pl_{\cal F}>x,B(Q_n,G_n)=0)\\
&\leq&P(\mid \sigma_n^{-1}N_{0n}\mid+\sigma_n^{-1} \pl X_n\pl_{{\cal F}(x_n)}>x,B(Q_n,G_n)=1)+ \alpha_n \\
&\leq& P(\mid \sigma_n^{-1}N_{0n}\mid+\sigma_n^{-1}\pl X_n\pl_{{\cal F}(x_n)}>x)+ \alpha_n \\
.
\end{eqnarray*}
For a given $x_n=x_0$, we have
\[
P(\mid \sigma_n^{-1}N_{0n}\mid+\sigma_n^{-1}\pl X_n\pl_{{\cal F}(x_0)}>x)\rightarrow P(\mid \sigma_0^{-1}N_0\mid +\sigma_0^{-1}\pl X_0\pl_{{\cal F}(x_0)}>x),
\]
or more generally,
\[\mid \sigma_n^{-1}N_{0n}\mid+\sigma_n^{-1}\pl X_n\pl_{{\cal F}(x_0)}\Rightarrow_d  \mid \sigma_0^{-1}N_0\mid +\sigma_0^{-1}\pl X_0\pl_{{\cal F}(x_0)} .\]
We can consistently estimate the limit distribution on the right-hand side. Let $S_{x_0}(\cdot)$ be the survivor function of \sigma_0^{-1}N_0\mid +\sigma_0^{-1}\pl X_0\pl_{{\cal F}(x_0)$.
Let $S_{x_0,n}$ be a consistent estimator of this survivor function. We estimate $P(\mid \sigma_n^{-1}N_{0n}\mid+\sigma_n^{-1}\pl X_n\pl_{{\cal F}(x_n)}>x)$
with $S_{x_n,n}(x)$.
Let $q_{0.95,n}$ be defined by
\[
S_{x_n,n}(q_{0.95,n})= 0.05-\alpha_n .\]
The higher order $0.95$-confidence interval is given by
\[
\psi_n\pm q_{0.95,n}\sigma_n/n^{1/2} .\]
By the asymptotic equicontinuity of $X_n$, we have  $\pl X_n\pl_{{\cal F}(x_n)}\rightarrow_p 0$. As a consequence,
\[
 P(\mid \sigma_n^{-1}N_{0n}\mid+\sigma_n^{-1}\pl X_n\pl_{{\cal F}(x_n)}>x)+ \alpha_n \rightarrow P(N(0,1)>x) .\]
 Therefore, $q_{0.95,n}\rightarrow 1.96$ converges to the $0.975$-quantile of the standard normal distribution.
 Thus our higher order confidence interval converges to the Wald-type confidence interval $\psi_n\pm 1.96\sigma_0/n^{1/2}$.

What is overall logic? Firstly, we write $\psi_n-\psi_0$ as the first order empirical mean that converges to optimal normal limit distribution plus a remainder.
This remainder equals the empirical process at $D^*(Q_n,G_n)-D^(Q_0,G_0)$ and the typical second-order term.
The second-order term is bounded with Cauchy-Schwarz in terms of $L^2(P_0)$-norms of $Q_n-Q_0$ and $G_n-G_0$ using strong positivity assumption.
Then, using that our estimators $Q_n,G_n$ are HAL-MLEs these $L^2$-norms are upper bounded by an empirical process at $L_1(Q_n)-L_1(Q_0)$ and $L_2(G_n)-L_2(G_0)$, resulting  in showing that the remainder is dominated by   $X_n(Q_n,G_n)-X_n(Q_0,G_0)$ for a stochastic process, where $X_n$ is a simple function of three empirical processes at $D^*(Q,G)-D^*(Q_0,G_0)$, $L_1(Q)-L_1(Q_0)$ and $L_2(G)-L_2(G_0)$. In other words, $X_n(f)$, $f\in {\cal F}$.
In this way we dominate the standardized estimator $\sqrt{n}(\psi_n-\psi_0)/\sigma_n$ with $\mid N_{0,n}\mid +\mid X_n(Q_n,G_n)-X_n(Q_0,G_0)\mid$.
We easily obtain asymptotic equicontinuity of the process $(X_n(f):f\in {\cal F})$ w.r.t $L^2(P_0)$-sum norm for $Q_n-Q_0$ and $G_n-G_0$, where ${\cal F}$ represents the parameter space of $(Q,G)$, thereby weak convergence of $X_n$ as well to a limit process $X_0$    (simple function of three Gaussian processes, correlated and we know how).
We now focus on establishing a tail probability for $\pl Q_n-Q_0\pl_{P_0}^2 $ and $\pl G_n-G_0\pl_{P_0}^2$.
We do this by using again that we can bound these by the empirical process applied to $L_1(Q_n)-L_1(Q_0)$ and $L_2(G_n)-L_2(G_0)$.
We now use our integration by parts formula to bound these by a supremum norm of empirical process indexed by simple indicators times the sectional variation norm of $L_1(Q_n)-L_1(Q_0)$ and $L_2(G_n)-L_2(G_0)$. The latter variation norms are bounded in terms of $M_1$ and $M_2$ by sectional variation norms of $Q,G$.
So now we have dominated the $L^2$-norms by a constant times the supremum norm of empirical process of indicators. We can estimate the survivor function of the supremum norm of empirical process indexed by indicators consistently. So we now have an upper bound of survivor probability of $L^2(P_0)$-norms of $Q_n-Q_0$ and $G_n-G_0$.We can use this to set a cut-off $x_{1n}$, $x_{2n}$ so that the probability that both are smaller than these cut-offs is larger than $1-\alpha_n$ for an $\alpha_n$ that converges to zero, user supplied parameter. The user could optimize this choice to minimize resulting width of confidence interval.
So we would even define the confidence interval in that way, to do. This result allows us now to bound the tail probability of $\mid N_{0n}\mid +\mid X_n(Q_n,G_n)-X_n(Q_0,G_0)\mid$ in terms of supremum of $X_n(f)$ over $f\in {\cal F}(x_n)$, where ${\cal F}(x_n)$ is set of $(Q,G)$ less than $x_n$ away from their true counterparts.
For the given $x_n$ we now estimate this tail probability, which we can do consistently, by weak convergence of all these suprema.
We now select the $0.95$-quantile $q_{0.95,n}$ of that distribution which gives us the confidence interval.Note $q_{0.95,n}(x_n)$ depends on $x_n$ so we can minimize it over this choice. Our confidence interval corresponds with a conservative finite sample confidence interval if we use the actual finite sample distribution of the supreme in the bound. We know that these supreme converge in distribution so our estimator will be consistent, not necessarily from below or above. So one clearly expects by estimating such  a conservative bound on the remainder while only relying on asymptotics for these conservative bound process which converges in distribution which could go either way. Therefore we expect finite sample coverage at minimal at 0.95. Nonetheless, asymptotically we converge to asymptotic optimal Gaussian confidence interval from above.
This is a valid confidence interval for HAL-TMLE. When one uses SL-HAL-TMLE then this should still be valid since by oracle inequality the upper bound of remainder in terms of $L^2$-norms only gets better, once again making us conservative.
The supremum of the empirical process indexed by indicators can be nicely estimated.
Then there is the supremum of $X_n(Q,G)-X_n(Q_0,G_0)$. This depends on $(Q_0,G_0)$. So it is an unknown supremum. So  we replace $Q_0,G_0$ by $Q_n,G_n$.
The sets ${\cal F}(x_n)$ are now a set of $(Q,G)$ not more than $x_n$ apart in $L^2$-norms of $(Q_n,G_n)$.

We also have some results for the bounds that they converges as $\sqrt{d}M$ which are just of theoretical interest showing how the remainder can get large relative to
$N_{0n}$ potentially as $d$ increases. The reward for sparsity is that $\pl Q_0\pl_v^*$ is smaller than one would think, making $M$ smaller than one would think based on $d$. Note $M=M(d)$ normally and will increase potentially very fast as function of $d$ $2^d$ if there is no sparsity at all. So one can see the curse of dimensionality kicking but we let CV select $M$ so that we can be adaptive to sparsity.

This is all very cool.

We see that this confidence interval will be hurt by large sectional variation norm. Suppose that we use CV-TMLE. Then one of the terms in $X_n$ will be fine, just empirical mean of iid random variables. But we still have the remainder and the rate of $Q_n-Q_0$ is still driven by $M$. So not that much difference.

Our method can be generalized since we can always bound remainder by CS by $L^2$-norms using strong positivity. So this is a completely general approach!
We should write a section on that in the paper. Or may be do general first and then use this as example.

We can discuss targeted bootstrap as a less conservative approach still taking into account higher order remainder, but it would not be conservative.
However, it would nicely respect that we use a substitution estimator, which is important and helps immensely in finite samples.
So we should probably add a targeted bootstrap section as well as a counter.
By the way, can we not build in upper bounds that also use global constants from the model and being substitution estimator to guarantee that our confidence interval respect what we know are global bounds.

What appears to be nice is that we make our complete bound a function of $Q,G$, making it at least respect a lot of structure of our true bound.
By when we do bounds of e.g. $L^2$-norms in terms of empirical process we should always max by maximal possible value of $\pl Q_n-Q_0\pl_{P_0}$ and $\pl G_n-G_0\pl_{P_0}$. In addition, if we have $\pl Q-Q_0\pl_{P_0}<x_{1n}$ we should make sure that $x_{1n}$ is maxed by maximal possible value.

If we have chosen $x_{1n}$ $x_{2n}$ w.r.t. $\alpha_{1n}$, $\alpha_{2n}$, then these imply bounds on $R_{2n}$ and also on empirical process of $D*(Q_n,G_n)-D^*(Q_0,G_0)$ since it puts bound on $L^2$ norm of  this $f_n$, so could simulate. Why is this not better?
I think because now we are getting a rate for $Q_n-Q_0$ and $G_n-G_0$ $n^{-1/4}$ or even slightly worse so that would end up with remainder $n^{-1/2}$.
While using empirical process makes it go to zero!
So it is better, but once again this bound could be used as a max to make sure we keep respecting the global bounds asa much as possible!!





The other stuff with aiming to optimize the second-order remainder is another topic,, e.g using C-TMLE for $G_n$ and other advances to optimize the TMLE can still be done but the above would still be the inference as if we used HAL-TMLE with $M$ selected with CV.





% We should also recommend a targeted bootstrap, proving it works asymptotically using HAL-SL.
% Seems we could even get finite sample inference if we can get an exact tail probability for empirical process indexed by Donsker class.







\end{document}

\section{Introduction}
We consider $O=(W,A,Y)\sim P_0\in {\cal M}$, where ${\cal M}$ is a nonparametric model.
Let $\Psi:{\cal M}\rightarrow\openr$ be defined by $\Psi(P)=E_PE_P(Y\mid A=1,W)$.
The canonical gradient is given by:
\[
D^*(Q,G)=D^*(\bar{Q},G)-\Psi(Q),\]
where
\[
D^*(\bar{Q},G)=\frac{A}{\bar{G}(W)}(Y-\bar{Q}(W))+\bar{Q}(W) .\]
We have
\[
\Psi(Q)-\Psi(Q_0)=-P_0 D^*(Q,G)+R_{20}(\bar{Q},\bar{Q}_0,\bar{G},\bar{G}_0),\]
where
\[
R_{20}(\bar{Q},\bar{Q}_0,\bar{G},\bar{G}_0)=\int (\bar{Q}(w)-\bar{Q}_0(w))\frac{(\bar{G}(w)-\bar{G}_0(w))}{\bar{G}(w)} dP_0(w). \]
We assume the strong positivity assumption $\bar{G}_0>\delta>0$.

We want to construct a TMLE that has a best rate of convergence for its second-order remainder.  A TMLE $\Psi(P_n^*)$ solving $P_n D^*(P_n^*)=0$ yields the expansion $\Psi(P_n^*)-\Psi(P_0)=(P_n-P_0)D^*(P_n^*)+R_{20}(P_n^*,P_0)$ which means that it has as remainder relative to a sample mean of mean zero random variables,  $(P_n-P_0)D^*(P_0)$,
$(P_n-P_0)(D^*(P_n^*)-D^*(P_0))+R_{20}(P_n^*,P_0)$. A CV-TMLE based on $V$-fold cross-validation defined by a random split $B\in \{0,1\}^n $ into training and validation sample yields an expansion:
\[
E_B\Psi({\bf P}_{n,B}^*)-\Psi(P_0)=E_B (P_{n,B}^1-P_0)D^*({\bf P}_{n,B}^*)+E_B R_{20}({\bf P}_{n,B}^*,P_0),\]
where ${\bf P}_{n,B}^*$ is the TMLE using as initial estimator ${\bf P}_{n,B}^0$ based on training sample $\{O_i:B(i)=0\}$ while targeting the estimator based on validation sample $\{O_i:B(i)=1\}$. The leading term is up till an $\epsilon_n$ fitting a sum of mean zero  independent random variables converging to a normal distribution as long as the variance of $D^*({\bf P}_{n,B}^*)$ converges to the variance of $D^*(P_0)$.  Therefore the only essential remainder  is now $E_B R_{20}({\bf P}_{n,B}^*,P_0)$.
Therefore we will focus on a CV-TMLE procedure, but we make another modification by requiring that $\bar{G}_0$ and $\bar{Q}_0$ are estimated on independent samples, giving the second-order remainder a particularly nice structure when $R_{20}$ has the double robust structure as in our example.

Let $B\in\{1,2,3\}^n$ be  a random variable, where $P(B=1)=1/V$, $P(B=2)=P(B=3)=1/2(V-1)/V$, represent a random  split of the sample $\{O_1,\ldots,O_n\}$ into
3 samples $\{O_i:B(i)=1\}$, $\{O_i:B(i)=2\}$ and $\{O_i:B(i)=3\}$. For simplicity, we will use a $V$-fold splitting, where we first split sample in $V$-subgroups, assign $B(i)=1$ to one of the $V$-subgroups, and divide the remaining $V-1$-subgroups in 2 equal samples that we assign $B(i)=2$ and $B(i)=3$ respectively. This then defines $V$ splits $B_n$. For notational convenience, we will suppress the dependence of $B$ on  $n$.
For a particular split $B$, we will refer to these three subsamples as the targeting sample, $\bar{Q}$-sample and $\bar{G}$-sample respectively, and let $P_{n,B}^1$, $P_{n,B}^2$, $P_{n,B}^3$ be the three empirical probability measures of these 3 samples.
Let $\bar{Q}_{n,B}^2$ be an estimator of $\bar{Q}_0$ based on $P_{n,B}^2$, $\bar{G}_{n,B}^3$ be an estimator of $\bar{G}_0$ based on $P_{n,B}^3$.
Let $\mbox{Logit}\bar{Q}_{n,B,\epsilon}^2=\mbox{Logit}\bar{Q}_{n,B}^2+\epsilon H(\bar{G}_{n,B}^3)$ be the least favorable submodel through $\bar{Q}_{n,B}^2$ using $\bar{G}_{n,B}^3$ as estimator of $\bar{G}_0$ w.r.t log-likelihood loss $L(\bar{Q})$  and define $\epsilon_n=\epsilon_{n,B}^1=\arg\min_{\epsilon}P_{n,B}^1 L(\bar{Q}_{n,B,\epsilon}^2$ be the MLE based on the targeting sample $P_{n,B}^1$.
We do this for each of the $V$ splits $B$. Let $Q_{n,B}^{2*}=\bar{Q}^2_{n,B,\epsilon_n}$ and note that this estimator is based on both $P_{n,B}^1$ and $P_{n,B}^2$.
Let $\psi_n^*=E_B\Psi(Q_{W,n,B}^1,\bar{Q}_{n,B}^{2*})=E_B P_{n,B}^1 \bar{Q}_{n,B}^{2*}$ be the average of these $V$ TMLEs.
We have
\begin{eqnarray*}
\psi_n^*-\Psi(Q_0)&=&E_B (P_{n,B}^1-P_0)D^*(\bar{Q}_{n,B}^{2*},\bar{G}_{n,B}^3) \\
&&+ E_B R_{20}(\bar{Q}_{n,B}^{2*},\bar{Q}_0,\bar{G}_{n,B}^3-\bar{G}_0).
\end{eqnarray*}
By using HAL-SL for both estimators $\bar{G}_{n,B}^3 $ and $\bar{Q}_{n,B}^2$ we can bound the second-order remainder by $\delta^{-1}E_B \pl \bar{G}_{n,B}^3-\bar{G}_0\pl_{P_0}\pl \bar{Q}_{n,B}^*-\bar{Q}_0\pl_{P_0}$, where the latter is $o_P(n^{-1/2-\alpha(d)}$ for some $\alpha(d)>0$ with $\alpha(d)$ behaving as $1/d$.
We can split $R_{20}(\bar{Q},\bar{Q}_0,\bar{G},\bar{G}_0)=R_{20,a}(\bar{Q},\bar{Q}_0,\bar{G},\bar{G}_0)+R_{30}(\bar{Q},\bar{Q}_0,\bar{G},\bar{G}_0)$, where now
\[
R_{20,a}(\bar{Q},\bar{Q}_0,\bar{G}-\bar{G}_0)=\int (\bar{Q}-\bar{Q}_0)(\bar{G}-\bar{G}_0)/\bar{G}_0 dP_0\]
is a clean second-order remainder by being linear in the first order difference $\bar{G}-\bar{G}_0$, instead of also having $\bar{G}$ in the denominator.
Here $R_{30}$ is now a third order remainder that can be bounded by $\delta^{-2}E_B \pl \bar{G}_{n,B}^3-\bar{G}_0\pl_{P_0}^2\pl \bar{Q}_{n,B}^*-\bar{Q}_0\pl_{P_0}$ which is thus $O_P(n^{-3/4-\alpha}$ for some $\alpha>0$.Similarly, $R_{30}$ can be split up in a clean $R_{30,a}$ that is linear in $(\bar{G}-\bar{G}_0)^2$ (not $\bar{G}$ in a  denominator) and a  fourth order remainder, etc.
We will focus on the analysis of $R_{20,a}$.


Thus, we want to analyze:
\[
R_{2n}\equiv E_B \int (\bar{Q}_{n,B}^{2*}-\bar{Q}_0)(\bar{G}_{n,B}^3-\bar{G}_0)\bar{G}_0^{-1} dP_0 .\]
We already know that this is $o_P(n^{-1/2})$ but we hope to utilize the special double robust structure and the independence of $\bar{Q}_{n,B}^{2*}$ and $\bar{G}_{n,B}^3$
to obtain a better bound.
We can write $R_{2n}$ as a sum of four terms:
\begin{eqnarray*}
A&=&E_B \int (\bar{Q}_{n,B}^{2*}-E\bar{Q}_{n,B}^{2*}) (\bar{G}_{n,B}^3-E\bar{G}_{n,B}^3)\bar{G}_0^{-1} dP_0\\
B&=&E_B \int (\bar{Q}_{n,B}^{2*}-E\bar{Q}_{n,B}^{2*}) (E\bar{G}_{n,B}^3-\bar{G}_0) \bar{G}_0^{-1} dP_0\\
C&=&E_B \int (E\bar{Q}_{n,B}^{2*}- \bar{Q}_0)(\bar{G}_{n,B}^3-E\bar{G}_{n,B}^3)\bar{G}_0^{-1} dP_0\\
D&=&E_B \int (E\bar{Q}_{n,B}^{2*}- \bar{Q}_0)(E\bar{G}_{n,B}^3-\bar{G}_0)\bar{G}_0^{-1} dP_0\\
\end{eqnarray*}
Since $EA=EB=EC=0$, it follows that $ER_{2n}=D$ so that $D$ is the bias of $R_{2n}$.
Thus, $E(R_{2n}-ER_{2n})^2=E( A+B+C)^2$.
Note that $EAB=0$ by taking the conditional expectation of $\bar{G}_{n,B}^3$, given $\bar{Q}_{n,B}^{2*}$.
Also $EAC=0$ and $EBC=0$  by taking the conditional expectation of $\bar{Q}_{n,B}^{2*}$, given $\bar{G}_{n,B}^3$.
Thus, we have
\[
E(R_{2n}-ER_{2n})^2=EA^2+EB^2+EC^2.\]
Immediate and general bounds are obtained by Cauchy-Schwarz inequality:
\begin{eqnarray*}
EA^2&\leq & \delta^{-2} E_B\pl \bar{Q}_{n,B}^{2*}-E\bar{Q}_{n,B}^{2*}\pl_{P_0}^2 E_B \pl \bar{G}_{n,B}^3-E\bar{G}_{n,B}^3\pl_{P_0}\\
EB^2&\leq &\delta^{-2} E_B  \pl \bar{Q}_{n,B}^{2*}-E\bar{Q}_{n,B}^{2*}\pl_{P_0}^2E_B\pl E\bar{G}_{n,B}^3-\bar{G}_0)\pl_{P_0}^2 \\
EC^2&\leq &\delta^{-2} E_B \pl E\bar{Q}_{n,B}^{2*}- \bar{Q}_0\pl_{P_0}^2 E_B\pl \bar{G}_{n,B}^3-E\bar{G}_{n,B}^3\pl_{P_0}^2 \\
D^2&\leq &\delta^{-2}E_B \pl E\bar{Q}_{n,B}^{2*}- \bar{Q}_0\pl_{P_0}^2 E_B\pl E\bar{G}_{n,B}^3-\bar{G}_0\pl_{P_0}^2 \\
\end{eqnarray*}
Suppose that the estimators are indexed by a tuning parameter $\lambda$. Let
\begin{eqnarray*}
B_1^2(n,\lambda)^2&=&E_B \pl E\bar{Q}_{n,B}^{2*}- \bar{Q}_0\pl_{P_0}^2 \\
B_2^2(n,\lambda)^2&=& E_B\pl E\bar{G}_{n,B}^3-\bar{G}_0\pl_{P_0}^2\\
\sigma^2_1(n,\lambda)&=& E_B\pl \bar{Q}_{n,B}^{2*}-E\bar{Q}_{n,B}^{2*}\pl_{P_0}^2\\
\sigma^2_2(n,\lambda)&=& E_B \pl \bar{G}_{n,B}^3-E\bar{G}_{n,B}^3\pl_{P_0}.
\end{eqnarray*}
These are average bias squared and average variance terms for the two estimators of $\bar{Q}_0$ and $\bar{G}_0$, respectively.
Thus, we have
\begin{eqnarray*}
ER_{2n}^2&\leq& \delta^{-2}\sigma^2_1(n,\lambda)\sigma^2_2(n,\lambda)+\delta^{-2}\sigma^2_1(n,\lambda)B_2^2(n,\lambda)\\
&&+\delta^{-2}B_1^2(n,\lambda)\sigma^2_2(n,\lambda)+\delta^{-2}B_1^2(n,\lambda)B_2^2(n,\lambda) .
\end{eqnarray*}
What is an optimal $\lambda$ regarding trade-off of bias and variance for the two estimators for the purpose of minimizing this bound on $ER_{2n}^2$?
It will be of interest to understand if this general upper bound already implies a different trade-off than what cross-validation would achieve.

This upper bound does not utilize any specific structure of the estimators. Specifically, many nonparametric estimators use local data for local $W$-regions which means these estimators are independent across different partitioning elements of the $W$-space. This independence might heavily reduce the variance of the integral over $W$.
Therefore we also want to derive bounds for estimators that have special independence structure. Three types of estimators of interest from this perspective are
histogram regression, kernel regression and HAL-regression.

Let $\cup_j A_j$ be a partitioning of the $W$-space and let $Q_n=\sum_j I_{A_j}Q_{n,j}$, where $Q_{n,j}$ use only data in $A_j$ or we  could have martingale structure as with HAL, where $Q_{n,j}$, given previously computed estimators according to ordering, is independent based on data in $A_j$ only. In other words, $
Q_{n,j}=Q_{n,j}^-+\tilde{Q}_{n,j}$. Same for $G_n=\sum_j I_{A_j}G_{n,j}$.
We can write $R_{2n}$ as a sum of four terms:
\begin{eqnarray*}
A&=&E_B\sum_j \int_{A_j} (\bar{Q}_{n,B,j}^{2*}-E\bar{Q}_{n,B,j}^{2*}) (\bar{G}_{n,B,j}^3-E\bar{G}_{n,B,j}^3)\bar{G}_0^{-1} dP_0\\
B&=&E_B \sum_j \int_{A_j} (\bar{Q}_{n,B,j}^{2*}-E\bar{Q}_{n,B,j}^{2*}) (E\bar{G}_{n,B,j}^3-\bar{G}_0) \bar{G}_0^{-1} dP_0\\
C&=&E_B \sum_j \int_{A_j} (E\bar{Q}_{n,B,j}^{2*}- \bar{Q}_0)(\bar{G}_{n,B,j}^3-E\bar{G}_{n,B,j}^3)\bar{G}_0^{-1} dP_0\\
D&=&E_B \int (E\bar{Q}_{n,B}^{2*}- \bar{Q}_0)(E\bar{G}_{n,B}^3-\bar{G}_0)\bar{G}_0^{-1} dP_0\\
\end{eqnarray*}
By same argument as above,  we still have
\[
E(R_{2n}-ER_{2n})^2=EA^2+EB^2+EC^2.\]
Note that $A=E_B A(B)$ and same for $B$ and $C$.
Let's focus on understanding the variance of $A(b)$ for each $B=b$, even though  the variance $EA^2$ also involves all covariances. But we can bound these by variances as well.
Notice that $A(b)=\sum_j X_{j,n}$ where $X_{j,n}$ are independent random variables. Or in HAL-case, $A(b)=M(N)\equiv \sum_{j=1}^N M_j$, where $E(M_j\mid {\cal F}(j-1))=0$ so that $A(b)$ is a discrete martingale. $M_j$ has the difference $Q_{n,j}-E(Q_{n,j}\mid {\cal F}(j-1))$ times a bias term, or with $Q_{n,j}$ replaced by $G_{n,j}$.
We can estimate the variance of $M(N)$ as the expectation of the sum of conditional variances. This gives then same type bound as we have below.
Thus, variance of $A(b)=\sum_j EX_{j,n}^2$.
This gives us bounds:
\begin{eqnarray*}
EA^2(b)&=&\sum_j E\left( \int_{A_j} (\bar{Q}_{n,b,j}^{2*}-E\bar{Q}_{n,b,j}^{2*}) (\bar{G}_{n,b,j}^3-E\bar{G}_{n,b,j}^3)\bar{G}_0^{-1} dP_0\right)^2\\
EB^2(b)&=&\sum_j E\left( \int_{A_j} (\bar{Q}_{n,b,j}^{2*}-E\bar{Q}_{n,b,j}^{2*}) (E\bar{G}_{n,b,j}^3-\bar{G}_0) \bar{G}_0^{-1} dP_0\right)^2\\
EC^2(b)&=&\sum_j E\left( \int_{A_j} (E\bar{Q}_{n,b,j}^{2*}- \bar{Q}_0)(\bar{G}_{n,b,j}^3-E\bar{G}_{n,b,j}^3)\bar{G}_0^{-1} dP_0\right)^2 .
%D&=&E_B \int (E\bar{Q}_{n,B}^{2*}- \bar{Q}_0)(E\bar{G}_{n,B}^3-\bar{G}_0)\bar{G}_0^{-1} dP_0\\
\end{eqnarray*}
We can also write down the Martingale variance formula but where expectations are conditional expectation given history and we have a final expectation outside.
In that case the conditional variances are just conditional variances of $\tilde{Q}_{n,j}$ based on data in $A_j$ only.
The fact that each term involves a cross-product of differences is actually nice since there might be a lot of cancelation occurring in these integrals over $A_j$ before it gets squared. In addition, we also still have independence within these integrals of the $Q$ and $G$-estimator for term $A$, while the other terms have only one random factor times a bias.
Nonetheless, we can use Cauchy-Schwarz again to obtain the following upper bounds:
\begin{eqnarray*}
EA^2(b)&\leq & \delta^{-2} \sum_j E \pl \bar{Q}_{n,b,j}^{2*}-E\bar{Q}_{n,b,j}^{2*}\pl_{P_0,A_j}^2 E \pl \bar{G}_{n,b,j}^3-E\bar{G}_{n,b,j}^3\pl_{P_0,A_j}\\
EB^2(b)&\leq &\delta^{-2} \sum_j  E \pl \bar{Q}_{n,b,j}^{2*}-E\bar{Q}_{n,b,j}^{2*}\pl_{P_0,A_j}^2 \pl E\bar{G}_{n,b,j}^3-\bar{G}_0)\pl_{P_0,A_j}^2 \\
EC^2(b)&\leq &\delta^{-2} \sum_j   \pl E\bar{Q}_{n,b,j}^{2*}- \bar{Q}_0\pl_{P_0,A_j}^2 E\pl \bar{G}_{n,b,j}^3-E\bar{G}_{n,b,j}^3\pl_{P_0,A_j}^2 \\
%D^2&\leq &\delta^{-2}E_B \pl E\bar{Q}_{n,B}^{2*}- \bar{Q}_0\pl_{P_0}^2 E_B\pl E\bar{G}_{n,B}^3-\bar{G}_0\pl_{P_0}^2 \\
\end{eqnarray*}
This will be a significantly better bound than the above bound. We have results for these local $L^2$-norm for HAL. These are results for $P_0(A_j)^{-1}\pl\cdot\pl_{P_0,A_j}^2$, therefore we can pull out $P_0(A_j)^2$ within each sum giving $\sum_j P_0(A_j)^2\ldots$. These bounds should still have $\lambda$ in it. In HAL I believe we get
$M_j/P_0(A_j) n^{-1/2}$ where $M_j=M_j(\lambda)$. We could define $M_j(\lambda)$ as proportional to sample size in $A_j$ so that all these $j$-specific variation norm constraints are defined by a single $\lambda$.
At this point we can define \begin{eqnarray*}
B_1^2(n,b,j,\lambda)^2&=& \pl E\bar{Q}_{n,b,j}^{2*}- \bar{Q}_0\pl_{P_0,A_j}^2 \\
B_2^2(n,b,j,\lambda)^2&=& \pl E\bar{G}_{n,b,j}^3-\bar{G}_0\pl_{P_0,A_j}^2\\
\sigma^2_1(n,b,j,\lambda)&=& E\pl \bar{Q}_{n,b,j}^{2*}-E\bar{Q}_{n,b,j}^{2*}\pl_{P_0,A_j}^2\\
\sigma^2_2(n,b,j,\lambda)&=&  E\pl \bar{G}_{n,b,j}^3-E\bar{G}_{n,b,j}^3\pl_{P_0,A_j}.
\end{eqnarray*}
These bounds will not depend on $b$ and the dependence on $j$ will be driven by $P_0(A_j)$ (e.g., $h^d$) and $N=O( P_0(A_j)^{-1})$ (e.g., $h^{-d}$).
We can now express
\begin{eqnarray*}
ER_{2n}^2&\leq& \delta^{-2}\sum_j \sigma^2_1(n,j,\lambda)\sigma^2_2(n,j,\lambda)+\delta^{-2}\sum_j\sigma^2_1(n,j,\lambda)B_2^2(n,j,\lambda)\\
&&+\delta^{-2}\sum_j B_1^2(n,j,\lambda)\sigma^2_2(n,j,\lambda)+\delta^{-2}\sum_j B_1^2(n,\lambda)B_2^2(n,\lambda) .
\end{eqnarray*}
Let's now optimize this w.r.t. $\lambda $ and choice of partitioning with $h$. For histogram $\lambda=h$, but for local ordered HAL we have both $h$ and $\lambda$.
For HAL we do not know how bias depends on $\lambda$, so we could do an example of assumed relation.




We have $ER_{2n}^2=E(R_{2n}-ER_{2n})^2+ E^2R_{2n}$, where the first is the variance of $R_{2n}$ and second is the square of the ''bias'' of $R_{2n}$ as an estimator of $0$. So to understand the rate of $R_{2n}$ we need to bound the variance and bias term.

Consider the case that $\bar{Q}_{n,B}^2$ and $\bar{G}_{n,B}^3$ are indexed by a  tuning parameter $\lambda$ such as the penalty of Lasso, where bias is increasing in $\lambda$ and variance is decreasing in $\lambda$. To optimize the rate of convergence for $ER_{2n}(\lambda)^2$ we need to understand the bias and variance term and determine an optimal trade-off of them w.r.t $\lambda$. Might want to use a representation $\sum_j \tilde{\psi}_j$ each one conditionally on previous based on independent sample. So martingale structure in $j$. This is what we dan use for analyzing HAL. We could start with histogram and kernel to determine what happens there regarding optimal bandwidth.

so work out optimal width for histogram.
work out optimal width for kernel.
then get into localized HAL, where now tuning is $M_j$ all parametrized by proportion f observations in $A_j$, so still a common lambda controlling all $M_j=\lambda P_n (A_j)$. This hal is not histogram since it use within each $A_j$ an actual HAL to fit $\psi_{0j}$ using offset. The martingale independence should help us with understanding the variance of $R_{2n}$. Will be important to understand what happens to variance when $\lambda$ converges with sample size to infinity.
\end{document}



\subsection{HAL-MLE preserves rate of convergence on nonparametric bootstrap sample} %after this we should be able to easily finish consistency of np bootstrap. also add subsection talking about incorporating random selection of M_n with CV (removing ties) in this bootstrap so that initial estimator of Q and G also included selection of bounds M on sectional variation norm. HAL.
\begin{lemma}\labe{generalhalmle}
We have
\begin{eqnarray*}
0&\leq & d_{n1}(Q_n^{\#},Q_n)\equiv P_n\{ L_1(Q_n^{\#})-L_1(Q_n)\}\\
&=& -(P_n^{\#}-P_n)\{L_1(Q_n^{\#})-L_1(Q_n)\}+P_n^{\#}\{L_1(Q_n^{\#})-L_1(Q_n)\}\\
&\leq& -(P_n^{\#}-P_n)\{L_1(Q_n^{\#})-L_1(Q_n)\},
\end{eqnarray*}
and similarly $d_{n2}(G_n^{\#},G_n)\leq -(P_n^{\#}-P_n)L_2(G_n^{\#},G_n)$.
As a consequence, we have $d_{n1}(Q_n^{\#},Q_n)=P_n L_1(Q_n^{\#})-P_nL_1(Q_n)=O_P(n^{-1/2})$.
 and $d_{n2}(G_n^{\#},G_n)=P_n L_2(G_n^{\#})-P_nL_2(G_n)$ are both $O_P(n^{-1/2})$.
In addition, since $L_1(Q_n^{\#})-L_1(Q_n)$ falls in a uniform Donsker class with probability 1 so that the empirical process is asymptotically equicontinuous, we have that if  $d_{n1}(Q_n^{\#},Q_n)\rightarrow 0$ and $d_{n2}(G_n^{\#},G_n)\rightarrow 0$ implies that $P_n \{L_1(Q_n^{\#})-L_1(Q_n)\}^2\rightarrow 0$ and $P_n \{L_2(G_n^{\#})-L_2(G_n)\}^2\rightarrow 0$,
then we have $d_{n1}(Q_n^{\#},Q_n)=o_P(n^{-1/2})$ and $d_{n2}(G_n^{\#},G_n)=o_P(n^{-1/2})$.
If these dissimilarities are equivalent in the sense that  $\pl L_1(Q_n^{\#})-L_1(Q_n)\pl_{P_n}^2\lesssim d_{n1}(Q_n^{\#},Q_n)$, then we have
$d_{n1}(Q_n^{\#},Q_n)=O_P(n^{-1/2-\alpha(d)})$ and similarly for $G_n^{\#}$.
\end{lemma}

The above lemma is completely general and demonstrates the HAL-MLE  on a bootstrap sample is still consistent at a same rate as the original HAL-MLE on the original data, but it is now w.r.t. the loss-based dissimilarity $d_{n1}(Q_n^{\#},Q_n)$. The question is if this type of $d_{n1}$ and $d_{n2}$-consistency of $Q_n^{\#}$  and $G_n^{\#}$ w.r.t. $Q_n$ and $G_n$ is such that the sampling distribution of the bootstrapped remainder $\tilde{R}_{2n}(Q_n^{\#},Q_n,G_n^{\#},G_n)$, conditional on $P_n$, provides a reasonable estimator of the sampling distribution of the remainder $\tilde{R}_{2n}(Q_n,Q_0,G_n,G_0)$ of the actual HAL-TMLE $\Psi(Q_n^*)$.
In order to derive some concrete results we focus now on the case that the parameter spaces for $Q$ and $G$ are nonparametric sets of cadlag functions with a uniformly bounded sectional variation norm.
So $Q_n=\arg\min_{Q\in D[0,\tau_1],\pl Q\pl_v^*<M_1}P_n L_1(Q)$ and $Q_n^{\#}=\arg\min_{Q\in D[0,\tau_1],\pl Q\pl_v^*<M_1}P_n^{\#}L_1(Q)$ and similarly $G_n=\arg\min_{G\in D[0,\tau_2],\pl G\pl_v^*<M_2}P_n L_2(G)$ and $G_n^{\#}=\arg\min_{G\in D[0,\tau_1],\pl G\pl_v^*<M_2}P_n^{\#}L_2(G)$.

We will prove the following lemma.
\begin{lemma}\label{bootstrapHALMLEstructure}
Suppose that $L_1(Q)(O)=(Y-Q(X))^2$ is the squared error loss. Then,
we have
\[
0\leq d_{n1}(Q_n^{\#},Q_n)\geq P_n (Q_n^{\#}-Q_n)^2 .\]
In particular, $P_n  \{L_1(Q_n^{\#})-L_1(Q_n)\}^2\lessim P_n \{L_1(Q_n^{\#})-L_1(Q_n)\}$ and thereby
\[
d_{n1}(Q_n^{\#},Q_n)=O_P(n^{-1/2-\alpha(d)}),
\]
and thus also $P_n (Q_n^{\#}-Q_n)^2=O_P(n^{-1/2-\alpha(d)})$.

For general loss, consider the following assumptions. Suppose that $L_1(Q)$ is differentiable at $Q=Q_n$ so that
\[
P_n \{L_1(Q_n^{\#})-L_1(Q_n)\}=P_n \frac{d}{dQ_n}L_1(Q_n)(Q_n^{\#}-Q_n)+R_{2n}(Q_n^{\#},Q_n)\]
for some second-order remainder involving square differences between $Q_n^{\#}$ and $Q_n$. We have $P_n\frac{d}{dQ_n}L_1(Q_n)(Q_n^{\#}-Q_n)\geq 0$ so that
\[
0\leq P_n\{L_1(Q_n^{\#})-L_1(Q_n)\}\geq R_{2n}(Q_n^{\#},Q_n).\]
Suppose that \[
P_n \{L_1(Q_n^{\#})-L_1(Q_n)\}^2\lesssim R_{2n}(Q_n^{\#},Q_n).\]
Then,
\[
P_n \{L_1(Q_n^{\#})-L_1(Q_n)\}^2\lesssim P_n\{L_1(Q_n^{\#})-L_1(Q_n)\},\]
and thus
\[
0\leq d_{n1}(Q_n^{\#},Q_n)=O_P(n^{-1/2-\alpha(d)}),\]
and thus also $R_{2n}(Q_n^{\#},Q_n)=O_P(n^{-1/2-\alpha(d)})$.
\end{lemma}
{\bf Proof:}
We first prove the results for the general loss function, and subsequently, we will consider the special case that $L_1(Q)$ is the squared error loss.
Consider a path $Q_{n,\epsilon}(x)=(1+\epsilon h(0))Q_n(0)+\sum_s \int_{(0_s,x_s]}(1+\epsilon h_s(u_s)) dQ_{n,s}(u_s))$, where $r(h,Q_n)\equiv  h(0)Q_n(0)+\sum_s \int_{(0_s,\tau_s]} h_s(u_s)\mid dQ_{n,s}(u_s)\mid \leq 0$ and $h$ is uniformly bounded. Let ${\cal H}$ be the set of $h$ functions (i.e., functions of $s,u_s$).
Note that  for $\epsilon\geq 0$, we have
\begin{eqnarray*}
\pl Q_{n,\epsilon}\pl_v^*&=&(1+\epsilon h(0))\mid Q_n(0))+\sum_s \int_{(0_s,\tau_s]}(1+\epsilon h_s(u_s))\mid dQ_{n,s}(u_s)\mid \\
&=& \pl Q_n\pl_v^*+\epsilon\left\{ h(0)Q_n(0)+\sum_s \int_{(0_s,\tau_s]}h_s(u_s) \mid dQ_{n,s}(u_s)\mid \\
&\geq & \pl Q_n\pl_v^*,
\end{eqnarray*}
by assumption on $h$.
Thus, this represents a path of cadlag functions with sectional variation norm is smaller equal than $M=\pl Q_n\pl_v^*$.
We also have that
 \[
 Q_{n,\epsilon}-Q_n=\epsilon\left\{ Q_n(0)h(0)+ \sum_s \int_{(0_s,x_s]} h_s(u_s)dQ_{n,s}(u_s))\right\} .\]
 Thus,
 \[
 \frac{d}{d\epsilon}Q_{n,\epsilon}=f(h,Q_n)\equiv Q_n(0)h(0)+ \sum_s \int_{(0_s,x_s]} h_s(u_s)dQ_{n,s}(u_s)) .\]
 %Note that $f(h,Q_n)$ represents a difference of two cadlag functions.
 Let ${\cal S}\equiv \{f(h,Q_n): h\in {\cal H}\}$.
 By definition of the MLE $Q_n$, we also have that $\epsilon \rightarrow P_n L_1(Q_{n,\epsilon})$ is minimal over $[0,\delta)$ at $\epsilon =0$.
This shows that the right-derivative $\frac{d}{d\epsilon+ }P_n L_1(Q_{n,\epsilon })\geq 0$ at $\epsilon =0$ and thus for each $h\in {\cal H}$, we have
\[
P_n \frac{d}{dQ_n}L_1(Q_n)(f(h,Q_n)) \geq 0 .\]
Suppose that
\begin{equation}\label{keya1}
Q_n^{\#}-Q_n\in {\cal S}=\{f(h,Q_n):h\in {\cal H}\}.\end{equation}
Then, we have
\[
P_n \frac{d}{dQ_n}L_1(Q_n)(Q_n^\#}-Q_n)\geq 0.\]
Combined with the assumed differentiability of $P_n L_1(Q)$ at $Q=Q_n$ with second-order remainder $R_{2n}(Q_n^{\#},Q_n)$, this proves
%\[P_n \{L_1(Q_n^{\#})-L_1(Q_n)\}=P_n \frac{d}{dQ_n}L_1(Q_n)(Q_n^{\#}-Q_n)+R_2(Q_n^{\#},Q_n)\]for some second-order remainder involving square differences between $Q_n^{\#}$ and $Q_n$. Then,
\[
0\leq P_n\{L_1(Q_n^{\#})-L_1(Q_n)\}\geq R_{2n}(Q_n^{\#},Q_n).\]
Thus it remains to show (\ref{keya1}).


% Since $\pl Q_n^\#}\pl_v^*=\pl Q_n\pl_v^*=M$ will both achieve the maximal allowed variation norm, and  $Q_{n,s}^{\#}\ll Q_{n,s}$ for all subset $s$ (i.e., the support of $Q_{n,s}^{\#}$ is a subset of the support of $Q_{n,s}$ due to the support of $P_n^{\#}$ being  a subset of support of $P_n$), one would generally expect that indeed this difference $Q_n^{\#}-Q_n$ is included in ${\cal S}$.
In order to prove (\ref{keya1}), let's solve explicitly for $h$ so that $Q_n^{\#}-Q_n=f(h,Q_n)$.
We have
\begin{eqnarray*}
Q_n^{\#}-Q_n&=&Q_n^{\#}(0)-Q_n(0)+\sum_s\int_{(0_s,x_s]} d(Q_{n,s}^{\#}-dQ_{n,s})(u_s)\\
&=& Q_n^{\#}(0)-Q_n(0)+\sum_s \int_{(0_s,x_s]} \frac{d(Q_{n,s}^{\#}-dQ_{n,s})}{dQ_{n,s}} dQ_{n,s}(u_s),
\end{eqnarray*}
where we used that $Q_{n,s}^{\#}\ll Q_{n,s}$ for each subset $s$.
Define for each $s$
\begin{eqnarray*}
h(Q_n^{\#},Q_n)(0)&=&(Q_n^{\#}(0)-Q_n(0))/Q_n(0)\\
h_s(Q_n^{\#},Q_n)&=&\frac{d(Q_{n,s}^{\#}-dQ_{n,s})}{dQ_{n,s}} .
\end{eqnarray*}
For this choice $h(Q_n^{\#},Q_n)$, we have $f(h,Q_n)=Q_n^{\#}-Q_n$.
Let's now check if we have that for this choice of $h$ $r(h,Q_n)\leq 0$.
We have
\begin{eqnarray*}
r(h,Q_n)&=&Q_n^{\#}(0)-Q_n(0)+\int_{(0_s,\tau_s]}\frac{dQ_{n,s}^{\#}-dQ_{n,s}}{dQ_{n,s}}\mid dQ_{n,s}\mid\\
&=&Q_n^{\#}(0)-Q_n(0)+\int_{(0_s,\tau_s]}I(dQ_{n,s}\geq 0) d(Q_{n,s}^{\#}-dQ_{n,s})+I(dQ_{n,s}<0)d(Q_{n,s}-Q_{n,s}^{\#})\\
&=&-\pl Q_n\pl_v^*+Q_n^{\#}(0)+\int_{(0_s,\tau_s]}I(dQ_{n,s}\geq 0) dQ_{n,s}^{\#}-I(dQ_{n,s}<0)dQ_{n,s}^{\#})\\
&\leq&-\pl Q_n\pl_v^*+\pl Q_n^{\#}\pl_v^*\\
&\leq &0,
\end{eqnarray*}
since $\pl Q_n^{\#}\pl_v^*\leq M=\pl Q_n\pl_v^*$.
Thus, this proves that indeed $Q_n^{\#}-Q_n\in {\cal S}$.


Consider  now the squared error loss $L_1(Q)=(Y-Q(X))^2$. Then,
\begin{eqnarray*}
P_n L_1(Q_n^{\#})-P_nL_1(Q_n)&=&\frac{1}{n}\sum_i \{2Y_iQ_n(X_i)-2Y_i Q_n^{\#}(X_i)+Q_n^{\#2}(X_i)-Q_n^2(X_i)\}\\
&=& \frac{1}{n}\sum_i\{2Y_i(Q_n-Q_n^{\#})(X_i)+Q_n^{\#2}(X_i)-Q_n^2(X_i)\}\\
&=&\frac{1}{n}\sum_i \{2(Y_i-Q_n(X_i))(Q_n-Q_n^{\#})(X_i)+2Q_n(X_i)(Q_n-Q_n^{\#})(X_i)+Q_n^{\#2}(X_i)-Q_n^2(X_i)\}
&=&\frac{1}{n}\sum_i 2(Q_n-Q_n^{\#})(X_i)(Y_i-Q_n(X_i))+\frac{1}{n}\sun_i (Q_n-Q_n^{\#})^2(X_i).\end{eqnarray*}
Note that the first term corresponds with $P_n\frac{d}{dQ_n}L_1(Q_n)(Q_n^{\#}-Q_n)$ and the second-order term with $R_{2n}(Q_n^{\#},Q_n)$.
We want to show that $ \frac{1}{n}\sum_i 2(Q_n-Q_n^{\#})(X_i)(Y_i-Q_n(X_i))\geq 0$.
The general equation above $P_n \frac{d}{dQ_n}L_1(Q_n)(f(h,Q_n)) \geq 0$ corresponds for the squared error loss with:
\[
2 P_n -f(h,Q_n)(Y-Q_n(X)) \geq 0.\]
As above shown, we have $f(h,Q_n)$ can be chosen to be equal to $Q_n^{\#}-Q_n$.
So this proves that $P_n (Q_n^{\#}-Q_n)(Y-Q_n)\leq 0$. This proves the desired result for the squared error loss.
Specifically,
\[
d_{n1}(Q_n^{\#},Q_n)=P_n \{L_1(Q_n^{\#})-L_1(Q_n)\}\geq P_n (Q_n-Q_n^{\#})^2.\]
Thus, $P_n  \{L_1(Q_n^{\#})-L_1(Q_n)\}^2\leq C P_n \{L_1(Q_n^{\#})-L_1(Q_n)\}=O_P(n^{-1/2})$ for some $C<\infty$.
As a consequence, using empirical process results (van der Vaart, Wellner), it follows that $(P_n^{\#}-P_n)\{L_1(Q_n^{\#})-L_1(Q_n)\}=O_P(n^{-1/2-\alpha(d)})$, and thus that
\[
d_{n1}(Q_n^{\#},Q_n)=P_n (Q_n^{\#})-Q_n)^2=P_n \{L_1(Q_n^{\#})-L_1(Q_n)\}=O_P(n^{-1/2-\alpha(d)}).\]
This completes the proof of all statements in the lemma. $\Box$
%Given the weak convergence of $Z_{n,4}^{\#}$ and this latter consistency of $Q_n^{\#}$ to $Q_n$, it follows that $X_n^{\#}(Q_n^{\#},G_n^{\#})$ converges weakly $N_0=N(0,\sigma^2_0)$, conditional on $(P_n:n\geq 1)$.


Define $\tilde{\epsilon}_{n}^{\#}=\arg\min_{\epsilon}P_n L_1(Q_{n,\epsilon}^{\#})$ as the target of $\epsilon_n^{\#}$ and assume the weak regularity condition
\begin{equation}\label{Qnstarconvb}
\tilde{\epsilon}_{n}^{\#}=O_P(d_{n1}^{1/2}(Q_n^{\#},Q_n) ).\end{equation}
Then,
\[
d_{n1}(Q_{n}^{\#*},Q_n)\leq d_{n1}(Q_n^{\#},Q_n)+O_P(n^{-1/2-\alpha(d)}).\]


Specifically,
\begin{eqnarray*}
d_{n1}(Q_n^{\#*},Q_n)&\leq& d_{n1}(Q_n^{\#},Q_n)-(P_n^{\#}-P_n)L_1(Q_{n,\tilde{\epsilon}_{n}^{\#} }^{\#},Q_n^{\#}) \\
&\leq& -(P_n^{\#}-P_n)L_1(Q_n^{\#},Q_n)-(P_n^{\#}-P_n)L_1(Q_{n,\tilde{\epsilon}_{n}^{\#} }^{\#},Q_n^{\#}) \\
&=&-(P_n^{\#}-P_n)L_1(Q_{n,\tilde{\epsilon}_{n}^{\#} }^{\#},Q_n).
\end{eqnarray*}

Under a weak regularity condition, we have $\epsilon_n^{\#}-\tilde{\epsilon}_{n}^{\#}=O_P(n^{-1/2})$.
Then,
\[
d_{n1}(Q_n^{\#*},Q_n)\leq -(P_n^{\#}-P_n)L_1(Q_n^{\#*},Q_n)+O_P(n^{-1}).\]
\end{lemma}


%This also proves that the iterative TMLE using a {\em finite} (uniform in $n$) number of iterations satisfies $d_{01}(Q_n^*,Q_0)\leq -(P_n-P_0)L(Q_n,Q_0)+O_P(n^{-1})$. So  if needed  one can iterate the TMLE to guarantee that $r_n$ is small enough to be neglected. \newline
{\bf Proof:}
We have
\begin{eqnarray*}
P_nL_1(Q_n^{\#*})-P_nL_1(Q_n)&=&\{ P_nL_1(Q_{n,\epsilon_n^{\#}}^{\#})-P_nL_1(Q_{n,\tilde{\epsilon}_{n}^{\#}}^{\#} )\}\\
&&+\{P_nL_1(Q_{n,\tilde{\epsilon}_{n}^{\#}}^{\#} )-P_nL_1(Q_n^{\#})\}\\
&&+P_nL_1(Q_n^{\#})-P_nL_1(Q_n) \\
&\leq &  \{P_nL_1(Q_{n,\tilde{\epsilon}_{n}^{\#}}^{\#},Q_n^{\#})\}
+\{P_nL_1(Q_n^{\#},Q_n)\}\\
&=&(P_n-P_n^{\#})L_1(Q_{n,\tilde{\epsilon}_{n}^{\#} }^{\#},Q_n^{\#}) +P_n^{\#} L_1(Q_{n,\tilde{\epsilon}_{n}^{\#} }^{\#},Q_n^{\#})
\\
&&+d_{n1}(Q_n^{\#},Q_n)\\
&\leq &-(P_n^{\#}-P_n)L_1(Q_{n,\tilde{\epsilon}_{n}^{\#} }^{\#},Q_n^{\#}) +d_{n1}(Q_n^{\#},Q_n).
\end{eqnarray*}
An exact first order Tailor expansion $f(\tilde{\epsilon}_{n}^{\#})-f(0)=\frac{d}{d\xi}f(\xi)\tilde{\epsilon}_n^{\#}$ for a $\xi$ between $0$ and $\tilde{\epsilon}_n^{\#}$, we obtain
\[L_1(Q_{n,\tilde{\epsilon}_{n}^{\#} }^{\#},Q_n^{\#})
=\tilde{\epsilon}_n^{\#}\frac{d}{d\xi}L_1(Q_{n,\xi}^{\#}).\]
It then follows that $(P_n^{\#}-P_n)L_1(Q_{n,\tilde{\epsilon}_n^{\#} }^{\#},Q_n^{\#})=O_P(n^{-1/2-\alpha(d)})$. This proves the first statement of the lemma.
The subsequent statement follow by our precise bounds above and that $d_{n1}(Q_n^{\#},Q_n)\leq -(P_n^{\#}-P_n)L_1(Q_n^{\#},Q_n)$.
$\Box$


==> refs.tex <==
(right-continuous and left-hand limits, \citep{Neuhaus71}) 

An estimator is asymptotically efficient if and only if it is asymptotically linear with influence curve equal to the canonical gradient (also called the efficient influence curve) of the pathwise derivative of the target parameter \citep{Bickeletal97}. 

 Such general estimating equation methodology for construction of efficient estimators  has been developed for censored and causal inference models in the literature (e.g.,  \citep{mark,Robins&Rotnitzky92}).
 
 The one-step TMLE of the target parameter is now the resulting plug-in estimator \citep{vanderLaan&Rubin06,vanderLaan08, vanderLaan&Rose11}.

In this article we focus on the one-step TMLE since it is a more robust estimator by respecting the global constraints of the statistical model, which becomes evident when comparing the one-step estimator and TMLE   in simulations for which the information is low for the target parameter (e.g., even resulting in one-step estimators of probabilities that are outside the (0,1) range) 
%\citep{Bembom&vanderLaan07,Rose&vanderLaan08,Rose&vanderLaan09,Rose&vanderLaan11,Moore&vanderLaan09, Moore&vanderLaan092, Moore&vanderLaan093,Bembometal09b,Neugebauer&Silverberg&vanderLaan10,Polley&vanderLaan09,Rosenblumetal09,vanderLaan&Gruber10,Stitelman&vanderLaan10,Gruber&vanderLaan10a,Rosenblum&vanderLaan10,Wang&Rose&vanderLaan10,Diaz11,Diaz12,Diaz13a,Diaz13b,Diaz13c,Stitelman&vanderLaan11a,vanderLaan10,Stitelman&vanderLaan11,Schnitzeretal13,Gruber&vanderLaan12,Gruber&vanderLaan12a,Petersen&Schwab&vanderLaan13,Brooks2013,Brooks2012,Sapp&vanderLaan13,Neugebaueretal13,ndeu,tmle_safety,subbaraman2013cravings,bsatmle,vanderLaan&Petersen&Zheng13, Zheng&vanderLaan12a,Zheng&vanderLaan12b,
(e.g., \citep{porteretal11,sekhonetal12,Gruber&vanderLaan10a}).

with a  super-learner based on a 
large library of candidate estimators \citep{vanderLaan&Dudoit03,vanderVaart&Dudoit&vanderLaan06,vanderLaan&Dudoit&vanderVaart06,vanderLaan&Polley&Hubbard07,Chpt3}.

the super-learner will also have excellent practical performance for finite samples relative to competing estimators \citep{Polleyetal12}. 
 Based on this fundamental result for the HAL-estimator and the super-learner, we proceed in this article with proving a general theorem for asymptotic efficiency of the one-step TMLE for arbitrary statistical models.
 In this article we  will use a  one-step cross-validated-TMLE (CV-TMLE), which avoids the Donsker-class entropy condition on the nuisance parameter space, in order to further minimize the conditions for asymptotic efficiency \citep{Zheng&vanderLaan12,vanderLaan&Rose11}. 
 In our accompanying technical report \citep{vanderLaan15} we present the analogue results for the one-step TMLE.
Beyond establishing these fundamental theoretical general results, we will also discuss the practical implementation of the HAL-estimator and corresponding TMLE.

By using a recent empirical process result by \citep{vanderVaart&Wellner11} we can establish  an upper bound for this  rate  of convergence in terms of the entropy of the model space. Here we rely on the fact that the space of Cadlag functions that have variation norm smaller than a constant $M$ is a convex hull of indicator functions, and, as a consequence, it is a Donsker class. So, by selecting $M$ larger than the unknown variation norm of the true nuisance parameter value, we obtain an initial estimator that converges at a faster rate than $n^{-1/4}$. 


this TMLE updating algorithm converges in one-step, and we developed a so called universal least favorable submodel that guarantees this convergence in one-step \citep{vanderLaan&Gruber15}.

Our proof of Lemma \ref{tmlelemma2} in Section \ref{section4}, which establishes the rate of convergence of the $M$-specific HAL-estimator, relies on an empirical process result by \citep{vanderVaart&Wellner11} that expresses the upper bound for this  rate  of convergence in terms of the entropy of the model space ${\cal Q}_1$ of $\bar{Q}$. 
The representation (\ref{cadlagrepresentation}) demonstrates that the set of  cadlag functions that have variation norm smaller than a constant $M$ is a difference of  a``convex'' hull of indicator functions, and, as a consequence of a general convex hull result in \cite{vanderVaart&Wellner96} this proves that  it is a Donsker class with a specified upper bound on its entropy. In this way, we obtain an explicit entropy bound for our model space ${\cal Q}_1$. Given this explicit upper bound for the entropy, the result in \citep{vanderVaart&Wellner11} establishes a rate of convergence of the $M$-specific HAL-estimator faster than $n^{-1/4-\alpha_1}$ for a specified $\alpha_1>0$. By selecting $M$ larger than the unknown variation norm of the true nuisance parameter value, we obtain an HAL-estimator that converges at a faster rate than $n^{-1/4}$.

For a $f\in \opend[0,\tau]$, we define  the variation norm of $f$ \citep{Gill&vanderLaan&Wellner95}  as
\begin{equation}\label{variationnorm}
\pl f\pl_v=\mid f(0)\mid +\sum_{s\subset \{1,\ldots,d\}}\int_{(0_s,\tau_s]}\mid f(dx_s,0_{-s})\mid .
\end{equation}
We will now apply Theorem \ref{thcvtmle} to the example introduced in Section \ref{section2}. 
We have the following sieve model bounds  \citep{vanderLaan&Dudoit&Keles04}: $M_{1Q,n}=O(\log \delta_n^{-1})$; $M_{2Q,n}= O(1/\delta_n)$; $M_{1G,n}=O(\log \delta_n^{-1})$; $M_{2G,n} =O(1/\delta_n)$; $M_{D^*,n}= O(1/\delta_n)$.


By now, we also have implemented the HAL-estimator for nonparametric regression and dimensions $d\leq 10$, and established that its practical performance appears to be very good
\citep{Benkeser&vanderLaan16}. 

In this article we assumed independent and identically distributed observations. Nonetheless, this type of super  learner and the resulting asymptotic efficiency of the one-step TMLE will be generalizable to a variety of dependent data structures such as data generated by a statistical graph that assumes sufficient conditional independencies so that the desired central limit theorems can still be established \citep{vanderLaan08,Chambaz&vanderLaan11a,Chambaz&vanderLaan11b,vanderLaan&Balzer&Petersen13,vanderLaan12network}.  


This article focused on a CV-TMLE that represents the statistical  target parameter  $\Psi(P)$ as a   function  $\Psi(Q_1(P),\ldots,Q_{k_1+1}(P))$ of variation independent nuisance parameters $(Q_1,\ldots,Q_{k_1+1})$. However, there are key examples in which representing $\Psi(P)$ in terms of recursively defined nuisance parameters has key advantages. For example, the longitudinal  one-step TMLE  of causal effects of multiple time point interventions  in \citep{Gruber&vanderLaan12,Petersen&Schwab&vanderLaan13} relies on a sequential   regression representation of the target parameter \citep{Bang&Robins05}.  In this case,  the next regression is defined as the regression of the previous regression on a shrinking history, across a number of regressions, one for each time point at which an intervention takes place.



In \citep{vanderLaan&Dudoit03,vanderLaan&Petersen12,Diaz13}  we establish oracle inequalities  for the cross-validation selector based on loss-functions indexed by an unknown nuisance parameter, which now also rely on a remainder concerning the rate at which $\hat{Q}_{k_1+1}(P_n)$ converges to $Q_{k_1+1,0}$. In this manner, one can establish that the super-learner of $Q_{k_1,0}$ will converge at the same or better rate than

Gill 89 bootstrap delta method.

refs for higher order influence functions:


In this chapter we propose a novel second-order TMLE of a second-order pathwise-differentiable target parameter, based on $n$ independent draws from an unknown element of a given semiparametric model. We will refer to this estimator as a $2$-TMLE, with $1$-TMLE corresponding to the usual first-order TMLE. Analogously to the large-sample properties of the usual TMLE requiring the asymptotic negligibility of a second-order remainder term, the asymptotic normality and efficiency of this $2$-TMLE will rely on the asymptotic negligibility of a third-order remainder term. As an illustration of its construction, we develop a $2$-TMLE of a point intervention G-computation parameter based on observing $n$ independent and identically distributed copies of a random vector consisting of baseline covariates, a binary treatment and a final binary outcome. While for simplicity of presentation and brevity we exclusively focus on $2$-TMLE in this chapter, the techniques are readily generalized to an arbitrary order. Further details regarding this generalization can be found in a technical report \citep{carone2014techreport}.

In many problems, the target parameter is only first-order pathwise-differentiable and a second-order gradient does not exist. As a solution, we propose a $2$-TMLE based on an approximate second-order gradient and present a corresponding theory. This additional approximation yields a supplementary bias term for the resulting $2$-TMLE, referred to as the \emph{representation error} in \cite{robins2009metrika}, and the asymptotic linearity and efficiency theorem of the $2$-TMLE requires this bias term to be asymptotically negligible as well. Control of this bias term can be carried out within the standard TMLE framework at no risk of losing the desirable properties of the first-order TMLE.  In our example, we demonstrate that, for an appropriate choice of kernel and bandwidth rate, and provided the data-generating distribution satisfies certain smoothness conditions, the asymptotic efficiency of the $2$-TMLE still only relies on the asymptotic negligibility of a third-order remainder term. We also propose a data-adaptive bandwidth selector based on the C-TMLE framework, essentially selecting the bandwidth maximizing bias reduction in the targeting step of the TMLE. We illustrate the use of $2$-TMLE by describing how it can be implemented to infer about a point intervention G-computation parameter and we report numerical results from its use, all of which are discussed in great detail in \cite{diaz2016ijb}.

 If there exists an element $D^{(1)}(P)\in
L_0^2(P)$ such that for any $P_1,P_2\in\mathscr{M}$ the linearization 
\begin{align*} 
  \Psi(P_2)-\Psi(P_1)\ &=\ (P_2-P_1) D^{(1)}(P_2)+R_2(P_1,P_2)\\
                   &=\ -P_1D^{(1)}(P_2)+R_2(P_1,P_2)
\end{align*} 
holds with $R_2(P_1,P_2)/\Delta(P_1,P_2)\rightarrow 0$ as
$\Delta(P_1,P_2)\rightarrow 0$ for some distance $\Delta$ on
$\mathscr{M}$, then $\Psi$ is said to be \emph{strongly
  differentiable} over $\mathscr{M}$ and any such element $D^{(1)}(P)$
is called a first-order gradient of $\Psi$ at $P$
\citep{pfanzagl1982}. 



A simple but key observation is that, for the sake of ascribing
additional properties to the TMLE, a targeted estimate $g_n^*$ of
$g_0$ can be constructed to solve specified equations and $Q_n^*$ can
easily be tailored to solve additional equations of interest. This is
accomplished notably by incorporating additional parameters in the
least-favorable parametric submodel through $(Q_{n,0},g_{n})$. This
generality of TMLE has been utilized in several instances before
(e.g.,
\citealp{vanderLaan:Rubin06,rubin2011tmlebook,vanderLaan:Rose11,gruber2012ijb,lendle2013techreport,vanderLaan14a})
and plays a fundamental role in the construction of a higher-order
TMLE, as described in this article.


olds for some element $D^{(2)}(P_2)\in L_0^{2*}(P_2^2)$ and a third-order
remainder term $R_3(P_1,P_2)$ such that
$R_3(P_1,P_2)/\Delta^2(P_1,P_2)\rightarrow 0$ as $\Delta(P_1,P_2)\rightarrow 0$
for some distance $\Delta$ on $\mathscr{M}$, then $\Psi$ is said to be
\emph{second-order strongly differentiable} over $\mathscr{M}$.  Any
such element $D^{(2)}(P)$ is called a second-order gradient of $\Psi$
at $P$ \citep{pfanzagl1985}.

In order to construct a $2$-TMLE, it will be necessary to identify a
gradient $D^{(2)}(P)\in L_0^{2*}(P^2)$ such that either
$o_1\mapsto D^{(2)}(P)(o_1,o)$ or $o_2\mapsto D^{(2)}(P)(o,o_2)$ lies
in $T_\mathscr{M}(P)$ for each $o\in\mathcal{O}$.  Any such element
will be referred to as a second-order partial canonical gradient. The
notion of second-order scores, tangent spaces and canonical gradients
have been defined and studied before (see, e.g.,
\citealp{pfanzagl1985,robins2009metrika,vandervaart2014statscience}). 


These
concepts are useful for the sake of obtaining a second-order partial
canonical gradient since, in particular, any second-order canonical
gradient is also a second-order partial canonical gradient. In
Supplementary Material available online, we provide a self-contained overview of these
concepts, including an account of the link between strong
differentiability and pathwise differentiability. We also provide a
constructive approach for obtaining a second-order gradient and
deriving the second-order canonical gradient.


As has been noted in \cite{robins2009metrika}, most statistical
parameters of interest are unfortunately not smooth enough as
functions of the data-generating distribution to allow the required
expansion for $R_2(P_n^*,P_0)$. Thes

ders have been recorded or when the available data are subject
to censoring. C-TMLE, as described, thoroughly discussed and
implemented in \cite{vanderLaan:Gruber10}, \cite{Gruber:vanderLaan10a},
\cite{Stitelman:vanderLaan10}, \cite{vanderLaan:Rose11}, \cite{Wang:Rose:vanderLaan11} 
\cite{gruber2012ijb}, and Chap.~10 of this book, provides a principled solution to this
problem. This approach can readily be utilized here as well.

 This is directly parallel to the advances made in
the seminal work of \cite{robins2009metrika} in the context of the
one-step estimators. Another advantage of including higher-order
partial canonical gradients into the TMLE framework as carried out in
this work is that they yield contributions to the influence
function of the higher-order TMLE that can be directly incorporated in
the construction of confidence intervals, thereby possibly leading to
finite-sample performance improvements.

The building blocks of this generalization were set several decades ago, notably in the works of J. Pfanzagl \citep{pfanzagl1985}, wherein the notion of higher-order gradients was introduced and higher-order expansions of finite-dimensional parameters over arbitrary model spaces were formalized. In this work, we seek to utilize higher-order expansions to enable and guide the construction of regular and asymptotically linear estimators of statistical parameters in rich infinite-dimensional models. This is the perspective that motivated the seminal contributions of J. Robins, L. Li, E. Tchetgen \& A. van der Vaart (e.g., \citealp{robins2008imsnotes,robins2009metrika,li2011statsprobletters,vandervaart2014statscience}); these authors are the first to have provided a rigorous framework for precisely addressing this problem. The first exposition is that of \cite{robins2008imsnotes}, where the focus resides primarily on the use of higher-order gradients to derive optimal estimators in settings where regular estimation is not possible. Subsequent works are concerned with the development of a higher-order analogue of the one-step estimator introduced early on in \cite{levit1975}, \cite{ibragimov1981}, \cite{pfanzagl1982} and \cite{bickel1982annals}, for example. The general approach is thus to identify the dominating terms of an asymptotic expansion for a naive plug-in estimator and to perform, accordingly, an additive correction on this naive estimator. In \cite{robins2009metrika}, the authors carefully establish the required foundations of a second-order extension of this approach and illustrate its use in the context of two problems, namely that of estimating the integral of the square of a density function and of estimating the mean response in missing data models. In \cite{li2011statsprobletters}, the authors study in great detail the problem of inferring a treatment effect using this approach and also establish minimax rate results for certain situations in which regular inference is not possible.

An excellent review of the general higher-order extension of the one-step  estimator is provided in \cite{vandervaart2014statscience}. The one-step  estimator is simple and easy to describe. However, in finite samples, it is vulnerable to decreased performance since it does not include any safeguard ensuring that the additive correction performed on the naive plug-in estimator does not drive the estimator near and possibly beyond the natural bounds of the parameter space. Rather than performing post-hoc bias correction in the parameter space, as does the one-step procedure, the TMLE framework, which we focus on in this chapter, provides guidelines for constructing an estimator of the underlying data-generating distribution, or whichever portion of it is needed to compute the parameter of interest, such that the resulting plug-in estimator enjoys regular and asymptotically linear asymptotic behavior. As such, the correction step is  performed in the model space rather than in the parameter space. The appeal of devising such an approach, even decades before its formal development, was highlighted in \cite{pfanzagl1982}. Since the resulting estimator automatically satisfies bounds on the parameter space, it never produces nonsensical output, such as a probability estimate outside the unit interval, and can outperform in finite samples asymptotically equivalent estimators that do not have a plug-in form. This issue arises when comparing first-order TMLE and one-step  estimators, but is likely of even greater importance in higher-order inference due to the increased complexity of the correction process.

As is highlighted by \cite{robins2009metrika} and discussed in this chapter, higher-order gradients do not exist for several statistical parameters of interest. Nonetheless, approximate higher-order gradients can be used to produce regular estimators. In practice, the notion of approximate higher-order gradients necessarily involves the selection of certain tuning parameters. This requirement is discussed in \cite{robins2009metrika} but practical guidelines are neither provided nor appear particularly easy to develop. An advantage of using TMLE in this context, as we discuss later, is that the selection of such tuning parameters can be effortlessly embedded in the framework of collaborative TMLE, hereafter referred to as C-TMLE. Thus, the practical complications associated with the need for carefully-tuned approximations in the context of inference based on higher-order expansions can be tackled readily. Furthermore, as will be discussed, the framework of TMLE also provides useful tools that aim to guarantee that the resulting higher-order estimator will not behave worse than the usual first-order TMLE.




==> simulation.tex <==
\section{Simulations} \label{sectsimul}

\subsection{Bootstrap HAL-TMLE using optimal tuning for
inference}\label{sec:lambda_star}

\textbf{[this subsection will be moved to method sections later]}

The nuisance parameter estimates $Q_n$ and $G_n$ are key inputs of the HAL-TMLE
bootstrap. The HAL estimations of these nuisance parameters depend largely on
the selection of the upper bound of the sectional variation norm $M$, or
equivalently, selection of L-1 penalty hyper-parameter $\lambda$. We will use the L-1 penalty formulation to refer to
the tuning of HAL-MLE. Under finite sample, when the true sectional variation norm
of the distribution is high ($\lambda_0$ is small), the cross-validated HAL will
tend to balance the bias-variance trade-off, which often results in the
cross-validation selected sectional variation norm to be smaller than the oracle
value ($\lambda_{CV} > \lambda_0$). Such trade-off minimizes the out-of-sample
MSE of the point TMLE $\Psi(Q^*_n)$, but might not be the optimal choice for
doing bootstrap. If we fix the same cross-validation selected $\lambda$
($\lambda_{CV}$) when we fit HAL on the bootstrap samples, the estimated
bootstrap distribution will under-estimate the variability of the sampling
distribution. As a result, the bootstrap interval will be anti-conservative and
will under cover.

We propose a modified bootstrap method, where the tuning parameter $\lambda$ for
both initial HAL estimate and bootstrap HAL are fixed at an optimal value
$\lambda_{optimal}$. Ideally, we want $\lambda_{optimal}$ to be equal to
$\lambda_0$. However, $\lambda_0$ is unknown from the sample, so
we come up with a good proxy for $\lambda_0$ using a newly proposed
`plateau tracking' method. Consider a pre-specified sequence of lambda
candidates $\Lambda = (\lambda_1, \lambda_2, ..., \lambda_J)$, and for each one
of them, we can compute the width of the Wald-type TMLE confidence interval
$(w_1, w_2, ..., w_J)$. Without loss of generality, we assume the lambda
sequence is decreasing ($\lambda_1 > \lambda_2 > ... > \lambda_J$), which forms
a sequence of HAL$_{\lambda_j}$, $j = 1, ..., J$ with increasing sectional
variation norm constraints. As a result, the interval width monotonically
increases and then plateaus ($w_1 < w_2 < ... < w_J$). Through numerical
simulation, we observe that $\lambda_0$ is close to where the plateau begins.
The `plateau tracking` method then computes the $\lambda_{optimal}$ at which the
plateau begins, which is characterized by the second derivative of the
`width-log($\lambda$)` curve is the most positive. More rigorously,
$\lambda_{plateau} \triangleq \lambda_j$, where $$j = \arg\max_{j = 2,...,J - 1}
\frac{(w_{j + 1} - w_j) - (w_j - w_{j - 1})}{(\log ({\lambda _{j + 1}}) - \log
(\lambda _j))(\log (\lambda _j) - \log (\lambda _{j - 1}))}$$

Figure \ref{fig:plateau_exist} illustrates a simulated example of the
`width-$\log(\lambda)$` curve. As the value of $\lambda$ decreases, there are
two plateaus where the width of the confidence interval stabilizes. When
$\lambda > \lambda_{CV}$, HAL-MLE is biased and decreasing $\lambda$ will
increase the spread of the sampling distribution of $\Psi(Q_n(\lambda))$. When
$\lambda <= \lambda_{CV}$, the sampling distribution of $\Psi(Q_n(\lambda))$
will stay stable and the width of the interval will reach the first plateau,
until $\lambda \approx \lambda_0$. When $\lambda < \lambda_0$, the
$Q_n(\lambda)$ is clearly overfitting and the resulting $\Psi(Q_n(\lambda))$
distribution will increase again until it reaches some upper bound allowed by
the data generating distribution. Thus, we believe by looking for the beginning
of the second plateau which is close to $\lambda_0$, we can find a good
candidate for $\lambda_{oracle}$.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\textwidth]{./fig/lambda_plateau_1e3.png}
    \caption{A simulated example of Wald-type interval width as a function of $\lambda$. Dotted line indicate $\lambda_0$, dashed line indicate $\lambda_{CV}$ and solid line indicate $\lambda_{plateau}$}
    \label{fig:plateau_exist}
\end{figure}

\paragraph{RMSE-scaled bootstrap}\label{sec:rmse_scaled}
Another modification of the bootstrap method concerns with the bias of the
bootstrap distribution. As we know from the bootstrap theory, the bootstrap
distribution will approximate all moments of the sampling distribution.
Therefore, not just the variance, but also the bias, will be inherited by the
bootstrap distribution. For example, if there is finite sample bias of
$\Psi^{*}_n$ that is hurting the coverage of Wald-type confidence interval, the
bootstrap distribution can further bias in the same direction, which is not what
we intended for the method. One may say, we can also estimate the bias and
compensate through shifting. However, this is not desirable because the bias
estimate is not reliable. We propose a more sensible modification of the
HAL-TMLE bootstrap, which we call ``RMSE-scaled bootstrap''. Instead of first
estimating the bias, and then compensate the bias back, we widen the bootstrap
confidence interval by replacing the bootstrap standard deviation with the RMSE
in the bootstrap sample, computed against $\Psi^{\#*}_n$ as the truth. More
rigorously in formula, the ``RMSE-scaled bootstrap'' takes the form 
\begin{align}
  [\Psi^*_n - \sigma^\#_n q^{3,\#}_{0.975,n}/n^{1/2}, \Psi^*_n - \sigma^\#_n q^{3,\#}_{0.025,n}/n^{1/2}],
\end{align}
where $\sigma^\#_n \triangleq \sqrt{ \frac{1}{N} \sum_{i =
1}^N{(\Psi^{\#*}_{i,n} - \Psi^*_n) ^ 2} } = \sqrt{bias(\Psi^{\#*}_{i,n})^2 +
stddev(\Psi^{\#*}_{i,n})^2}$ is the estimated RMSE of the bootstrap estimator
$\Psi^{\#*}_n$, and $q^{3,\#}_{\alpha,n}$ is the $\alpha$-quantile of the
bootstrap distribution of standardized estimates $Z^{3,\#}_{i,n} =
n^{1/2}(\Psi^{\#*}_{i,n} - \frac{1}{N} \sum_{i = 1}^N \Psi^{\#*}_{i,n}) / stddev(\Psi^{\#*}_{i,n})$. We
know that $\sigma^\#_n \geq stddev(\Psi^{\#*}_{i,n})$ and that $\sigma^\#_n \leq
|bias(\Psi^{\#*}_{i,n})| + stddev(\Psi^{\#*}_{i,n})$. Therefore, the
``RMSE-scaled bootstrap interval'' is wider than regular HAL-TMLE bootstrap, but
narrower than ``bias-penalized bootstrap'', which add absolute bias on both ends
of the interval.

The full modified HAL-TMLE bootstrap procedure we propose in this paper can be
summarized in the following pseudo-algorithm:

\begin{algorithm}[H]
\caption{modified HAL-TMLE bootstrap procedure}
pre-specify a grid of $\lambda$ values $\Lambda$\;
\For{$\lambda \in \Lambda$}{
    fit HAL-MLE $Q_n$ using tuning parameter $\lambda$\;
    perform HAL-TMLE and record point TMLE $\Psi^*_n(\lambda)$\;
    compute and record the width of Wald-type confidence interval $w(\lambda)$\;
}
perform cross-validation to select $\lambda_{CV}$; record the HAL-TMLE point estimate $\Psi(Q^*_n)$\;
perform `plateau tracking' to select $\lambda_{plateau} \geq \lambda_{CV}$ from $\Lambda$\;
perform HAL-TMLE bootstrap $N$ times where $Q_0$ is re-estimated with $\lambda = \lambda_{plateau}$; compute $\sigma^\#_n = \sqrt{ \frac{1}{N} \sum_{i = 1}^N{(\Psi(Q^{\#^*}_{i,n}) - \Psi(Q^*_n)) ^ 2}}$ \;
% compute the scaling factor $S$\;
report $\Psi(Q^*_n)$ as the final point estimator; report the 95\% confidence interval of the target parameter as $[\Psi(Q^*_n) - \sigma^\#_n q^{3,\#}_{0.975,n}/n^{1/2}, \Psi(Q^*_n) - \sigma^\#_n q^{3,\#}_{0.025,n}/n^{1/2}$ \;
\end{algorithm}


\subsection{Average treatment effect}

To illustrate the finite sample performance of the proposed bootstrap method, we
simulate a continuous outcome $Y$, a binary treatment $A$, and a continuous
covariate $W$ that confounds $Y$ and $A$. The random variables are drawn from a
family of distributions indexed by $a_1$, which characterizes the conditional
distribution of $Y$, given $A$ and $W$. The distribution of variables are as
follows: $W \sim N(0, 4^2, -10, 10)$ is drawn i.i.d. from a truncated normal
distribution with mean equals 0, standard deviation 4, bounded within
$[-10,10]$. $A \sim Bernoulli(p(W))$ is a Bernoulli binary random variable, with
a probability $p(W)$ as a function of $W$, given by
\begin{align*}
    p(W)= 
    \begin{cases}
        0.3,& \text{if } 0.3 + 0.1Wsin(0.1W) + \varepsilon_1 < 0.3\\
        0.7,& \text{if } 0.3 + 0.1Wsin(0.1W) + \varepsilon_1 > 0.7\\
        0.3 + 0.1Wsin(0.1W) + \varepsilon_1, & \text{otherwise}
    \end{cases}
\end{align*}
where $\varepsilon_1 \sim N(0, 0.05^2)$. $Y = 3sin(a_1W) + A + \varepsilon_2$ is
a sinusoidal function of $W$, where $\varepsilon_2 \sim N(0, 1)$. $a_1$ controls
the amplitude of the sinusoidal function. It can be shown that increasing $a_1$
(frequency) of the sin function increases the sectional variation norm, so that
estimating $Q_0$ becomes more difficult under fixed sample size. In our study,
we increase $a_1$ while fixing the sample size so that the second order
remainder increases in magnitude (assuming $\| G_n - G_0 \| = O(n^{-1/2 - \alpha(d)})$,
which is our setting). The value of the parameter of interest, ATE $\Psi_0$, is
1. The experiment is repeated 1000 times. The estimation routine
including the tuning parameter search is implemented in the `ateBootstrap'
function in the open-source R package ``TMLEbootstrap'' \citep{cai2018software}.

To analyze the above simulated data, we computed coverages and widths of (1) the
Wald-type confidence interval where the nuisance functions $(Q_0, G_0)$ are
estimated using HAL($\lambda_{CV}$) and (2) bootstrap confidence interval
discussed in Section \ref{sec:lambda_star} where HAL($\lambda_{plateau}$) is
used for nuisance function estimators. Method (1) reflects common practice in
making TMLE inference. We used correctly specified HAL regression and
classification models to ease computations and focus ideas, but in practice, we
suggest using a SuperLearner \citep{van2007super} which include HAL as part of
the learner library to achieve the best out-of-sample generalizability. Results
under samples sizes 500 and 1000 are shown in Figure \ref{fig:ate-simu}.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=1\textwidth]{./fig/dgd_ate.png}
    \caption{(A) True conditional outcome functions $E(Y|A=1,W)$ and $E(Y|A=0,W)$ at $a_1 = 0.5,1,3,5,10,15$ and (B) true propensity score function}
    \label{fig:ate-dgd}
\end{figure}


\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.9\textwidth]{./fig/simu_ate.png}
    \caption{Results for ATE parameter comparing our bootstrap method and
    classic Wald-type method as a function of the $a_1$ coefficient (sectional
    variation norm) of the $Q_0$ function. Panel A is the coverage of the
    intervals, where dashed line indicate 95\% nominal coverage. Panel B is the
    widths of the intervals. Within each panel, the upper plot is under sample
    size 500 and the lower plot is under sample size 1000.}
    \label{fig:ate-simu}
\end{figure}

The simulations results reflect what is expected based on theory. In particular,
since the sectional variation norm of the $Q_0$ function is large (relative to
sample size), HAL regression fit in the finite sample is not ideal, which leads
to a below than nominal coverage of Wald-type interval. Bootstrap intervals pick
up the second-order remainder, and the coverage is very close to nominal and is
robust to increasing sectional variation norm ($a_1$). The results for sample
size 1000 confirm our asymptotic analysis of the methods, with Wald-type coverage
improving and two methods eventually converging to nominal.

\subsection{Average density value}

It is known that the average density value parameter has non-zero second-order
remainder term after Taylor expansion. To illustrate our proposed method and
explore finite-sample performance, we simulate a family of univariate densities
with increasing sectional variation norm. $$f(x;\theta_K) =
\frac{1}{K}\sum\limits_{k = 1}^K{g(x;\mu_k,\sigma_K)},$$ where
$$g(x;\mu_k,\sigma_K) = \frac{1}{\sqrt{2\pi}
\sigma_K}\exp[-\frac{1}{2}(x-\mu_k)^2/\sigma_K^2].$$ For a given $K$, $\mu_k, k
= 1,...,K$ are equi-distantly placed in interval $[-4,4]$. $\sigma_K=10/K/6$.
The true sectional variation norm of the density increases roughly linearly with
K, that is $||f_K|| = K||f_1||, K = 1,...,13$. Examples of the density family
for $K$ values used in the simulation are shown in Figure \ref{fig:avgdens-dgd}.
We simulate from univariate densities for the sake of presentation and we expect
the results under high dimensional densities to hold true, as the sectional
variation norm can increase more rapidly with increasing number of dimensions.
The value of the parameter of interest $\Psi_0$ is not too variant with $K$. The
experiment is repeated 1000 times. Similar to the analysis for ATE, we compute
interval coverages and widths for (1) Wald-type ($\lambda_{CV}$) and (2)
HAL-TMLE bootstrap ($\lambda_{plateau}$).

The HAL-TMLE consists of a HAL-MLE density learner, combined with a targeting
step through the universal least favorable submodel. The HAL-MLE density learner
first transforms the density estimation task to a longitudinal data format, so
that the original problem reduces to a hazard estimation task where standard
classification algorithms can be directly applied. Predicting the hazard and
transforming back to probability density function retrieves the HAL density
estimator. The software implementations can be found in the `cv\_densityHAL'
function in the open-source R package ``TMLEbootstrap'' \citep{cai2018software}.


\begin{figure}[!ht]
    \centering
    \includegraphics[width=1\textwidth]{./fig/dgd_avgdens.png}
    \caption{True probability density function $f(x;\theta_K)$ at $K = 1,3,5,7,9,11,13$}
    \label{fig:avgdens-dgd}
\end{figure}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.9\textwidth]{./fig/simu_avgdens.png}
    \caption{Results for average density value parameter comparing our bootstrap
    method and classic Wald-type method as a function of the number of modes in
    true density (sectional variation norm). Panel A is the coverage of the
    intervals, where dashed line indicate 95\% nominal coverage. Panel B is the
    widths of the intervals. Within each panel, the upper plot is under sample
    size 500 and the lower plot is under sample size 1000.}
\end{figure}

The simulations reflect what is expected based on theory: bootstrap methods
control type-I error better than Wald-type confidence interval, uniformly across
different sample sizes. In particular, when true sectional variation norm
increases (with the number of modes in the density), non-zero second-order
remainder term increases and Wald-type interval coverage declines. On the other
hand, bootstrap can pick up the non-zero second-order remainder. Bootstrap
confidence interval controls the coverage close to nominal rates and is less
sensitive to the true sectional variation norm of the density function. When
sample size increases to 1000, the Wald-type interval coverage increases, and in
simple cases where the true sectional variation norm is small, Wald-type
coverage can reach nominal. Bootstrap confidence interval keeps nominal and is
robust to the true sectional variation norm.

